Enabling Unstructured Sparse Acceleration on Structured Sparse Accelerators

Exploiting sparsity in deep neural networks (DNNs) has been a promising area for meeting the growing computation requirements. To minimize the overhead of sparse acceleration, hardware designers have proposed structured sparsity support, but it provides limited flexibility and requires extra model fine-tuning. Moreover, any sparse model fine-tuned for certain structured sparse HW cannot be accelerated by other structured hardware. To enable acceleration using unstructured sparsity of DNNs on structured sparse hardware, we propose an approximation method leveraging the distributive property in linear algebra to turn any sparse tensor into a series of structured sparse tensors. We also develop a software framework, TASDER, to apply high-quality structured approximation on weights and activations of DNNs. Our method accelerates dense and sparse DNNs without fine-tuning and improves energy-delay-product (EDP) by up to 83% and 74%. It achieves up to 39% speed-up on a real system.

==> algorithms/find_config.tex <==


\begin{minipage}[t]{\linewidth}
\begin{center}
\vspace{-0.3em}
\begin{lstlisting}[caption={The sparsity-degree-based TASD selection.}\label{lst:tasd},escapechar=\%]
target_sparsity = sparsity + alpha;
if (target_sparsity > H[3]): return H[3];
else if (target_sparsity > H[2]): return H[2];
else if (target_sparsity > H[1]): return H[1];
else if (target_sparsity > H[0]): return H[0];
\end{lstlisting} 

\end{center}
\end{minipage}



==> include/shorthands.tex <==
%%%%% BLUE is same as hyperref, could be confusing, so not keeping here %%%%%
\newcommand{\GJ}[1]{{\color{brown}\bfseries [Geonhwa:: #1]}}
\newcommand{\PT}[1]{{\color{magenta}\bfseries [Po-An:: #1]}} 
%\newcommand{\AB}[1]{{\color{magenta}\bfseries [Abhimanyu:: #1]}}
%\newcommand{\cjh}[1]{{\color{cyan}\bfseries [Chris:: #1]}} 
%\newcommand{\HK}[1]{{\color{violet}\bfseries [Hyesoon:: #1]}}
\newcommand{\SK}[1]{{\color{teal}\bfseries [Steve:: #1]}}
\newcommand{\TK}[1]{{\color{cyan}\bfseries [Tushar:: #1]}}
\newcommand{\todo}[1]{\textcolor{red}{TODO:: #1}}
\newcommand{\rev}[1]{\textcolor{red}{#1}}

% Sections
\def\Snospace~{\S{}}
\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section }


==> mlsys2025style/algorithms/find_config.tex <==


\begin{minipage}[t]{\linewidth}
\begin{center}
\vspace{-0.3em}
\begin{lstlisting}[caption={The sparsity-degree-based TASD selection.}\label{lst:tasd},escapechar=\%]
target_sparsity = sparsity + alpha;
if (target_sparsity > H[3]): return H[3];
else if (target_sparsity > H[2]): return H[2];
else if (target_sparsity > H[1]): return H[1];
else if (target_sparsity > H[0]): return H[0];
\end{lstlisting} 

\end{center}
\end{minipage}



==> mlsys2025style/include/shorthands.tex <==
%%%%% BLUE is same as hyperref, could be confusing, so not keeping here %%%%%
\newcommand{\GJ}[1]{{\color{brown}\bfseries [Geonhwa:: #1]}}
\newcommand{\PT}[1]{{\color{magenta}\bfseries [Po-An:: #1]}} 
%\newcommand{\AB}[1]{{\color{magenta}\bfseries [Abhimanyu:: #1]}}
%\newcommand{\cjh}[1]{{\color{cyan}\bfseries [Chris:: #1]}} 
%\newcommand{\HK}[1]{{\color{violet}\bfseries [Hyesoon:: #1]}}
\newcommand{\SK}[1]{{\color{teal}\bfseries [Steve:: #1]}}
\newcommand{\TK}[1]{{\color{cyan}\bfseries [Tushar:: #1]}}
\newcommand{\todo}[1]{\textcolor{red}{TODO:: #1}}
\newcommand{\rev}[1]{\textcolor{red}{#1}}

% Sections
\def\Snospace~{\S{}}
\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section }


==> mlsys2025style/sections/0_abstract.tex <==
\begin{abstract}

Exploiting sparsity in deep neural networks (DNNs) has been a promising area for meeting the growing computation requirements.
%However, in practice, sparse DNN acceleration still faces a key challenge. 
To minimize the overhead of sparse acceleration, hardware designers have proposed \emph{structured sparsity} support, but it provides limited flexibility and requires extra model fine-tuning. Moreover, any sparse model fine-tuned for certain structured sparse HW cannot be accelerated by other structured hardware.
%To bridge the gap between sparse DNN models and hardware, 
To enable acceleration using unstructured sparsity of DNNs on structured sparse hardware, we propose an approximation method leveraging 
%tensor approximation via structured decomposition (TASD), which leverages 
the distributive property in linear algebra to turn any sparse tensor into a series of structured sparse tensors.
We also develop a software framework, TASDER, to apply high-quality structured approximation on weights and activations of DNNs.
%to accelerate DNNs by searching layer-wise, high-quality structured decomposition for both weight and activation tensors so that they can be accelerated by any systems with structured sparse hardware support.
%by exploiting prior structured sparse hardware baselines
Our method accelerates dense and sparse DNNs without fine-tuning and improves energy-delay-product (EDP) by up to 83\% and 74\%. It achieves up to 39\% speed-up on a real system.
\end{abstract}


==> mlsys2025style/sections/1_intro_old.tex <==
\section{Introduction}

\TK{pls rewrite! see my comment on slack}

DNNs have revolutionized various domains, such as computer vision~\cite{krizhevsky2012alexnet,convnext,vit}, personal recommendation~\cite{dlrm}, speech recognition~\cite{deepspeech2}, and natural language processing~\cite{gpt2,devlin-etal-2019-bert}. 
%Meanwhile, DNNs are also demanding more computation for diverse model capabilities and higher operational performance. The DNN models are scaling to billions of model parameters \cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron} often with high-resolution 2D and 3D inputs~\cite{lin2017focal,cciccek20163d} under real-time requirements.
Meanwhile, DNN inference is also demanding more computation as they scale to billions of model parameters \cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron} and consume an enormous amount of input data~\cite{lin2017focal,cciccek20163d}.
%Recently, Deep Learning (DL) has achieved great success across various domains including, but not limited to, computer vision, personal recommendation, speech recognition, and natural language processing~\cite{lecun2015deep}. 
%To squeeze out the full potential of DNN models with large datasets and powerful compute resources, one of the recent trends is making the model deeper and larger, often exceeding billions or trillions model parameters such as Megatron, PaLM, and Switch Transformer~\cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron}.
%On the other hand, some DNN models use high-resolution inputs to exploit more information from the input to achieve higher accuracy while incurring larger intermediate feature maps as the trade-off.
%The enormous number of parameters and large feature maps cause huge memory footprint as well as an extremely large number of computations, which is a critical problem for both edge devices and datacenter computers.
%Since performance is an overloaded term, we distinguish computational (i.e., latency, throughput, etc.) and operational (i.e., the accuracy of DNN classification) performance in this paper.
To address the increasing demand for DNN models, researchers propose to exploit \emph{sparsity} in DNN models.  
%Fortunately, researchers have found a technique called model compression to reduce the memory footprint and improve performance.
%that there are two sparsities that they can exploit to reduce the burden; weight (static) sparsity and input (dynamic) sparsity; the former is extrinsic while the latter is intrinsic.
%Weight sparsity is the result of a well-known model compression technique, model pruning~\cite{han2015deep}, which removes a set of parameters in the target DNN model based on certain rules, thereby potentially reducing both memory footprint and the required number of computations. 
Model pruning~\cite{han2015deep} is the most popular method to remove a set of parameters in the target DNN model based on certain criteria, inducing \emph{weight sparsity}.
%Weight sparsity is often called as static sparsity since the sparsity pattern is fixed across different inferences using the model.
This optimization exploits a phenomenon that empirically, large models are often overly parameterized and do not need all parameters to maintain the target accuracy at inference time.
Deep learning (DL) model developers prefer to induce \textbf{unstructured sparsity} on weights so that they can focus on developing pruning algorithms to achieve better model accuracy and computation/model size trade-offs without any restriction.
Also, many DNN models naturally exhibit \emph{activation sparisty} due to the rectified linear unit (ReLU) that clips negative activation values to zeros, which induces unstructured activation sparsity.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/tasd-high-level-fig.pdf}
 \vspace{-1.5em}
	\caption{Different flows to exploit sparsity in DNNs.}
 \vspace{-1.5em}
	\label{fig:tasd-high-level-fig}
\end{figure}
%While unstructured sparsity is the preferred method to compress DNNs, 
As a result, early sparse DNN accelerators~\cite{parashar2017scnn,wang:dual-side,qin2020sigma} target unstructured sparsity and can accelerate any sparse DNNs.
Unfortunately, unstructured sparsity support is challenging to deploy as a specialized HW unit 
%support for unstructured sparsity in commercial devices, 
as it causes significant area and energy overhead for indexing logic and flexible distribution/reduction logic~\cite{jeong:vegeta}.
Without native HW support, unstructured sparsity in DNNs lead to irregular memory accesses and diverged control/execution patterns, which are hostile to parallel architectures like GPUs%
\footnote{The only sparse DNN accelerators on commercial devices is NVIDIA Sparse Tensor Core\cite{nvidia_ampere}, which supports a fixed 2:4 
 structured sparsity.} and specialized tensor accelerators like tensor core and systolic array. 
This forces DNN model developers today to constrain the DNN sparsity search space to only consider coarse-grained \emph{structured patterns}, such as channel or filter pruning~\cite{molchanov2022lana, chen2022coarsening}, while maintaining iso-accuracy, thereby, moving the burden to DNN model developers.

%To address this issue, an alternative to bridge
%DNN sparsity and HW performance is to introduce extra design
%spaces that are parallel HW-oriented, namely structure (or
%the degree of structuredness) and granularity.
To balance the need, recently, hardware (HW) designers~\cite{nvidia_ampere,jeong:vegeta,liu2021s2ta,zhu2019micro} have proposed \emph{fine-grained} structured sparsity support.
Such designs force DNN developers to induce sparsity with certain constraints at a cost of achievable sparsity degree for iso-accuracy comparison, but promise predictable performance
gain on top of the existing DNN supports.
For example, NVIDIA’s fine-grained 2:4 structured sparsity support balances the imposed constraints and achievable performance and provides a good target for DNN developers to optimize the network for.
However, such methods impose an extra burden on DNN developers on top of the existing huge design space (DNN architectures, training recipes, etc.) to explore. Moreover, extending the existing support to more patterns~\cite{jeong:vegeta, sun2021domino} means more overhead and design space exploration for both HW designers and DNN developers.
We summarize different flows to exploit sparsity in \autoref{fig:tasd-high-level-fig}.

%In this paper, we ask "how can we design a system to provide the unstructured sparse interface to the DNN developers, but only with structured sparse hardware support, while providing predictable performance and efficiency gains?" 
\textbf{In this paper}, we ask ``Can we design a system to expose the flexible unstructured sparse interface to the DNN developers, but only with the efficient, less flexible structured sparse HW support?" 
Our answer is to introduce a new level of abstraction between DL model developers and hardware designers, similar to the abstraction layer in the instruction-set architectures. Specifically, we introduce a method, structured sparse tensor decomposition, to approximate any sparse tensor with a series of structured sparse tensors.
Leveraging the distributed property of tensor algebra,
we further propose to dynamically "decode" an unstructured
sparse tensor algebra into a series of "microcode", i.e., structured sparse tensor algebra, which are efficient and compatible with prior structured sparse hardware.
%\TK{I think somewhere in this section or in the first bullet a strong statement like ``First work to .." will be nice to have}
%To exploit the benefits of both approaches, we propose a novel method, Tensor Approximation via Structured Decomposition (TASD) and show how it can be used to leverage unstructured input sparsity using a set of structured sparse tensors.
%Furthermore, we have observed that different layers prefer different TASD configurations, so we propose an efficient method to choose TASD configurations per layer to minimize accuracy loss while maximizing performance gain.

We make the following contributions: 
\begin{itemize}
    \item We present the first work to bridge unstructured sparse DNN and structured sparse HW with Tensor Approximation via Structured Decomposition (TASD), which approximate any sparse tensor with a series of structured sparse tensors.
    \item We propose a framework, TASDER, which finds the TASD series for each DNN layer to accelerate dense/sparse DNNs with structured sparse hardware.
    \item We propose a simple architectural extension and dataflow on top of existing structured sparse accelerators~\cite{jeong:vegeta} to execute TASD series efficiently.
    \item For various off-the-shelf dense and sparse DNNs, we show that TASD improves EDP by up to 83\% and by 70\% on average. We also show that across a range of DNNs, TASD can reduce the computation by 40\%. We validate the effectiveness of TASD on a real NVIDIA GPU and achieve up to 39\% speed-up.
\end{itemize}


\begin{comment}
The organization of the paper is the following.
\begin{itemize}
    \item Section 2 reviews the background in DNN sparsity and
how DNN developers induce sparsity, as well as previous HW support DNN sparsity. We also show why
providing unstructured sparse HW support might not
be the best solution.
    \item Section 3 explains the idea of TASD and a preliminary analytical study of how effective TASD is as an
approximation method.
    \item Section 4 describes a TASD-based HW and SW codesign that enables the DNN developer to freely induce
sparsity without structured and granularity constraints.
    \item Section 5 shows the evaluation of the proposed system,
as well as a case study of applying TASD on off-the-shelf HW (NVIDIA Ampere GPUs).
    \item Finally, we discuss extra related work in Section 6 and conclude this paper in section 7.
\end{itemize}
\end{comment}

%Thus, For example, the only commercial HW that can leverage sparsity for efficient calculation is NVIDIA Sparse Tensor Core.
%During the pruning, This HW-agnostic design space and preference from the developer leads to a friendlier abstraction toward unstructured
%sparsity, because the designer does not need to think about
%HW, just to focus on the network accuracy and flops/model size tradeoff.





==> mlsys2025style/sections/1_new_intro.tex <==
\section{Introduction}
%My suggestion is to talk purely about 
% 1. sparsity being promising from model side but extremely expensive to support in HW .. 
% 2. then talk purely about HW - how there is a spectrum of choices (i think the figure from your thesis talk may be valuable) .. cite the diff works .. and show how HW is converging towards structured - mentioning NVIDIA STC, VEGETA etc ..
%And then say this limits this HW to only be used if model is trained in structured manner. And then say this work allows any unstructured sparse model to run on structured HW ..

%speech recognition~\cite{deepspeech2}, 
%DNNs have revolutionized various domains, such as computer vision~\cite{krizhevsky2012alexnet,convnext,vit}, personal recommendation~\cite{dlrm}, and natural language processing~\cite{gpt2,devlin-etal-2019-bert}. 

DNNs have revolutionized various domains~\cite{krizhevsky2012alexnet,convnext,vit, dlrm, gpt2,devlin-etal-2019-bert}, but DNN inference demands extreme compute power, memory footprints, and memory bandwidth as models scale to billions and trillions of parameters \cite{shoeybi2019megatron, fedus2021switch, chowdhery2022palm}.
%touvron2023llama2openfoundation
%and large input datasets~\cite{lin2017focal,cciccek20163d}.
To mitigate this growing demand, \emph{sparsity} has emerged as a promising opportunity. 
%DNN models.  
Model pruning~\cite{han2015deep} is the most popular method to remove a set of parameters in DNNs.
%based on certain criteria. %, inducing \emph{weight sparsity}.
This optimization exploits a phenomenon that large models are often overly parameterized and do not need all parameters to maintain the target accuracy. % at inference time.
Model pruning induces unstructured sparsity on weights (i.e. there is no specific pattern in the distribution of zeros) \text{unless} constraints are enforced during the pruning.
Also, many DNN models naturally exhibit activation sparsity due to the rectified linear unit (ReLU) that clips negative activation values to zeros resulting in unstructured sparsity.

%While unstructured sparsity is the preferred method to compress DNNs, 

Unfortunately, unstructured sparsity in DNNs leads to irregular memory accesses and diverged control/execution patterns, which are hostile to parallel architectures like GPUs, tensor cores~\cite{nvidia_volta}, and systolic arrays~\cite{jouppi2017tpu}. 
%and specialized dense tensor accelerators like tensor cores~\cite{nvidia_volta} and systolic arrays~\cite{jouppi2017tpu}.
This has led to a plethora of academic research on unstructured sparsity support in DNN accelerators~\cite{parashar2017scnn, extensor,qin2020sigma,wang:dual-side, eureka2023micro}. 
Nonetheless, the complexity in hardware required for unstructured sparsity, such as indexing logic~\cite{extensor} and flexible distribution/reduction logic~\cite{qin2020sigma}, has been prohibitive in their commercial adoption.

%nvidia_hopper
Recent sparse DNN accelerators \cite{zhu2019micro,nvidia_ampere, liu2021s2ta, jeong:vegeta, AMD_MI300, Moffett_antoum} have proposed \textit{structured sparsity} support. 
The most popular example is \emph{fine-grained} N:M sparsity, 
which constrains at most N non-zeros in each block composed of M consecutive elements.
A commercial example of this is NVIDIA's sparse tensor core (STC) with 2:4 structured sparsity.
%N:M structured sparsity imposes some degree of regularity in data, allowing lower overhead for sparsity support compared to unstructured sparsity while promising predictable performance gains.
%on top of the existing DNN supports.
Structured sparse hardware forces DNN model developers to induce sparsity with certain constraints. \textit{Otherwise, that hardware is unusable.}
%at a cost of achievable sparsity degree for iso-accuracy comparison.
For example, NVIDIA’s fine-grained 2:4 structured sparsity support could provide 2$\times$ throughput by skipping ineffectual computations \textit{only if} the model is tuned with 2:4 structured sparsity. 
A model that does not follow 2:4 structured sparsity would, in fact, need to run on the dense tensor core, losing the benefits of sparsification.
%\footnote{It may benefit from compressed storage in memory but has to be decompressed and run on dense tensor cores without taking compute benefits.}. 
On the flip side, a 2:4 structured sparse model cannot be accelerated on different structured sparse hardware, such as a sparse tensor core with 1:4 or 2:8 structured sparsity support.
Therefore, while the availability of structured sparse hardware is extremely promising, it remains limiting for model developers as it requires tuning the model to the specific sparsity support of the hardware, in addition to navigating the already vast design space, including DNN architectures and training recipes. This makes the broad adoption of structured sparse hardware challenging.
%Therefore, the availability of structured sparse hardware, while extremely promising, is still very limiting for model developers as it requires tuning the model for the specific sparsity support in the hardware, on top of the already huge design space (DNN architectures, training recipes, etc.) to explore, making the adoption of the structured sparse HW challenging. 
%Moreover, we get no benefits today from the structured sparse hardware for unstructured activation sparsity.
%To execute the model on another HW with 4:8 structured sparsity, the model has to be tuned again to meet the constraint.
%Therefore, such methods impose an extra burden on DNN developers to tune the model for each HW to leverage structured sparsity support on top of the existing huge design space (DNN architectures, training recipes, etc.) to explore, making the adoption of the structured sparse HW difficult. 
%Also, extending existing structured sparse hardware support to more patterns~\cite{jeong:vegeta, sun2021domino} means adding more overhead and a larger design space exploration and cost vs. benefit trade-off space.


%This forces DNN model developers today to constrain the DNN sparsity search space to only consider certain \emph{structured patterns}, such as channel or filter pruning~\cite{molchanov2022lana, chen2022coarsening} while maintaining iso-accuracy, thereby, moving the burden to DNN model developers.

%The only sparse DNN accelerators on commercial devices is NVIDIA Sparse Tensor Core\cite{nvidia_ampere}, which supports a fixed 2:4  structured sparsity.

%Deep learning (DL) model developers prefer to induce \textbf{unstructured sparsity} on weights so that they can focus on developing pruning algorithms to achieve better model accuracy and computation/model size trade-offs without any restriction.
%Also, many DNN models naturally exhibit \emph{activation sparisty} due to the rectified linear unit (ReLU) that clips negative activation values to zeros, which induces unstructured activation sparsity.
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/tasd-high-level-fig.pdf}
 \vspace{-1em}
	\caption{Different flows to exploit sparsity in DNNs.}
 \vspace{-1em}
	\label{fig:tasd-high-level-fig}
\end{figure}

In this paper, we ask and answer the following  question \textbf{``Can we decouple the dependency between DNN models and HW, so that a model with \textit{any sparsity pattern} can be accelerated on \textit{any structured sparse HW}?}"
%Can we design a system to expose the flexible unstructured sparse interface to the DNN developers, but only with the efficient, less flexible structured sparse HW support?" 
Our answer is to introduce a new level of abstraction between DL model developers and hardware designers. %similar to the abstraction layer in instruction-set architectures. 
Specifically, we introduce a method, structured sparse tensor decomposition, to approximate any sparse tensor (such as pruned weights or intrinsic sparse activations) with a series of structured sparse tensors.
%\TK{maybe add a footnote here saying we can also approximate dense tensors with TASD, allowing us to leverage multiple passed through the sparse hardware for dense tensors}
Leveraging the distributed property of tensor algebra,
we further propose to dynamically ``decode" an unstructured sparse tensor algebra into a series of %``microcode", i.e., 
structured sparse tensor algebra, which is efficient and compatible with prior structured sparse hardware. 
%\footnote{In fact, not only for sparse tensors, but also one can use our proposed method to approximate dense tensors to execute it over structured sparse HW, helping utilize sparse HW for dense workloads instead of keeping it idle.}. 
We contrast our proposed approach with current flows to exploit sparsity in \autoref{fig:tasd-high-level-fig}.
%\TK{I think somewhere in this section or in the first bullet a strong statement like ``First work to .." will be nice to have}
%To exploit the benefits of both approaches, we propose a novel method, Tensor Approximation via Structured Decomposition (TASD) and show how it can be used to leverage unstructured input sparsity using a set of structured sparse tensors.
%Furthermore, we have observed that different layers prefer different TASD configurations, so we propose an efficient method to choose TASD configurations per layer to minimize accuracy loss while maximizing performance gain.

We make the following contributions: 
\begin{itemize}
    \item We propose Tensor Approximation via Structured Decomposition (TASD), which approximates any sparse tensor with a series of structured sparse tensors. TASD is the first work to demonstrate running unstructured sparse DNNs on structured sparse HW.
    \item We propose a framework, TASDER, a bridge between HW and SW to find the TASD series % for each DNN layer to 
    to accelerate dense/sparse DNNs on structured sparse hardware.
    \item We propose a simple architectural extension and dataflow on top of existing structured sparse accelerators~\cite{jeong:vegeta} to execute TASD series efficiently.
    %off-the-shelf
    \item For various dense and sparse DNNs, we show that TASD improves EDP by up to 83\% and by 70\% on average. 
    We also show that across a range of DNNs, TASD can reduce the computation by 40\%.
    \item We show the effectiveness of TASD on commercial hardware (NVIDIA RTX 3080 GPU) with 2:4 sparse tensor cores and achieve up to 39\% performance gain.
\end{itemize}

==> mlsys2025style/sections/2_background.tex <==
\section{Background}
%In this section, we first explain several terminologies related to DNN sparsity as different terms are being used interchangeably in various communities such as HPC, ML, and hardware design. 
%Next, we summarize how sparsity is induced in DNN models and we illustrate the prior work on hardware acceleration exploiting DNN sparsity.

\subsection{Terminology}
%\textbf{Tensor} is a generalized form of scalars, vectors, and matrices with an arbitrary number of dimensions (or ranks), $N$, which are used to represent multi-dimensional data.

\textbf{Sparsity} is a characteristic of data that includes zeros. 
The sparsity degree of a given tensor is measured as the fraction of the number of zeros to the number of the total elements in the tensor.
If a tensor has 0\% sparsity degree, we call the tensor \emph{dense}. 
Sparsity by itself is often used to indicate sparsity degree.
To describe the distribution of zeros, a \textit{sparsity pattern} can be given to the tensor.
If there is no defined sparsity pattern, we call it \emph{unstructured sparsity}.
Various patterns can be classified as structured sparsity, such as block sparse~\cite{narang2017block}, butterfly sparse~\cite{dao2021pixelated}, and mixed patterns~\cite{zaheer2020big}.

One of the most popular patterns is \textbf{N:M structured sparsity}~\cite{zhou2021nm}, as it is supported in both commercial products~\cite{nvidia_ampere, AMD_MI300, Moffett_antoum} and academic proposals~\cite{liu2021s2ta,jeong:vegeta, bambhaniya2023accelerating} with active training recipe research~\cite{pool2021channel,mishra2021accelerating, nvidia_asp, NM_training_recipe,lu2023step, sparsegpt, bambhaniya2024progressive}.
% \TK{pls add more citations for N:M training recipe research - to showcase this is an active area. Also add venue (arxiv) for the current cited paper from Amir/Abhi.}.
%\TK{since this is background section, I *think* you can give examples of other structured sparse patterns like block sparse, butterfly (Beidi's paper), N:M .. and then add citations showing recent popularity of N:M and corresponding HW support,  fwd pointing to Sec 2.2 which will have more details.}
An N:M structured sparse tensor means that there can be at most N non-zeros in each M-element block in a certain rank of the tensor as shown in \autoref{fig:sparsity_patterns} (c).
%\autoref{fig:sparsity_patterns} shows different sparsity patterns.
%Sparsity constraint = the rules for the non-zero distribution in a tensor
%\TK{throughout the paper we seem to use structured and N:M interchangeably which is confusing. Maybe put a footnote here clarifying that in paper structured means flexible N:M}

We define \textbf{a view} of a tensor $A$ for a sparsity pattern as a tensor after potentially dropping some elements to meet the rule of the sparsity pattern.
For a matrix filled with non-zeros randomly, it is possible that the matrix does not meet the 2:4 sparsity pattern, i.e. there could be a block composed of 4 consecutive elements with more than two non-zeros.
To generate a 2:4 view of the matrix, some non-zeros in the matrix should be dropped (pruned in DNNs) to meet the pattern. As this process could drop some original values, it can be \textit{lossy}.
\autoref{fig:sparsity_patterns} also shows various tensors under different structured sparse views.

Prior work in DNN accelerators also proposed dense accelerators, unstructured sparse accelerators, 2:4 structured sparse accelerators, etc.
To clarify the nomenclatures, in this paper, \emph{if a sparsity pattern is used to describe a hardware accelerator, that accelerator should provide \textbf{lossless} and native support for any input tensor under such view.}
For example, we call Google TPU a dense accelerator and NVIDIA Sparse Tensor Core a 2:4 accelerator.
%\TK{I think I get what you mean but an example may help here. I think whats confusing is - the prev para said the view can make it lossy.}
%\TK{this is probably one of the most important lines in the paper .. but easy to missesp  .. esp as its in a background section II-A. }
%It also means that the accelerator assumes such a view of the input tensors with the sparsity pattern.
% sparse optimization -- skipping patterns
% hw constraint ISA
%the accelerator assumes a view 
%If a HW assumes a certain view X, then the HW should guarantee to provide the lossless result for any X.
% compressed

%\textbf{Compressed representations:}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.46\textwidth]{figures/different-sparsity-patterns-small.pdf}
 \vspace{-0.5em}
	\caption{Different sparsity patterns and views.
 %\TK{once we add a N:M ``view", shouldnt we add the block around the M elements?}
 }
 \vspace{-1em}
	\label{fig:sparsity_patterns}
\end{figure}
\subsection{DNN SW: Inducing sparsity in DNNs}
%\subsubsection{Sparsity in weights}
\textbf{Weight Sparsity.}
%The most popular method to introduce sparsity in DNNs is model pruning to generate weight sparsity.
%From 1980s, researchers have shown that DNN models are often overly-parameterized so that unimportant weights could be removed without causing loss of accuracy, which can reduce the size of models and the execution runtime while making the model generalize better~\cite{lecun:optimal}. 
Without a specific pattern in mind, common model pruning methods introduces unstructured sparsity in weights~\cite{SparseZoo}. 
%Unstructured sparsity is the most generic sparsity without any specific pattern in the data.
Due to the irregular accesses to handle non-zeros in unstructured sparse matrices, unstructured sparsity is not adequate for accelerating DNNs on the existing parallel hardware, such as GPUs.  

To address the issue, structured pruning forces pre-defined sparsity constraints in weights. For example, \textbf{N:M} structured sparsity~\cite{zhou2021nm,hubara2021accelerated,sun2021domino,mishra2021accelerating,fang2022algorithm,zhang2022learning,NM_training_recipe}
%\TK{add more citations -- there seem to be several N:M training recipe papers} 
ensures there are at most \textbf{N} non-zeros in each block composed of \textbf{M} consecutive elements, so the required acceleration hardware can be trivial by exploiting the regularity in sparsity patterns.
Thus, various accelerators, including recent sparse tensor cores in NVIDIA Ampere GPUs~\cite{nvidia_ampere}, target to exploit the fine-grained structured sparsity instead of unstructured sparsity.
Nonetheless, structured pruning suffers from a higher loss of accuracy~\cite{sparsegpt} than unstructured pruning since the extra pruning constraints reduce the flexibility.
This extra loss of accuracy often leads to longer fine-tuning time (e.g., repeat the whole training process again) than unstructured sparse method to recover the loss in accuracy due to pruning~\cite{mishra2021accelerating}.

%One of the major downsides of model pruning techniques, regardless of whether it is structured or unstructured, is that it often requires extra training steps to recover the loss in accuracy due to pruning~\cite{mishra2021accelerating}, with structured sparse pattern needs 

%, unless it is trained to be sparse from scratch \cite{zhou2021nm}.

%\subsubsection{Sparsity in activations}
\textbf{Activation Sparsity.}
%\PT{we can talk about activation sparsity in the self-attention block too}
Activation sparsity arises at runtime due to the non-linear activation functions such as ReLU, ReLU6~\cite{mobilenets}, and SquaredReLU~\cite{so2021primer}, which clips negative values to zero. Activation sparsity is prevalent in both conventional Convolutional Neural Networks (CNNs) and recent Transformers~\cite{li:transformer-sparsity}. Since it is intrinsic in DNN models, no extra fine-tuning or pruning steps is required to introduce activation sparsity.
%While the weight sparsity can be determined statically, 
Unlike weight sparsity, activation sparsity is dynamic as the intermediate input activation values depend on the inputs of the DNN model.
Thus, the location of non-zeros and the degree of sparsity are unpredictable, similar to unstructured pruning making it hard for structured sparse hardware to exploit input sparsity.
Another challenge is that recently proposed activation functions, such as GELU~\cite{gelu}, and Swish~\cite{ramachandran2017searching}, do not generate zero, which nullifies the benefits of exploiting activation sparsity in prior work~\cite{jang2021samsung}.


\subsection{DNN HW: Exploiting sparsity in DNNs}
\label{subsec:dnnhw}

%\subsection{Comparison of DNN HWs}
%In ~\autoref{table:nm-hw}, we summarize different DNN HWs (Dense, Unstructured Sparse, and Structured Sparse) and compare them with our work.

%As mentioned before, depending on the sparsity patterns, different sparsities can be categorized into unstructured sparse, structured sparse, and dense.
%In \autoref{fig:research-objective}, we position several sparse tensor accelerator architecture works based on their specialization.
%In \autoref{fig:sparsity_patterns}, we show three patterns, dense, unstructured sparsity, and N:M structured sparsity where N is 2 and M is 4.
%\autoref{table:nm-hw} shows the comparison of various sparse HW support. % for different DNN models.
Unstructured sparse accelerators, including SCNN \cite{parashar2017scnn}, SIGMA \cite{qin2020sigma}, Samsung NPU~\cite{jang2021samsung}, and dual-side sparse core (DSTC)~\cite{wang:dual-side} target unstructured sparsity and skip redundant computations aggressively, but they suffer from non-trivial area/power costs due to the complex indexing and reduction logic, often introducing workload imbalance problems~\cite{liu2022hpca} as well. 
For example, SIGMA \cite{qin2020sigma} introduces 38\% area overhead compared to the dense architecture due to its flexible and non-blocking distribution/reduction networks.
SCNN \cite{parashar2017scnn} and Griffin~\cite{shin2021griffin} produce 34\% and 32\% area overhead due to the support for the unstructured sparse dataflow.
%SIGMA’s key overheads are the highly flexible, non-blocking distribution and reduction networks that lead to a 37.7% area overhead.
%Samsung NPU~\cite{jang2021samsung} instead focuses on exploiting unstructured input sparsity to avoid extra training stages required to enforce weight sparsity in the target model.
Moreover, when the sparsity degree is low or zero, they provide no improvement or even degrade performance/efficiency due to the overhead for supporting unstructured sparsity \cite{highlight2023micro}.
%\input{tables/comparison3}
%Zhu et. al~\cite{zhu2019micro}
More recent structured sparse tensor accelerator architectures, such as STA \cite{liu2020sta}, Sparse Tensor Core from NVIDIA GPUs (NV-STC) \cite{nvidia_ampere}, and VEGETA \cite{jeong:vegeta}, provide HW support for structured sparsity
%\TK{no they only provide HW support for N:M structured sparsity}
with minimal area overhead.
However, these designs accelerate \textbf{only structured pruned models} with the specific pattern and focus on weight sparsity since exploiting unstructured activation sparsity without much overhead is not trivial.
%\PT{We need to have figures to provide example of structured sparsity.}
S2TA~\cite{liu2022hpca} has tried to circumvent the challenge by forcing structured sparse patterns dynamically, but it requires modifying the models and even more fine-tuning steps. %, which is not preferable for real-world deployments.
We compare different DNN HWs in \autoref{table:nm-hw}.
\input{tables/comparison4}

%\TK{given that the N:M HW is the target HW in this work, we are missing a figure explaining how N:M HW works. even logically showing a PE with a mux to pick N elements out of M .. }

%SCNN~\cite{parashar2017scnn} consumes around 30\% more energy for a dense workload.
%~\cite{shin2021griffin}.
%\PT{We need actual data to show unstructured sparsity is bad. "SCNN incur XX\% energy overdense, SIGMA introduce XX\% area over baseline, and blahblah"}
%Finally, dual-side sparse core~\cite{wang:dual-side} introduced an architecture to exploit both input and weight unstructured sparsity.

%\textbf{Our research objective of this project is to extend existing NVIDIA dense and sparse tensor cores so that they can leverage input sparsity to improve performance.}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/TASD-interface.pdf}
        \vspace{-1.5em}
	\caption{TASD Interface.
 }
        \vspace{-1em}
	\label{fig:tasd_inteface}
\end{figure}
\subsection{Tension between sparse DNN SW and HW}
\autoref{fig:tasd_inteface} shows the state of sparse DNN software and hardware. On the one hand, model developers have shown that unstructured sparsity provides better model accuracy and higher sparsity degree. On the other hand, hardware developers have shown that structured sparsity support is more practical to include in GPUs and other DNN accelerators. Such tension in the desired sparsity patterns hampers the progress in bringing sparse DNN acceleration to practice.

The main drawback of the previous hardware-specific patterns is that the pruning software and hardware support are tightly coupled, such that the software generates a model specifically pruned for the pattern supported by the hardware. For example, a model pruned for the NV-STC can only be accelerated by NV-STC, not by S2TA.
To decouple the tight relationship, we propose another layer of system software between the model developers and DNN hardware for sparsity. Our insight is to approximate a tensor by decomposing it into a series of structured sparse tensors. 
We leverage the distributive property in tensor algebra to execute the series of structured sparse GEMM. This mechanism provides an unstructured sparse interface for developers but only requires structured sparse support from hardware. As shown in \autoref{table:nm-hw}, by bridging DNN model and HW, this work is able to accelerate all types of sparsity seamlessly with a low area overhead.



%We illustrate our view in ~\autoref{fig:tasd_inteface}.
%Once we prove that TASD could achieve reasonable accuracy, we would explore HW design space to provide native TASD support.


==> mlsys2025style/sections/3_tasd.tex <==
\section{TASD: Tensor Approximation via Structured Decomposition} 

In this section, we introduce a method to \textbf{approximate unstructured sparsity using a series of structured sparsity}, which we call \textbf{TASD}.
In this paper, we use a set of N:M structured sparsities for TASD to explain the method and show how to use it practically, but the method is general and not limited to only N:M structured sparsity.

\label{sec:tasd}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/tasd-example.pdf}
        \vspace{-1em}
	%\caption{TASD example using a 2$\times$8 matrix $A$ whose sparsity degree is 37.5\%.}
        \caption{TASD example using a 2$\times$8 matrix $A$.}
	\label{fig:tasd_example}
    \vspace{-2em}
\end{figure}

\subsection{Overview}
We use an unstructured sparse matrix $A$ to illustrate how TASD works in \autoref{fig:tasd_example}.
The matrix $A$ has 6 zero elements out of 16 total elements with a 37.5\% sparsity degree. 
Also, note that the sum of all elements in $A$ is 25.

Matrix $A$ can be rewritten as a 2:4 structured sparse matrix (a 2:4 view of $A$) plus a remaining matrix, $A_{1}^{2:4}$ and $R_1$, where $A_{1}^{2:4}$ is derived by extracting two \textbf{largest} elements out of four elements in each row in $A$ while $R_1$ is the remaining matrix (i.e. $A - A_{1}^{2:4}$) after the extraction, as shown in \autoref{ss-decomp}. 
\begin{align}
    A & = A_{1}^{2:4} + R_1 \label{ss-decomp}
\end{align}
The extracted matrix, $A_{1}^{2:4}$ covers 70\% in terms of the number of non-zero values while covering 84\% in terms of the sum of the magnitudes.
The percentage for the lost magnitudes is smaller than the percentage of the lost non-zero values because we extract two \textit{largest} elements out of four consecutive elements.
If we discard the remaining matrix $R_1$, then the original matrix $A$ can be \textit{approximated} as $A_{1}^{2:4}$.
Thus, we call this approximation, \textbf{structured decomposition}.
%and the metrics mentioned above can be used to describe how lossy the approximation is. 
If we approximate $A$ with a 3:4 pattern instead of the 2:4 pattern, we can derive matrix $A_{1}^{3:4}$ with a structured decomposition that drops only one non-zero element, covering 90\% of the number non-zeros and 96\% of the sum of total magnitudes.

Instead of using a denser N:M, we can further decompose $R_1$ using another structured pattern, such as 2:8.
$A_2$ can also be derived by extracting two largest elements out of \textbf{eight} consecutive elements in $R_1$, making $A_2$ as a 2:8 structured sparse matrix.
Similar to the previous decomposition, we call the remaining matrix $R_2$ as shown in \autoref{fig:tasd_example}.
%Instead of extracting two largest elements out of \textbf{four} consecutive elements in the remaining matrix, $B_2$ can also be derived by extracting two largest elements out of \textbf{eight} consecutive elements in the remaining matrix, making $B_2$ as a 2:8 structured sparse matrix. 
%In this case, not all elements of $B$ could be distributed across $B_1$ and $B_2$, so $B$ might not be equal to $B_1 + B_2$, but can be \textbf{approximated} as $B_1 + B_2$ as shown in \autoref{ss-decomp2}.
All elements of $A$ are covered by $A_{1}^{2:4}$ and $A_{2}^{2:8}$, so $A$ is equal to $A_{1}^{2:4} + A_{2}^{2:8}$, thus the approximation of $A$ to $A_{1}^{2:4} + A_{2}^{2:8}$ is lossless.
Since the unstructured sparse matrix is approximated using a set of structured sparse matrices, we call this method as Tensor Approximation via Structured Decomposition (TASD).

Theoretically, structured decomposition can have infinite terms. 
Below, we formalize the process more generally using different structured sparse patterns denoted as $s_i$.
%if one wants to approximate $B$ more precisely, i.e. $B_3$ can also be added by extracting two out of 16 consecutive elements (2:16) in the remaining matrix ($B - B_1 - B_2$) as shown in \autoref{ss-decomp3}, or until any $B_n$. 
\begin{align}
    A & \simeq A_1^{s_1} + A_2^{s_2} \label{ss-decomp2}\\ \label{ss-decomp3}
      & \simeq A_1^{s_1} + A_2^{s_2} + A_3^{s_3} \\ \label{ss-decomp4}
      & \simeq A_1^{s_1} + A_2^{s_2} + A_3^{s_3} ... + A_n^{s_n}
\end{align}
We call $A$ as the original matrix and $\sum A_i^{s_i}$ as \textbf{TASD series}, to draw an analogy to the classic Taylor series%
\footnote{Taylor series approximates any function with polynomials, while TASD series approximates any tensor with structured sparse tensors.}%
: Each successive term (residual structure sparse tensor) improves the accuracy of the approximation.
A TASD series configuration includes the number (``order") of TASD terms ($n$) and the structured sparsity pattern ($s_i$) for each TASD term.
Using TASD, one can generate a structured sparse view of a given tensor, and the error between the view and the original tensor would depend on the TASD series configuration.

\subsection{Using TASD for matrix multiplication}
TASD decomposes any tensor $A$ into a series of structured sparse tensors.
Decomposed tensors can be used in any tensor algebra, such as matrix multiplication ($C = A\times B$), which can be approximated as $A_1^{s_1}\times B$. If $s_1$ is 2:4, and the matrix multiplication is running on NVIDIA Sparse Tensor Cores, potentially 50\% of  Multiply-and-Accumulate (MAC) operations could be skipped.

With the distributive property of tensor algebra, matrix $A$ can be approximated using more TASD terms such as $(A_1^{s_1} + A_2^{s_2})B = A_1^{s_1}B + A_2^{s_2}B$. 
If $s_1$ is 2:4 and $s_2$ is 2:8, about 25\% of MAC operations could be skipped.
Finding the proper TASD series to minimize the error while maximizing compute reduction will determine the quality of the approximation.
We provide a detailed analysis of TASD with synthetic data in \autoref{append:additional_details}.


==> mlsys2025style/sections/4_application.tex <==
\section{HW/SW Co-Design with TASD}
\label{sec:codesgin}
%\input{tables/potential_perf}
%\begin{figure}[!t]
%	\centering
%	\includegraphics[width=0.45\textwidth]{figures/tasd-high-level.pdf}
%	\caption{tasd-high-level. -- maybe table.. train once and get all the benefits}
%	\label{fig:tasd-high-level}
%\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/system-overview-simple-new.pdf}
    \vspace{-0.5em}
	\caption{System overview with TASDER.}
	\label{fig:system_overview}
    \vspace{-0.5em}
\end{figure}

In \autoref{sec:tasd}, we introduce our approximation method, TASD, in general. In this section, we show how our method can be used to accelerate DNN models with sparse weights and inputs.
Although TASD can also be used to accelerate the DNN training, we focus on how to accelerate DNN inference in this work.
There are two main insights that inspired us to use TASD for DNN inference.

1) By its nature, DNN models are able to tolerate small errors in their internal computations. 

2) Although TASD is a lossy approximation method, carefully selected TASD terms can provide high-quality approximations with a limited number of non-zeros being dropped.

%\todo{Discuss and use "TCONV" for the whole section. Make the HW to be a TCONV HW and say any structured sparse HW can be a TCONV HW.}

\subsection{System architecture overview}
We introduce our optimizer system, TASDER, which takes a DNN model, sample data, target HW information including structured sparsity patterns, and hyperparameters as shown in \autoref{fig:system_overview}.
Internally, TASDER will search for the TASD configuration for each layer of the given DNN model and return the configurations.
In the following subsections, we introduce TASD-W and TASD-A, which are the methods to exploit TASD on weights and activations, respectively.
We also explain how the TASD configuration per layer is selected in our framework.
In this work, we only consider convolution (CONV) and fully-connected (FC) layers in DNN models to apply TASD as they usually consume most of the execution cycles, and they get converted to matrix multiplication operations using algorithms such as \texttt{im2col} for parallelization.
%TASD; TASD-W, TASD-I

%Outputs: TASD Group -- 
%SW/HW requirements for TASD
% Clearly state what is the assumption.
% Compiler phase
% profile guided optimized for the HW
% we can cover both dense/structured sparse

\subsection{TASD-W: Applying TASD on weights}
\label{subsec:tasd-w}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50_layer_sparsity.pdf}
        \vspace{-1em}
	\caption{Sparsity degrees for each layer in 95\% unstructured sparse ResNet50 from SparseZoo.}
	\label{fig:resnet50_layer_sparsity}
    \vspace{-1em}
\end{figure}

\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.95\textwidth]{figures/conv-spconv-tconv-wide.pdf}
        \vspace{-0em}
	\caption{Comparison of flows of an original model with a conventional CONV/FC layer and transformed models with a TCONV/TFC layer with structured sparse weights, and a TCONV/TFC/TASD layer with structured sparse activations. 
 %\TK{I was a little confused about how Figure 6 and Figure 8 gel together. Both seem to show TASDER but the outputs of TASDER seem to flow to HW in Fig 6 but seem to be within SW (say PyTorch) in Fig 8 .. this is just a high level glance, i didnt read the text describing it.}
 }
	\label{fig:conv-tconv}
    \vspace{-1em}
\end{figure*}

We expose an unstructured interface to ML model developers as the target of optimization so that they can focus on the techniques to prune their models as much as possible without considering any specific HW-friendly sparsity pattern.
Therefore, the optimization problem for TASD-W is that given the weights of DNN models as unstructured sparse tensors, use the available structured sparse HW to accelerate the model execution as much as possible. 

We assume that the target hardware can accelerate the structured sparsity patterns, $S_1, ..., S_n$.
A TASD configuration of the $i$th layer, $C_i$, is a sequence of $S$.
For a given DNN model $M$, a TASD transformation of the model, $T$, is defined as applying a sequence of $C_i$ where $C_i$ is the TASD configuration for each layer in the model.
%
Then, the target is to find a TASD transformation $T_{opt}$ for a given model where
\vspace{-0.5em}
\begin{align}
& T_{opt} = \argmin_T (Latency(M_T)) \\  %&= \{x \mid c(x) = \min_{x'} f(x')\}
& \text{such that } Accuracy(M_T) \approx {Accuracy}(M_{original}) 
\end{align}

\vspace{-0.5em}
A simple way to use TASD-W is using the same TASD configuration for all layers in  the model, i.e. applying \textbf{network-wise TASD-W}.
As the number of supported structured sparsity patterns, $n$, is not large enough, the $T_{opt}$ for network-wise TASD-W could be found with the exhaustive search.

A better method to use TASD-W is using different TASD configurations for different layers, i.e. \textbf{layer-wise TASD-W}.
The set of TASD transformations that can be covered by layer-wise TASD-W is a super-set of the TASD transformations in network-wise TASD-W. 
Usually, a pruned model with unstructured sparsity does not guarantee the same sparsity across layers, i.e. even though the overall sparsity is 95\% for the model, different layers could have different sparsity degrees as shown in \autoref{fig:resnet50_layer_sparsity}.
%there is a notable variance in sparsity degrees across different layers.
Unlike network-wise TASD-W where all the layers use the same TASD configuration, it is not straightforward how to choose a TASD configuration per layer as there could be numerous options per layer. 
To minimize the accuracy drop, it is crucial to reduce the number of dropped non-zeros after applying TASD, which would prefer conservative TASD configurations. 
On the other hand, to maximize the performance gain, it would be better to apply aggressive TASD configurations, which would be able to be translated into higher sparsity and efficiency gain. 

To address this, we design and implement a greedy-based algorithm that optimizes across all layers.
This greedy algorithm first measures the percentage of dropped non-zero elements of each TASD configuration for all layers and sorts the configuration-layer pairs by their percentage of dropped elements.
Next, it greedily applies the TASD configuration based on the sorted order until the model quality is $<$99\% of the original model (i.e., prioritize the option with the smallest dropped non-zeros). 
Since it only takes a single pass to all layers, the runtime overhead is trivial (a few seconds per model), while the extra training needed for structured sparse HW often takes hundreds of GPU hours~\cite{sun2021domino}.

We use TCONV/TFC to indicate a CONV/FC layer with TASD as shown in \autoref{fig:conv-tconv}, and the TASD configurations found above would be applied to the corresponding TCONV/TFC layers.
In \autoref{fig:conv-tconv} (a), we show how the conventional CONV/FC layer works with unstructured sparse activations (usually from ReLU) with dense weights. In \autoref{fig:conv-tconv} (b) shows how a TCONV/TFC layer works with unstructured sparse weight. 
TASDER would modify unstructured sparse weights to structured sparse weights with TASD-W.



\subsection{TASD-A: Applying TASD on activations}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/tasd-i-updated-2.pdf}
 \vspace{-1.5em}
	\caption{
 ResBlocks with CONV and TASD/TCONV and Transformer Blocks with FC and TASD/FC.}
 
	\label{fig:tasd-a}
 \vspace{-1.5em}
\end{figure}
TASD can also be applied to activations to improve a DNN execution as shown in \autoref{fig:conv-tconv} (c).
Unlike weights which are static, TASD should be applied for dynamic decomposition during the runtime as activations are dynamic. 
In \autoref{fig:tasd-a} (a) and (b), we show a baseline ResBlock and a ResBlock with TCONV and TASD layers, which decompose activation tensors with given TASD configurations. 
We add TASD layers after ReLU layers so that they can minimize the number of dropped non-zeros after approximation. 
The same can be applied to a Transformer Block, where the FC layers in the multi-layer perception module can be replaced with TFC by inserting a TASD layer before TFC layers as shown in \autoref{fig:tasd-a} (c) and (d).
Ideally, other FC layers in a Transformer Block could also be replaced with TASD and TFC layers, but empirically we found it hard to maintain the model quality.

Similar to TASD-W, the simplest way to choose a TASD configuration for each TASD layer is using network-wise TASD where all TASD configurations are same across all TASD layers. 
Assuming limited supported structured sparsity patterns from HW, only a handful number of options need to be explored.
However, similar to weights, this may not be efficient as activations from different layers show significantly different degrees of sparsity, as shown in \autoref{fig:resnet50_layer_sparsity}.

To address this issue, we again leverage layer-wise TASD as it can tailor the TASD configuration to each layer.
However, 
unlike the TASD-W,
it is not feasible to test every option for each layer to find out the best options as the target tensors (activations) are dynamically generated.
%, unlike the case of TASD-W (static weights). 
%due to the combinatorial explosion.
%To choose a TASD configuration for each layer, we use a sparsity-based TASD selection method instead of the non-zero-based method for TASD-W.
%that we introduced in \autoref{subsec:tasd-w}.
We find that a small set of calibration dataset (e.g., 1000 images for ImageNet~\cite{deng2009imagenet}) can provide enough insights. 
As shown in \autoref{fig:resnet50_layer_sparsity}, while different layers have different sparsity degrees, for a particular layer, the activation sparsity degree remains in a small range across different input images.
Therefore, TASDER takes calibration data as an input, so it can profile the given DNN model with the calibration data and collect the statistics (e.g., average, 99th percentile) about activation sparsity per layer. 

To choose a TASD-A configuration for each layer, we use a \emph{sparsity-based} selection method, instead of the dropped-non-zero-based method for TASD-W.
We use a hyperparameter, $\alpha$, to tune the aggressiveness of the TASD approximation. 
For a given layer $L_i$ and the available configurations in the target HW (e.g., $H_1, ... , H_4$), we choose $C_i$ as $H_j$ where $j$ is the largest integer where $S(L_i) + \alpha > H_j$.
If we use a larger $\alpha$, we choose the TASD configuration more aggressively (i.e. allowing more dropped non-zeros). 

%We summarize the algorithm in \autoref{lst:tasd}.
%\vspace{-1em}
%\input{algorithms/find_config}



\textbf{Beyond sparsity: Supporting non-ReLU-based DNNs.}
%ReLU-based DNNs naturally induce sparsity in activation tensors, so by collecting the sparsity statistics, TASD-A can find the appropriate configuration for each layer. 
%However, 
For better accuracy, state-of-the-art DNNs have replaced ReLU with other activation functions, such as GeLU \cite{gelu} and Swish~\cite{ramachandran2017searching}, which do not induce any sparsity in activations making the activations dense.
Thus, our sparsity-degree-based TASD selection to choose TASD configuration for TASD-A for each layer would not work for those DNNs.

\begin{table}[t]
\small
\caption{Supported sparse patterns with TTC-VEGETA.}
%\vspace{-1em}
\begin{center}
\begin{tabular}{cc|cc}
{\bf Pattern} & {\bf TASD series} & {\bf Pattern} & {\bf TASD series}\\
\hline
1:8 & 1:8 & 5:8 & 4:8 + 1:8\\
2:8 & 2:8 & 6:8 & 4:8 + 2:8\\
3:8 & 2:8 + 1:8 & 7:8 & - \\
4:8 & 4:8  & 8:8 & Dense\\

\end{tabular}
\label{tab-ttc-vegeta}
\end{center}
\vspace{-1em}
\end{table}

%(\autoref{lst:tasd})
To address this, we investigate the distribution of the magnitude of all elements in the activation tensors from GeLU/Swish-based DNN.
%as shown in \autoref{fig:tasd-pseudo-density}. 
We found that, while no element in the tensor is exactly zero, a huge number of elements have tiny magnitude, compared to the range of magnitude for all elements. Therefore, we let TASD-A leverage this skewed distribution and collect the magnitude statistics. We introduce another heuristic, \emph{pseudo-density}, which aims to preserve a fixed percentage (e.g., 99\%) of the sum of all elements in a tensor, to determine the best TASD configuration for every layer.
Using the pseudo-density for the non-ReLU-based DNNs, we can use the same sparsity-degree-based method 
%(\autoref{lst:tasd}) 
%that we proposed in \autoref{subsec:tasd-w} 
(i.e. by replacing \textit{sparsity} to \textit{1 - pseudo-density}). The approximating nature of TASD allows the system to also accelerate non-ReLU-based DNNs, while prior work that specifically targets activation sparsity cannot.

% TODO; Challenge of sparse activation
% random dropping / magnitude dropping ...
% magnitude based selection
% pseudo-sparsity
% define approximated sparsity
% Sparse BERT; sparse - dense act
% Dense BERT; dense - dense act

% ResNet50 sparseloop
% TASD-W for BERT-Base/ accuracy
% BERT-Base sparse using sparseloop
% BERT-Base dense using sparseloop
% qkv projection FF1 FF2

%In this section, we introduce how to use TASD to exploit input sparsity in DNNs. 
%The key intuitions are that 1) Input activations in each layer of a DNN already have many zeros 2) TASD configurations  3) Dropping a small number of non-zeros by approximation could be tolerable in terms of the accuracy of a DNN model. 
%Thus, we apply TASD on input activations in each layer of the target DNN.
%One can apply extreme [1:8] to the input activations of all layers, which could be able to achieve 8$\times$ reduction in terms of the number of required MAC operations, but this would lose many non-zero values, thus incurring significant accuracy drop. 
%A good TASD configuration should be able to decompose $B$ using a small number of sparse $B_i$ without losing a high number of zeros.
%If we apply good TASD configurations to all layers, we should be able to achieve reduced computation while maintaining the original accuracy.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-hw-overview-simple-new.pdf}
  \vspace{-1em}
	\caption{TASD-HW composed of four TTCs. 
 %\TK{I presume RF MAC etc is basically plug and play for different N:M accelerators (STC/VEGETA etc) .. might be good to just show a box called "N:M Accelerator" or sthg and expan it out to show the RF/MAC etc}
 }
	\label{fig:tasd-hw}
 \vspace{-1em}
\end{figure}
\subsection{Structured sparse HW for TASD}
TASD works best when there are at least a few supported structured sparse patterns in the target sparse accelerator. While the TASDER optimizer is HW-agnostic, we propose to build on top of a recently proposed flexible structured sparse tensor accelerator to maximize the benefit.
Inspired by previous structured sparse accelerators~\cite{nvidia_ampere,liu2021s2ta,jeong:vegeta}, we introduce TASD Tensor Core (TTC).
We adopt a design similar to VEGETA~\cite{jeong:vegeta} engine composed of multiple processing elements (PEs) while providing support for 1:8, 2:8, and 4:8 structured sparse patterns, and we call it TTC-VEGETA.
With TASD and a limit of up to 2 terms, a TTC-VEGETA engine can support 7
out of all the N:8 patterns 
%\footnote{The 7:8 pattern needs 3 TASD terms and is rarely used in practice.}%
as shown in \autoref{tab-ttc-vegeta} even though the original VEGETA supports only three sparse patterns.
Note that TTC can adopt other structured sparse designs, such as STC~\cite{zhu2019micro} with supports for 2:4 and dense, which we call TTC-STC. 
This would limit the flexibility in approximation using TASD compared to VEGETA-based TTC design, but TASDER is still able to optimize some layers. 
We explore the benefit of flexibility in \autoref{sec:eval}.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-flow.pdf}
    \vspace{-1em}
	\caption{Dataflow between PE array and TASD units.}
	\label{fig:tasd-flow}
    \vspace{-2em}
\end{figure}


In \autoref{fig:tasd-hw}, we show the overall design of a TASD HW composed of four TTCs similar to the one used in the previous work \cite{wu2022sparseloop}.
%\todo{walk throught the design}
The modification we add on top of the N:M accelerator, such as STC or VEGETA, is the TASD unit (shown in the right part of \autoref{fig:tasd-hw}) that dynamically extracts TASD terms from the activation tensor, similar to the DAP unit in S2TA~\cite{liu2022hpca}.
TASD-W can be applied offline through pre-processing since weights do not change during runtime, but TASD-A requires the TASD unit as activations will be dynamically generated at runtime.

Given the computation latency on TTCs, the minimum number of TASD units per TTC to hide the latency of TASD units depends on the mapping and TTC implementations.
%that we describe in the following. 
For example, each TTC-VEGETA with M=8 generates 16 (number of PE columns in each TTC) output elements per cycle (i.e. 2 blocks per cycle) as shown in \autoref{fig:tasd-flow}, which will be fed to TASD units. 
For an M-element block, a TASD unit sequentially extracts the largest values, so the decomposition takes up to M cycles %for any TASD configuration 
as the sum of Ns in a TASD configuration cannot be larger than M.


The example in \autoref{fig:tasd-flow} uses TASD configuration composed of 4:8 and 1:8, so it takes 5 cycles per block. 
At T1 (cycle 1), two blocks (Blk-1, Blk-2) will be produced from the PE array, and Blk-1 and Blk-2 will be processed by TASD Unit 1 and TASD Unit 2, respectively (each cycle, two TASD units start execution). 
During T2-T5, Blk-1 and Blk-2 will be used to extract Decomposed Blocks, DBlk-1 and DBlk-2 for 4:8 Tiles.
Then, during T6, DBlk-1 and DBlk-2 for 1:8 Tiles will be generated and stored. The decomposed blocks will be used as the inputs of the next layer.
With 16 TASD units, a TTC-VEGETA can operate without stalls on the PE array due to the decomposition as a TASD unit is always guaranteed to be available after M cycles (i.e. by Little's law, $16 = 2\times8$). 
%TODO ADD a sentence that DB will be used.
We present the area overhead for TASD units in \autoref{sec:eval}.
%How this is used to split a tensor into two? I can imagine that you sequentially output the largest values, and cut off the first 4 (out of 8) for a 4:8 term, and then the next 2 for a 2:8 term, etc. Such sequential execution seems to have very low throughput. How many such TASD units are needed then? What is the ratio between number of MAC units and number of TASD units to achieve a balanced throughput? The evaluation only mentions a 2% area overhead in 5.5 without any details.

%From our synthesis result, the area of a PE-M8 and TASD-M8 is 241um^2 and 88um^2 each. Considering the PE to TASD ratio (256:16), the area overhead of TASD on top of PEs is 88*16/241*256 = 2.3\%. To understand the impact of different M in terms of overhead, we also synthesized for different Ms (4 and 16), and observed 1.3\% and 3.4\% area overhead, respectively.


% I may need to fix the following
% The current arch file assumes
% LRF/PE holds A
% RF only holds C
% SMEM holds B
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-hw-mapping-simple.pdf}
 \vspace{-1em}
	\caption{A mapping of matrix multiplication on TTCs.
 }
    \vspace{-1em}
	\label{fig:tasd-mapping}
\end{figure}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/sparseloop_results.pdf}
    \vspace{-0.5em}
    \caption{
    Energy-delay-products for running dense and sparse ResNet50 and BERT. For TTC-STC and TTC-VEGETA, we use the TASD transformations found from TASDER.
    %and DNN layers assuming the VEGETA engines frequency as 0.5GHz.
    M4/M8 represents design with N:4/N:8 supports.
    }
    \vspace{0.5em}
    \label{fig:dense_sparse_comparison}
\end{figure*}
\textbf{Decomposition-aware dataflow.}
In \autoref{fig:tasd-mapping}, we show a mapping of a matrix multiplication with an approximated matrix A using a TASD configuration, 4:8 and 1:8 for the TTC.
We first show how we tile the matrices and how they are mapped in the private register file and shared buffer of each TTC.
When matrix $A$ is decomposed into two TASD terms, $A_1$, and $A_2$, the original matrix multiplication can be approximated as the sum of the two matrix multiplications and accumulation ($A_1\times B + A_2\times B$). 
As the two matrix operations share the same input $B$ and partial sum $C$, we \textbf{keep B tiles in the L2 Scratchpad Memory (SMEM) and C tiles stationary in the L1 SMEM} of TTC while changing decomposed A tiles to temporally reuse B and C tiles for data reuse (between timestep 1 and 2, timestep 3 and 4 in ~\autoref{fig:tasd-mapping} (b)).
For each accelerator tile, (i.e. for each timestep), we \textbf{keep each element of A tile stationary in the register file of each PE} for the temporal reuse, while the B and C elements are mapped correspondingly. 
By increasing the tile size for GEMM-N dimension, the reuse count for A tile at PE level could increase, which is limited by the size of the capacity of each SMEM.
We swap C tiles at the very end to minimize the number of write-back operations to other levels.
Although we maximize reuses for decomposed tiles, there is still unavoidable overhead such as reading C tiles again, but this is insignificant compared to the energy saving by skipping ineffectual computations using TASD.
In \autoref{subsec:energy_breakdown}, we quantify the energy overhead.

%Using the proposed accelerator, we show a mapping .

%Intuitively, it would be better to use a greedy approach which would allow $B_j$ be more important than $B_k$ if $j < k$.

% theoritical numbers for running 8:8 using 1:8
%  4 8 16?
% 1 : 16

% 2:4
% 2:4, 2:8
% 2:4, 2:8, 1:8

% 2:4
% 2:4, 2:8 --> 4:8, 2:8 == 6:8
% 2:4, 2:8, 1:8 --> 4:8, 2:8, 1:8
% 2^n : 2^m with fixed m
% use TASD


==> mlsys2025style/sections/5_eval.tex <==





\section{Evaluation}
\label{sec:eval}
\subsection{Methodology}



TASD accelerates both sparse and dense DNNs \textit{without fine-tuning}, so we evaluate TASD-W on sparse DNNs from SparseZoo~\cite{SparseZoo} and TASD-A on dense DNNs from TorchVision~\cite{torchvision}.
We use a classic convolutional network, ResNet50~\cite{he2016resnet}, and a transformer-based network, BERT~\cite{devlin-etal-2019-bert}.  %to illustrate detailed trade-offs between accuracy and performance.
For the baseline HW, we compare against dense tensor core (TC)~\cite{nvidia_ampere} and dual-side sparse tensor core (DSTC)~\cite{wang:dual-side} as representative dense and unstructured sparse accelerators.
We configure these baselines as in the Sparseloop Artifacts~\cite{sparseloop-artifact}.
We use 4 variants of TTC, based on STC and VEGETA with N:4 and N:8 designs, to show the extra benefits of TASD from the flexibility of the structured sparse hardware as summarized in \autoref{tab:hw}.
%(TTC-STC-M4, TTC-STC-M8, TTC-VEGETA-M4, TTC-VEGETA-M8).
All designs use the same memory hierarchy and the same amount of PEs (MACs) to ensure a fair comparison.
We clarify that we do not exploit both sparsities concurrently for skipping computations. We either use TASD-W or TASD-A depending on the workloads since supporting both sparsities requires non-trivial area/energy costs~\cite{wu2021sparseloop, highlight2023micro} and is not compatible to approximate with TASD.

%We use one of the most popular DNN, ResNet50 (both dense and pruned with 95\% unstructured sparsity) 


%To evaluate the effectiveness of TASD methods on accelerators, 
We develop TASDER as a framework to search for TASD transformations and calculate the accuracy of the model with each TASD transformation using PyTorch~\cite{paszke2019pytorch}. 
Following the requirement in MLPerf~\cite{mlperf} inference benchmark, we only consider a model as valid with TASD \textit{if the model achieves an accuracy higher than 99\% of the accuracy of the original model.}
%For TASD-A, we randomly pick 0.1\% of the data for calibration.
Next, we run each DNN layer with the given TASD series configuration using Sparseloop~\cite{wu2022sparseloop}, a sparse accelerator modeling framework to obtain per-layer results and aggregate the results for the entire network, which is consistent with prior accelerator simulation frameworks~\cite{timeloop, cosa, maestro, zigzag, scale-sim}. Sparseloop estimates the performance and energy consumption of the given HW by analyzing data movements across different memory hierarchy levels and processing elements, and actual computation based on the given dataflow. 
\textbf{We simulate all layers in the networks (marked as ``Overall")}, but to show per-layer results additionally, we choose three representative layers (from early, mid, late) as shown in \autoref{tab:workload}.
%In \autoref{tab:hw} and \autoref{tab:workload}, we show specific HW designs and target workload configurations used in \autoref{sec:eval}.

%%%% Tables
\begin{small}
\begin{table}[t]

%\small
\begin{center}
\small

\caption{Summary of different HW designs. TASD 1T and 2T indicates using TASD 1 term and 2 terms, respectively.
}
\vspace{1em}
\begin{tabular}{c|c}
{\bf HW Design} & {\bf Sparsity Support from HW} \\
\hline
\hline
TC  & None  \\
\hline
DSTC & Unstructured \\
\hline
%\cline{1-3}
TTC-STC-M4 & 2:4 (TASD 1T) \\               
\hline
TTC-STC-M8 & 4:8 (TASD 1T) \\
\hline
TTC-VEGETA-M4 & 
\begin{tabular}[c]{@{}c@{}}1:4, 2:4 (TASD 1T) \\ + 3:4 (TASD 2T)\end{tabular} 
  \\
\hline
TTC-VEGETA-M8 
&\begin{tabular}[c]{@{}c@{}}1:8, 2:8, 4:8 (TASD 1T) \\ + 3:8, 5:8, 6:8 (TASD 2T)\end{tabular}  

\end{tabular}

\label{tab:hw}
\end{center}
\end{table}
\end{small}


\begin{small}
\begin{table}[t]
%\small
\begin{center}
\footnotesize

\caption{Representative layers from the target workloads. L1, L2, and L3 are representative layers. RN and Act. refer to ResNet and Activation, respectively.
%We use ``Overall" for the entire network. 
%Sp: Sparse, D: Dense. Wgt: Weights. Act: Activations. %\TK{I initially thought L1, L2 and L3 are layers 1, 2 and 3 .. but seems like they are some other representative ones. Why not explicitly mention which layer it is? Eg L4, L31, L40 ..}
}
\begin{tabular}{c|c|c|c}
{\bf Model} &{\bf Weight}& {\bf Act.} & {\bf Layers Dimensions}\\
\hline
\hline   

\begin{tabular}[c]{@{}c@{}}Dense RN50 \\ (ReLU-based)\end{tabular}     &Dense& Sparse & 
\begin{tabular}[c]{@{}c@{}}L1: M784-N128-K1152 \\ L2: M3136-N64-K576\end{tabular}
\\
\cline{1-3}
Sparse RN50 &Sparse& Sparse & L3: M196-K2304-N256 \\
    
\hline
\begin{tabular}[c]{@{}c@{}}Dense BERT \\ (GeLU-based)\end{tabular}     &Dense& Dense & 
\begin{tabular}[c]{@{}c@{}}L1: M768-N128-K768 \\ L2: M3072-N128-K768\end{tabular}
\\
\cline{1-3}
Sparse BERT &Sparse& Dense & L3: M768-N128-K3072 \\




\end{tabular}

\label{tab:workload}
\end{center}
\end{table}
\end{small}
%\section{Experiments Settings}

We use energy-delay product (EDP), latency, and energy for the metrics. We also provide additional experiment results on the theoretical MACs reductions for other various DNNs, comparison against structured sparse accelerators, and TASD on a real system.
%in \autoref{append:additional_experiments}.

%To show the applicability of TASD for other sparse and dense DNNs, we evaluate the MACs reductions for 8 DNNs, similar to prior work in pruning for structured sparse patterns~\cite{chmiel2022optimal,sun2021domino}.


%First, we show the impact of applying different TASD configurations, both network-wise and layer-wise, on the DNN accuracy.
%Fine-tuning can be used for the target TASD configurations to regain lost accuracy, but we have not assumed that as it will add extra training costs.

%show preliminary results of a few experiments to estimate the potential of TASD to leverage input sparsity in DNN inferences.


\subsection{DNN acceleration with TASD}


\autoref{fig:dense_sparse_comparison} shows the EDP for the 4 workloads on various DNN accelerators, normalized to the dense TC.
Even though DSTC is able to exploit unstructured sparsity, the overhead of unstructured sparse acceleration (such as accessing accumulation buffer frequently) offsets the benefit and even outweighs the benefits when the workload has only one sparse operand or there is no sparse operand, causing 12\% and 167\% \textbf{larger} EDP for dense ResNet50 and dense BERT while reducing EDP by 55\% for sparse BERT.
DSTC works best for sparse ResNet50 and improves EDP by 87\%, as both weight and activation tensors are unstructured sparse with a high sparsity degree (95\% sparse weight).
%with expensive gather-scatter operations. 
Overall, it is able to reduce EDP by 35\% across all workloads on average.
%\footnote{For the conservative evaluation, we assume 2$\times$ L1 SMEM bandwidth for DSTC compared to TTC.}
%TTC only required 4$\times$. 
%while costing 30-40\% area overhead as discussed in \autoref{subsec:dnnhw}
%}.

%DSTC works best for sparse ResNet50 and improves EDP by 87\%, as both weight and activation tensors are unstructured sparse with a high sparsity degree (95\% sparse weight) only if L1 SMEM bandwidth is large enough (). 
%Moreover, 
%(55\% for sparse BERT)

Unlike DSTC, TASD-based TTC accelerators improve EDP over the TC baseline for all workloads. 
With the flexibility in sparsity patterns, TTC-VEGETA-M8 improves EDP for all workloads, by 58\%/61\% for dense ResNet50/BERT and 83\%/82\% for sparse ResNet50/BERT. 
Even with a single fixed pattern, TTC-STC-M4 improves by 4\%/32\% for dense ResNet50/BERT and 49\%/53\% for sparse ResNet50/BERT. 
This result shows that TASD can effectively leverage structured sparse hardware for off-the-shelf dense and sparse DNNs with no fine-tuning, and the extra flexibility (increasing M) in the baseline accelerator increases the benefit.



\autoref{fig:overall_energy_latency_edp} provides end-to-end latency and energy consumption for various designs. TTC-VEGETA-M8 is the most energy-efficient across all workloads and is slightly slower than DSTC only for sparse ResNet50. % (by 22\%). 
This result shows TASD provides a better overall tradeoff than unstructured sparse accelerators, considering their high area overheads.










 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/overall_energy_latency_edp.pdf}
        \vspace{-3em}
	\caption{
        Latency and energy for various designs.
 }
        %\vspace{-0.5em}
	\label{fig:overall_energy_latency_edp}
 \end{figure}

  \begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/resnet50-95-networkwise-w.pdf}
 	\includegraphics[width=0.49\textwidth]{figures/resnet50-95-networkwise-a.pdf}
        \vspace{-1em}
	\caption{
Network-wise and Layer-wise TASD on ResNet50. Upper: TASD-W. Lower: TASD-A.
 }
        \vspace{-1em}
	\label{fig:resnet50-95-networkwise-w}
\end{figure}
%\subsection{Analysis of TASD-W on sparse DNNs} 
\subsection{Analysis of TASD} 
%\vspace{-1mm}
%To understand the impact of TASD on accuracies of DNN models, we implement TASDER using PyTorch~\cite{paszke2019pytorch} and conducted experiments for both TASD-W and TASD-A.
%\subsubsection{Network-wise vs. layer-wise TASD}
\paragraph{Network-wise vs. layer-wise TASD.}
The upper plot of \autoref{fig:resnet50-95-networkwise-w} shows the impact of network-wise TASD-W on the top-1 accuracy of unstructured sparse ResNet50 (95\% sparsity).
We applied network-wise TASD-W with N:4, N:8, and N:16 structured sparsities. 
For example, the network-wise TASD-W with 2:4 uses one TASD term with the 2:4 pattern to the weights of all convolution and fully-connected layers in the sparse ResNet50. 
Since TASD is a lossy method, aggressive TASD series approximation can result in a notable accuracy drop.
Among different N:4, N:8, N:16 options, we found that 3:4, 5:8, 10:16 is the most aggressive approximation among the available options while meeting the 99\% accuracy requirement. 
Especially, using network-wise TASD-W 5:8 (4:8 + 1:8 for TTC-VEGETA) and gating the compute units for sparse activations, compared to the dense baseline, we observe it achieves 24\% and 53\% reduction in cycle and energy respectively, thus reducing 75\% EDP for Sparse ResNet50. 

%networkwise 5:8
%energy,,,0.472,,,,,,
%cycles,,,0.7579,,,,,,
%edp,,,0.2493,,,,,,

%layerwise G 0.35
%energy,,,0.4136,,,,,,
%cycles,,,0.5891,,,,,,
%edp,,,0.2053,,,,,,

%\subsubsection{Layer-wise TASD-W on sparse ResNet50}

Using different TASD series configurations for different layers is more effective as it can adjust the aggressiveness for each layer. 
To choose a TASD configuration per layer, we use the sparsity-based selection method that we introduce in \autoref{sec:codesgin}. %\autoref{subsec:tasd-w}. 
By changing the hyperparameter, alpha, we are able to adjust the aggressiveness of our approximation method.
%We show how the top-1 accuracy and the dropped number of non-zero percentage changes with varying alphas in \autoref{fig:resnet50-95-layerwise-w}.
As layer-wise TASD-W can be adaptive to each layer, the overall approximation can be applied more aggressively.
As a result, compared to the dense baseline, we observe 47\% and 61\% reduction in energy and cycle, respectively, thus reducing 83\% EDP for Sparse ResNet50 as shown in \autoref{fig:dense_sparse_comparison}.


%\subsection{Analysis of TASD-A on dense DNNs} 
%{'cycles': {'TASD-L':0.77 3690167}, 'energy_pJ': {'TASD-L':0.70 6021474651.840003}, 'edp': {'TASD-L':0.42 389056984145620.25}, 'utilization': {'TASD-L': 82.015625}}
%TC-RF2x-24-bandwidth 1.0 4777536
%energy_pJ TC-RF2x-24-bandwidth 1.0 8593036953.436165
%edp TC-RF2x-24-bandwidth 1.0 917293317143056.9
%\subsubsection{Network-wise TASD-A on dense ResNet50}
In the lower plot of \autoref{fig:resnet50-95-networkwise-w}, we show the top-1 accuracy when network-wise and layer-wise TASD-A is applied with different TASD series.
Similar to TASD-W, layer-wise TASD-A is more effective than network-wise TASD-A.
However, the accuracy loss due to approximation shows up with a much smaller approximated sparsity.
As shown earlier in ~\autoref{fig:resnet50_layer_sparsity}, the sparsity degree is larger in weights compared to that in activations for sparse ResNet50.
Thus, the same TASD series drops a larger portion of non-zeros in TASD-A than TASD-W, incurring a higher loss of accuracy.

%\subsubsection{Layer-wise TASD-A on dense ResNet50}

%\autoref{fig:resnet50-95-networkwise-a} shows a similar trend compared to the result of the layer-wise TASD-W on sparse ResNet50.
%With the same approximated sparsity, TASD-A gives lower accuracy while being more tolerant in terms of dropping non-zeros. 
%It is because the sparse weight in ResNet50 is a result of aggresive pruning, so each remaining element is more valuable than the dense model.
%Using the most sparse configuration which meets the requirement, we observe 30\% and 23\% reduction in energy and cycle respectively, thus reducing 58\% EDP, compared to the dense baseline.
%Compared to the dense baseline, we observe 30\% and 23\% reduction in energy and cycle respectively, thus reducing 58\% EDP. 
%\subsubsection{Impact of TASD on more DNN models} 




 



\subsection{
Energy and area overhead due to TASD
}
\label{subsec:energy_breakdown}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth,]{mlsys2025style/figures/energy_breakdown_update.png}
        \vspace{-1.5em}
	\caption{
        Energy Breakdown: TTC vs. Dense TC.}
        \vspace{-0.5em}
        
	\label{fig:energy_breakdown}
 \end{figure}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/sparse-resnet34-rtx3080-tasd-w.pdf}
	        \vspace{-0.5em}
    \caption{
        TASD-W on NVIDIA RTX3080 GPU with Sparse ResNet34.}
        \vspace{-0.5em}
	\label{fig:gpueval}
 \end{figure}
 
\autoref{fig:energy_breakdown} shows the energy breakdown for a representative layer from sparse ResNet50 for dense TC and TTC-VEGETA with a TASD configuration of 4:8+1:8. TTC-VEGETA exploits sparsity and saves energy at all levels of the architecture, which saves 55\% energy over the dense TC. Moreover, the decomposition-aware dataflow in \autoref{sec:codesgin} minimizes decomposition overheads by accessing the RF (with C reuse) and SMEM (with B reuse) instead of accessing DRAM.
%\subsection{Area overhead of the TASD unit}

We measured the area overhead to support TASD on top of the existing structured sparse HW (the TASD units) through RTL prototyping and synthesis with Nangate 15nm Technology Library. We observe up to 2\% of the area for all PEs as TASD units are composed of simple comparator trees.


\subsection{Using TASD on a real system}
To validate the effectiveness of TASD, we evaluate TASD on a real system.
%we apply TASD-W to the unstructured sparse ResNet34 model from SparseZoo \cite{SparseZoo} and run it with NVIDIA TensorRT 8.5.0 on an NVIDIA RTX3080 GPU.
First, we use our framework, TASDER, to find the TASD-W configuration that meets the accuracy constraint with an unstructured sparse ResNet34 model from SparseZoo \cite{SparseZoo}. For the accuracy evaluation, we use ImageNet as the dataset. Next, we export the model using ONNX format. 
To properly measure the inference latency of DNNs exported with ONNX format, we use TensorRT, the state-of-the-art deep learning inference runtime maintained by NVIDIA. We build TensorRT engines for both the baseline model and the model with TASD-W exported in the previous step. Finally, we execute the engine with (3, 224, 224) inputs, with a batch size of 32-128, and measure the latency for each model. We achieved 28\%/39\% speed-up compared to the dense model execution with 0.9\%/1.5\% accuracy drop as shown in \autoref{fig:gpueval}. We also evaluated TASD-W with ResNet50, ResNet101, BERT, and observed up to 25\% speed-up.

%by applying TASD with \textbf{the same TASD configuration} on the input tensors of all convolution layers except the first convolution layer in the pretrained models (AlexNet~\cite{krizhevsky2012alexnet} and ResNet18~\cite{he2016resnet}) during inference. 

%We enforced the structured sparsity to the channel dimension of the tensors.
%We used 1,000 images from the ImageNet~\cite{deng2009imagenet} validation dataset.
%\input{tables/alexnet_results.tex}
%\input{tables/resnet_results.tex}

%In \autoref{table:alexnet_results} and \autoref{table:resnet_results}, we show the Top 1/Top 5 accuracies, a percentage of the number of pruned (dropped) non-zeros, and potential speedup for each TASD configurations and the base pre-trained model. 
%Potential speedup is calculated based on the total effectual computations of convolution layers compared to the base case (dense).
%These preliminary results show that using some TASD configurations could achieve comparable accuracies to the base model, which is encouraging for this direction.
%Still, there are a few things to consider carefully to validate the idea of TASD.
%Since we applied TASD right after ReLU layers instead of right before convolution layers, the numbers would be different when we apply TASD right before convolution layers.
%First, the overhead of applying TASD is not estimated yet, which could harm the overall potential speedup.
%Also, how to support and schedule multiple TASD configurations in tensor cores has not been explained.
%Next, deeper and larger recent DNN models using different activation functions could behave differently.
%Finally, different layers can prefer different TASD configurations and a layer-dependent decomposition scheme might achieve a better trade-off between accuracy and speedup.
%since different layers exhibit different input activation sparsities.




==> mlsys2025style/sections/6_related_work.tex <==
\section{Related Work}
\subsection{SW techniques for structured sparse HW}
%Since the structured sparse (2:4) accelerator is available in off-the-shelf NVIDIA GPUs with Ampere~\cite{nvidia_ampere} and Hopper~\cite{nvidia_hopper} architecture,
%ample work has focused on exploiting structured sparse acceleration for DNNs.

\textbf{Solutions with fine-tuning.}
DominoSearch \cite{sun2021domino} proposed a method to find layer-wise N:M sparsity during training. 
Optimal N:M~\cite{chmiel2022optimal} enforces the structured pattern during training and applies the structured pattern to input activations.
This line of work is orthogonal to our work as we focus on approximating unstructured sparsity without fine-tuning.
%We can also fine-tune DNNs with TASD series configurations and adopt the above approaches.
Fine-tuning will increase the benefit of TASD, as more aggressive approximation can now maintain the same model accuracy. 
Doping~\cite{thakker2021doping} uses an extremely sparse matrix in addition to a compressed matrix derived from Kronecker products to improve the quality of the model, but unlike TASD, it uses the extra extremely sparse matrix to give additional freedom during the training.
%, not for the approximating the given sparse matrix.

\textbf{Solutions without fine-tuning.}
SparseTIR~\cite{ye2023sparsetir} introduces composable formats and transformations for sparse compilation of DL workloads.
%, which also exploits the distributive property to effectively decompose any sparse tensor algebra into multiple well-optimized sparse GPU kernels.
However, they have not considered approximating sparse tensors and accelerating DNNs using structured sparse hardware. Another work~\cite{pool2021channel} shows permuting channels in the weight tensors can recover accuracy easily when training N:M sparse networks. 
%The work also briefly explored turning unstructured sparse models into 2:4 structured sparse models with channel permutations.
TASD is compatible with channel permutation, and we believe combining these two orthogonal techniques will further improve the accuracy of decomposed models with approximation.

\subsection{HW support for sparse DNNs}
%Meanwhile, extensive work has focused on exploiting sparsity in DNNs through specialized HW acceleration.

\textbf{Sparsity support for DNN inference.}
Different architectures have been proposed to support for weight sparsity~\cite{eyerissv2, nvidia_ampere, rasa, eureka2023micro},
for activation sparsity~\cite{jang2021samsung},
and more recently, for both~\cite{wang:dual-side, rmstc2023micro, highlight2023micro}.
%As mentioned earlier, these accelerators can be broadly classified as structured sparse or unstructured sparse HW. 
As mentioned earlier, unstructured sparse HW provides native support for any sparsity pattern but is more costly to build; structured sparse HW is efficient but requires model fine-tuning.
TASD bridges the gap by providing an unstructured sparse interface while only requiring structured sparse HW.

\textbf{Sparsity support for DNN training.}
Since weight tensors are mostly dense during training, prior work has focused on activation and gradient sparsity during DNN training.
A simpler support is to compress sparse activation and gradient, such as CompressDMA~\cite{rhu2018cdma} and ZComp~\cite{akin2019zcomp}. These techniques save data movements and memory requirements, but not overall compute.
The more complex techniques target reducing computation during training, such as TensorDash~\cite{mahmoud2020tensordash} and SAVE~\cite{gong2020save}. However, they need to give up data movement savings for better support for sparse tensor transposition during training.
TASD can potentially be used to approximate sparse activations and gradients, but we leave this to future work. 
%As prior work~\cite{li2022large, rhu2018cdma} has shown that the degree of activation and gradient sparsity stays stable, TASD-A can approximate these dynamic tensors during runtime to enable the efficient structured sparse HW support for sparse training. We leave this to future work.

%OFA ...
%\begin{itemize}
%    \item Add more works related to weight sparsity
%    \item Add more works related to input sparsity
%    \item Add more works related to converting unstructured to structured
%    \item Add more works on sparse HW
%    
%\end{itemize}

==> mlsys2025style/sections/7_conclusion.tex <==
% Conv/FF -> GEMM
% Inference
% Define Approximated sparsity
% 2 TASD terms -> 1:8 to 6:8
% small value distribution for GELU
% figure 8; across images

% 4 workloads representative layers
% dense resnet50/bert
% spares resnset50/bert


\section{Conclusion}
%Exploiting sparsity is a promising area to improve DNN efficiency. 
%However, 
Sparse DNN model developers prefer to induce unstructured sparsity for expressibility, while sparse DNN hardware designers prefer to support structured sparsity for HW efficiency.
This mismatch of the desired sparsity pattern 
between different parties
prevents sparse DNN acceleration from being widely adopted in practice.
To close the gap,
%between sparse DNN models and hardware,
we introduce TASD, a method that approximates an unstructured sparse tensor with a series of structured sparse tensors.
Next, we propose a framework, TASDER, which finds TASD configuration for each DNN layer
% to apply TASD
to accelerate sparse and dense DNNs.
To maximize the benefit of TASD,
we propose a simple architectural extension and dataflow on top of structured sparse accelerators.
%We evaluate TASD across DNN workloads to show TASD enables pragmatic sparse DNN acceleration.
%For four different DNNs,
TASD improves EDP up to 83\% and 74\% on average, while maintaining 99\% of the model accuracy without any fine-tuning.
We also show it achieves up to 39\% performance improvement on a real system evaluation.
    



%~\ref{sample-table}.


==> mlsys2025style/sections/backups.tex <==
%%%%
\subsection{Search algorithm for TASD selection}
\begin{algorithm}[tb]
   \caption{TASD Selection Algorithm}
   \label{alg:tasd_sel}
\begin{algorithmic}
   \STATE {\bfseries Input:} $target\_sparsity$, $alpha$, $H$
   \STATE $target\_sparsity = sparsity + alpha$
   \IF{$target\_sparsity > H[3]$}
   \STATE return $H[3]$
   \ENDIF
   \IF{$target\_sparsity > H[2]$}
   \STATE return $H[2]$
   \ENDIF
   \IF{$target\_sparsity > H[1]$}
   \STATE return $H[1]$
   \ENDIF
   \IF{$target\_sparsity > H[0]$}
   \STATE return $H[0]$
   \ENDIF
\end{algorithmic}
\end{algorithm}

In \autoref{alg:tasd_sel}, we show the sparsity-degree-based TASD Selection algorithm explained in \autoref{subsec:tasd-w}.
%\vspace{-2em}
%\input{algorithms/find_config}
%%%%
%%%% Background
\begin{comment}
     
    Dense: 
    - "8:8"
    Unstructured sparse is 
    - "flexible N: fix M"

    Data itself: 
    View? 

    Matrix (c)
    matrix c is sparse. -- data 
    Matrix C has 2:4 sparsity patterns. -- compression format
    Matrix C has unstructured sparsity patterns -- compression format
    Matrix C has flexible N:8 sparsity patterns.
    
    Matrix C is 2:4 sparse.
    Matrix C is unstructured sparse. 
    Matrix C is flexible N:8 sparse.

    Matrix A is 2:4 sparse. -- false
    Matrix A is unstructured sparse. 
    
    Matrix A is flexible N:8 sparse. -- yes
    Matrix B is flexible N:8 sparse. -- yes
    Dense and unstructured sparsity are same?
    
    Matrix B is 2:4 sparse.
    Matrix B is unstructured sparse. 

    "Dense" in HW and SW means differently

    tensor
    "a view of a tensor" from SW
    "a view of a tensor" from HW
    architecture contract
    
    
    flexible N:M == unstructrued sparsity pattern
\end{comment}

\begin{comment}
To summarize, there are two main research questions in this project.
\begin{enumerate}
    \item Could TASD be applied to DNN models without losing significant accuracy compared with the baseline model?
    \item What are the efficient accelerator architecture and programming model to support TASD?
\end{enumerate}

\end{comment}
%%%% TASD
\begin{comment}
With the insight from \autoref{subsec:tasd_analysis}, we propose a sparsity-degree-based method to choose the TASD configuration based on the sparsity degree of each layer.
Consider a flexible structured sparse HW with 2:4 and 2:8 support as the target, 
to express the approximated sparsity, the sparsity degree covered by a TASD configuration $C$, we use $S(C)$.
For example, $S([2:4]) = 50\%$ while $S([2:4, 2:8]) = 25\%$.
There are four TASD configurations available with the target HW, $H_1$ = [1:1], $H_2$ = [2:4, 2:8], $H_3$ = [2:4], and $H_4$ = [2:8] where the corresponding sparsity covered by the TASD configuration is 0\%, 25\%, 50\%, and 75\%.

We use a hyperparameter, $\alpha$, to tune the aggressiveness of the TASD approximation. 
For a given layer $L_i$ and the TASD configurations available to the target HW ($H_1, ... , H_4$ for this case), we choose $C_i$ as $H_j$ where j is the largest integer where $S(L_i) + \alpha > H_j$.
If we use a larger $\alpha$, we choose the TASD configuration more aggressively (allowing more dropped non-zeros). 
We summarize the algorithm in \autoref{lst:tasd}.
We use TCONV/TFC to indicate a CONV/FC layer with TASD as shown in \autoref{fig:conv-tconv}, and the TASD configurations found above would be applied to the corresponding TCONV/TFC layers.
In \autoref{fig:conv-tconv} (a), we show how the conventional CONV/FC layer works with unstructured sparse activations (usually from ReLU) with dense weights. In \autoref{fig:conv-tconv} (b) shows how a TCONV/TFC layer works. As explained above, TASDER would modify unstructured sparse weights to structured sparse weights with TASD-W.
\vspace{-1em}
\input{algorithms/find_config}
\vspace{-1em}
\end{comment}

\begin{comment}
% PDF For ConvNEXT Pseudo Density
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-pseudo-density.png}
        %\vspace{-1.5em}
	\caption{PDF of the element magnitude of an activation tensor from a GELU-based DNN, \textit{ConvNext-Tiny}. TASD-A uses a pseudo-density heuristic for non-ReLU DNNs.}
	\label{fig:tasd-pseudo-density}
 \vspace{-1em}
\end{figure}
\end{comment}
\begin{comment}
For simplicity, let $B$ be an unstructured sparse matrix representing input activations (usually derived by the image-to-column algorithm to convert a convolution operation into a general matrix multiplication, GEMM with $D = A \times B + C$ where $A$, $C$, and $D$ refer to a weight, bias, and output, respectively).  

Then, the matrix multiplication $AB$ can be expressed as $A(B_1 + B_2) = AB_1 + AB_2$ and each $AB_i$ can be executed on a sparse tensor core which supports 2:4 structured sparsity (such as the ones in NVIDIA Ampere GPUs).
However, this decomposition does not reduce the number of computations required for the entire $AB$, so it cannot improve performance under the same number of Multiply and Accumulate (MAC) units.
\end{comment}
\begin{comment}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.47\textwidth]{figures/uniform_result.pdf}
 \vspace{-0.5em}
	\caption{Percentages of dropped non-zeros and the sum of dropped non-zeros after applying different TASD series on a matrix generated with \textbf{uniform random distribution}.}
	\label{fig:uniform_result}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-w.pdf}
	\caption{ResBlocks from ResNet50 with CONV and TCONV layers.}
	\label{fig:tasd-w}
\end{figure}
\end{comment}

\section{Po-An's brain dump}
Sparsity in the DNNs gives a huge opportunity to improve efficiency and performance, by eliminating storing, transferring, and computing on zeros. The most effective and natural way to induce sparsity while preserving accuracy is to introduce sparsity across the whole network and make a global decision on 1) which elements (in both weight and activation tensors) and 2) how much (sparsity degree) to introduce zeros. This HW-agnostic design space and preference from the developer leads to a friendlier abstraction toward unstructured sparsity, because the designer does not need to think about HW, just to focus on the network accuracy and flops/model size tradeoff.

Nonetheless, unstructured sparsity often is incompatible with the popular and emerging parallel HW architecture that serves the DNN need well. For example, unstructured sparsity introduces irregular memory accesses and diverged control/execution patterns that are hostile to parallel HW GPU and specialized HW like tensor core/systolic array.

To address this issue, a new method to bridge between sparsity and its HW performance is to introduce extra design spaces that are parallel HW-oriented, namely structure (or the degree of structuredness) and granularity. Such design space forces the DNN designer to induce sparsity with certain constraints at a cost of achievable sparsity degree for iso-accuracy comparison, but promises predictable performance and energy efficiency benefits on top of the existing parallel or specialized HW. For example, NVIDIA's fine-grained structured sparsity support balances the imposed constraints and achievable performance and provides a good target for DNN developers to optimize the network for.

However, such methods also move the burden from the HW designers to DNN developers, as there is already a massive design space (network architecture, training recipe, hyperparameters) to explore. Moreover, extending the existing support to more patterns (e.g., not only 2:4, cite VEGETA and S2TA) also means more overhead and burden for both HW designers and DNN developers.

In this paper, we ask "how can we design a system to provide the free and simple unstructured sparse interface to the DNN developers, but only use structured sparse HW support while providing predictable performance and efficiency gains?" Our answer is to redefine the DL sparsity programming abstraction and introduce a level of indirection through DL system SW and HW. Specifically, we introduce an idea named structured tensor decomposition to approximate any unstructured sparse tensor with a series of structured sparse tensors. Leveraging the distributed property of tensor algebra, we further propose to dynamically "decode" an unstructured sparse tensor algebra operation into a series of "microcode", structured sparse tensor algebra operations, which are efficient and compatible with existing parallel and specialized HW architecture. 

%%%% Eval
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/acc_flop_resnet50_overview.pdf}
	\caption{Evaluation of TASD-A on ResNet50.}
	\label{fig:maccounts}
\end{figure}


\begin{comment}
\subsection{
Impact of TASD configuration search
}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/greedy-search.pdf}
         \vspace{-2em}
	\caption{
        \rev{EDP comparison between different TASD configuration selection methods on Sparse ResNet50. CHANGE THIS TO TABLE!!
        }
 }
	\label{fig:greedy-search}
 \end{figure}

In \autoref{subsec:tasd-w}, we introduced a simple, per-layer sparsity-based heuristic to determine the TASD configuration.
Such a heuristic may not lead to the optimal configuration for the whole DNN that preserves 99\% model quality and minimizes total computation.
To address this, we design and implement another greedy-based algorithm that optimizes across all layers.
This greedy algorithm first measures the percentage of dropped non-zero elements of each TASD configuration for all layers and sorts the configuration-layer pairs by their percentage of dropped elements.
Next, it greedily applies the TASD configuration based on the sorted order until the model quality is <99\% of the original model (i.e., prioritize the option with the smallest dropped non-zeros).


We find that this global, greedy-search-based method further improves EDP for TTC-VEGETA-M8 by 18\%, and TTC-VEGETA-M4 by 10\% for sparse ResNet50, which shows that finding a high-quality TASD configuration can further improve the effectiveness. 
We leave developing the optimal algorithm leveraging other metrics for future work. 
\end{comment}

\begin{comment}    
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-networkwise-a.pdf}
 \vspace{-0.5em}
	\caption{
 \rev{Network-wise and Layer-wise TASD-A on dense ResNet50.}
 }
	\label{fig:resnet50-95-networkwise-a}
\end{figure}
\end{comment}    

\begin{comment}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-layerwise-a.pdf}
 \vspace{-0.5em}
	\caption{Layer-wise TASD-A on dense ResNet50.}
	\label{fig:resnet50-95-layerwise-a}
\end{figure}
\end{comment}
\begin{comment}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-a-maccounts.pdf}
         \vspace{-0.5em}
	\caption{Layer-wise TASD-A on more DNN models.}
	\label{fig:maccounts}
 \end{figure}
\end{comment}

\begin{comment}    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-layerwise-w.pdf}
 \vspace{-0.0em}
	\caption{Layer-wise TASD-W on sparse ResNet50.}
	\label{fig:resnet50-95-layerwise-w}
\end{figure}
\end{comment}



%%% Table
\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


==> mlsys2025style/tables/comparison.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
%\newcommand{\xmark}{ %\textcolor{darkyellow}{\ding{56}}}
\newcommand{\xmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}

\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
&
{\textbf{Dense}}
&
{\textbf{Unstructured}}
&
{\textbf{Structured}}
&

\\
&
{\textbf{Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Pruned Model}}
&

\\
\hline
Sparsity Degree
&
None
&
High
&
Low-Mid
&
{\textbf{Extra}}
\\
\cline{1-4}
Fine-tuning Time
%& \textbf{Intrinsics} 
&
None
&
Short
&
Long
&
{\textbf{Area}}
\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& None
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured HW
\end{tabular}
& \downmark
& \upmark
& \xmark~or \upmark
& High
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured HW
\end{tabular}
& \xmark
& \xmark
& \upmark
& Low
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark %~(TASD-A)
& \upmark
& \upmark
& Low
\\
\hline

\end{tabular}

\hfill
\caption{Comparison of sparse DNN models and sparse DNN HW supports.  \upmark~: Better than dense HW in EDP (Energy Delay Product). \downmark~: Worse than dense HW in EDP. \xmark~: No EDP Improvement.}
%\vspace{-1.em}
\label{table:nm-hw}
\end{table}

==> mlsys2025style/tables/comparison2.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
%\newcommand{\xmark}{ %\textcolor{darkyellow}{\ding{56}}}
\newcommand{\xmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}

\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
&
{\textbf{Dense}}
&
{\textbf{Unstructured}}
&
{\textbf{Structured}}
&
{\textbf{Extra}}
\\
&
{\textbf{Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Area}}
\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense HW~\cite{jouppi2017tpu}
\end{tabular}
& \xmark
& \xmark
& \xmark
& None
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstr. HW~\cite{qin2020sigma,parashar2017scnn,wang:dual-side}
\end{tabular}
& \downmark
& \upmark
& \xmark~or \upmark
& High
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Str. HW~\cite{liu2021s2ta,jeong:vegeta}
\end{tabular}
& \xmark
& \xmark
& \upmark
& Low
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark %~(TASD-A)
& \upmark
& \upmark
& Low
\\
\hline

\end{tabular}

\hfill
\caption{Comparison of sparse DNN models and sparse DNN HW supports. \xmark~: No EDP Improvement over dense HW. \upmark~: Better than dense HW in EDP (Energy Delay Product). \downmark~: Worse than dense HW in EDP. }
\vspace{-1.em}
\label{table:nm-hw}
\end{table}

==> mlsys2025style/tables/comparison3.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
%\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
\newcommand{\xmark}{ \textcolor{darkred}{\ding{56}}}
\newcommand{\hmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}
\begin{scriptsize}
\begin{table}[t] 
\scriptsize
\centering
\caption{Comparison of DNN HWs. Unstr: Unstructured sparse. Str: Structured sparse. Wgt: Weights. Act: Activations.}
\begin{tabular}{|c|c|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
HW Support
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Str}}
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Area}}

\\
$\downarrow$
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Act}}
&{\textbf{Act}}
&
{\textbf{Cost}}

\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense~\cite{jouppi2017tpu, nvidia_volta, rasa}
\end{tabular}
& \cmark
& \xmark
& \xmark %\xmark~or \upmark
& \cmark
& \xmark
& \cmark\cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstr~\cite{qin2020sigma,parashar2017scnn,wang:dual-side}
\end{tabular}
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
%\tablefootnote{Unstructured sparse HW could be energy efficient if the workload is very sparse, which is not often the case for DNN models.}
& \cmark
& \cmark %\xmark~or \upmark
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
& \cmark
& \xmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Str~\cite{zhu2019micro, liu2020sta,jeong:vegeta, nvidia_ampere}
\end{tabular}
& \cmark
& \xmark
& \cmark
& \cmark
& \xmark
& \cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \cmark %~(TASD-A)
& \cmark
& \cmark
& \cmark\cmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[7]
%\tablefootnote{TASD enables further acceleration through approximation.}
& \cmark 
& \cmark
\\
\hline

\end{tabular}

\hfill
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\begin{minipage}{1.0\linewidth}
\footnotemark[1]{With extra wiring/logic, unstructured sparse HW is inefficient if the tensor is dense.}\mbox{}\hfill
\end{minipage}
\begin{minipage}{1.0\linewidth}
\footnotemark[7]{TASD enables further acceleration by approximating dense tensors with sparse tensors.}\mbox{}\hfill
\end{minipage}

\vspace{-2.5em}
\label{table:nm-hw}
\end{table}
\end{scriptsize}


==> mlsys2025style/tables/comparison4.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
%\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
\newcommand{\xmark}{ \textcolor{darkred}{\ding{56}}}
\newcommand{\hmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}
\begin{small}
\begin{table*}[!ht] 
\small
\centering
\caption{Comparison of DNN HWs. Unstr: Unstructured sparse. Str: Structured sparse. Wgt: Weights. Act: Activations.}
\begin{tabular}{|c|c|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
HW Support
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Str}}
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Area}}

\\
$\downarrow$
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Act}}
&{\textbf{Act}}
&
{\textbf{Cost}}

\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense~\cite{jouppi2017tpu, nvidia_volta, rasa}
\end{tabular}
& \cmark
& \xmark
& \xmark %\xmark~or \upmark
& \cmark
& \xmark
& \cmark\cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstr~\cite{qin2020sigma,parashar2017scnn,wang:dual-side}
\end{tabular}
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
%\tablefootnote{Unstructured sparse HW could be energy efficient if the workload is very sparse, which is not often the case for DNN models.}
& \cmark
& \cmark %\xmark~or \upmark
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
& \cmark
& \xmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Str~\cite{zhu2019micro, liu2020sta, nvidia_ampere,jeong:vegeta}
\end{tabular}
& \cmark
& \xmark
& \cmark
& \cmark
& \xmark
& \cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \cmark %~(TASD-A)
& \cmark
& \cmark
& \cmark\cmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[7]
%\tablefootnote{TASD enables further acceleration through approximation.}
& \cmark 
& \cmark
\\
\hline

\end{tabular}

\hfill
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\begin{minipage}{1.0\linewidth}
\footnotemark[1]{With extra wiring/logic, unstructured sparse HW is inefficient if the tensor is dense.}\mbox{}\hfill
\end{minipage}
\begin{minipage}{1.0\linewidth}
\footnotemark[7]{TASD enables further acceleration by approximating dense tensors with sparse tensors.}\mbox{}\hfill
\end{minipage}

%\vspace{-2.5em}
\label{table:nm-hw}
\end{table*}
\end{small}


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/algorithms/find_config.tex <==


\begin{minipage}[t]{\linewidth}
\begin{center}
\vspace{-0.3em}
\begin{lstlisting}[caption={The sparsity-degree-based TASD selection.}\label{lst:tasd},escapechar=\%]
target_sparsity = sparsity + alpha;
if (target_sparsity > H[3]): return H[3];
else if (target_sparsity > H[2]): return H[2];
else if (target_sparsity > H[1]): return H[1];
else if (target_sparsity > H[0]): return H[0];
\end{lstlisting} 

\end{center}
\end{minipage}



==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/include/shorthands.tex <==
%%%%% BLUE is same as hyperref, could be confusing, so not keeping here %%%%%
\newcommand{\GJ}[1]{{\color{brown}\bfseries [Geonhwa:: #1]}}
\newcommand{\PT}[1]{{\color{magenta}\bfseries [Po-An:: #1]}} 
%\newcommand{\AB}[1]{{\color{magenta}\bfseries [Abhimanyu:: #1]}}
%\newcommand{\cjh}[1]{{\color{cyan}\bfseries [Chris:: #1]}} 
%\newcommand{\HK}[1]{{\color{violet}\bfseries [Hyesoon:: #1]}}
\newcommand{\SK}[1]{{\color{teal}\bfseries [Steve:: #1]}}
\newcommand{\TK}[1]{{\color{cyan}\bfseries [Tushar:: #1]}}
\newcommand{\todo}[1]{\textcolor{red}{TODO:: #1}}
\newcommand{\rev}[1]{\textcolor{red}{#1}}

% Sections
\def\Snospace~{\S{}}
\renewcommand*\sectionautorefname{\Snospace}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section }


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/0_abstract.tex <==
\begin{abstract}

Exploiting sparsity in deep neural networks (DNNs) has been a promising area for meeting the growing computation requirements.
%However, in practice, sparse DNN acceleration still faces a key challenge. 
To minimize the overhead of sparse acceleration, hardware designers have proposed \emph{structured sparsity} support, but it provides limited flexibility and requires extra model fine-tuning. Moreover, any sparse model fine-tuned for certain structured sparse HW cannot be accelerated by other structured hardware.
%To bridge the gap between sparse DNN models and hardware, 
To enable acceleration using unstructured sparsity of DNNs on structured sparse hardware, we propose an approximation method leveraging 
%tensor approximation via structured decomposition (TASD), which leverages 
the distributive property in linear algebra to turn any sparse tensor into a series of structured sparse tensors.
We also develop a software framework, TASDER, to apply high-quality structured approximation on weights and activations of DNNs.
%to accelerate DNNs by searching layer-wise, high-quality structured decomposition for both weight and activation tensors so that they can be accelerated by any systems with structured sparse hardware support.
%by exploiting prior structured sparse hardware baselines
Our method accelerates dense and sparse DNNs without fine-tuning and improves energy-delay-product (EDP) by up to 83\% and 74\%. It achieves up to 39\% speed-up on a real system.
\end{abstract}


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/1_intro_old.tex <==
\section{Introduction}

\TK{pls rewrite! see my comment on slack}

DNNs have revolutionized various domains, such as computer vision~\cite{krizhevsky2012alexnet,convnext,vit}, personal recommendation~\cite{dlrm}, speech recognition~\cite{deepspeech2}, and natural language processing~\cite{gpt2,devlin-etal-2019-bert}. 
%Meanwhile, DNNs are also demanding more computation for diverse model capabilities and higher operational performance. The DNN models are scaling to billions of model parameters \cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron} often with high-resolution 2D and 3D inputs~\cite{lin2017focal,cciccek20163d} under real-time requirements.
Meanwhile, DNN inference is also demanding more computation as they scale to billions of model parameters \cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron} and consume an enormous amount of input data~\cite{lin2017focal,cciccek20163d}.
%Recently, Deep Learning (DL) has achieved great success across various domains including, but not limited to, computer vision, personal recommendation, speech recognition, and natural language processing~\cite{lecun2015deep}. 
%To squeeze out the full potential of DNN models with large datasets and powerful compute resources, one of the recent trends is making the model deeper and larger, often exceeding billions or trillions model parameters such as Megatron, PaLM, and Switch Transformer~\cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron}.
%On the other hand, some DNN models use high-resolution inputs to exploit more information from the input to achieve higher accuracy while incurring larger intermediate feature maps as the trade-off.
%The enormous number of parameters and large feature maps cause huge memory footprint as well as an extremely large number of computations, which is a critical problem for both edge devices and datacenter computers.
%Since performance is an overloaded term, we distinguish computational (i.e., latency, throughput, etc.) and operational (i.e., the accuracy of DNN classification) performance in this paper.
To address the increasing demand for DNN models, researchers propose to exploit \emph{sparsity} in DNN models.  
%Fortunately, researchers have found a technique called model compression to reduce the memory footprint and improve performance.
%that there are two sparsities that they can exploit to reduce the burden; weight (static) sparsity and input (dynamic) sparsity; the former is extrinsic while the latter is intrinsic.
%Weight sparsity is the result of a well-known model compression technique, model pruning~\cite{han2015deep}, which removes a set of parameters in the target DNN model based on certain rules, thereby potentially reducing both memory footprint and the required number of computations. 
Model pruning~\cite{han2015deep} is the most popular method to remove a set of parameters in the target DNN model based on certain criteria, inducing \emph{weight sparsity}.
%Weight sparsity is often called as static sparsity since the sparsity pattern is fixed across different inferences using the model.
This optimization exploits a phenomenon that empirically, large models are often overly parameterized and do not need all parameters to maintain the target accuracy at inference time.
Deep learning (DL) model developers prefer to induce \textbf{unstructured sparsity} on weights so that they can focus on developing pruning algorithms to achieve better model accuracy and computation/model size trade-offs without any restriction.
Also, many DNN models naturally exhibit \emph{activation sparisty} due to the rectified linear unit (ReLU) that clips negative activation values to zeros, which induces unstructured activation sparsity.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/tasd-high-level-fig.pdf}
 \vspace{-1.5em}
	\caption{Different flows to exploit sparsity in DNNs.}
 \vspace{-1.5em}
	\label{fig:tasd-high-level-fig}
\end{figure}
%While unstructured sparsity is the preferred method to compress DNNs, 
As a result, early sparse DNN accelerators~\cite{parashar2017scnn,wang:dual-side,qin2020sigma} target unstructured sparsity and can accelerate any sparse DNNs.
Unfortunately, unstructured sparsity support is challenging to deploy as a specialized HW unit 
%support for unstructured sparsity in commercial devices, 
as it causes significant area and energy overhead for indexing logic and flexible distribution/reduction logic~\cite{jeong:vegeta}.
Without native HW support, unstructured sparsity in DNNs lead to irregular memory accesses and diverged control/execution patterns, which are hostile to parallel architectures like GPUs%
\footnote{The only sparse DNN accelerators on commercial devices is NVIDIA Sparse Tensor Core\cite{nvidia_ampere}, which supports a fixed 2:4 
 structured sparsity.} and specialized tensor accelerators like tensor core and systolic array. 
This forces DNN model developers today to constrain the DNN sparsity search space to only consider coarse-grained \emph{structured patterns}, such as channel or filter pruning~\cite{molchanov2022lana, chen2022coarsening}, while maintaining iso-accuracy, thereby, moving the burden to DNN model developers.

%To address this issue, an alternative to bridge
%DNN sparsity and HW performance is to introduce extra design
%spaces that are parallel HW-oriented, namely structure (or
%the degree of structuredness) and granularity.
To balance the need, recently, hardware (HW) designers~\cite{nvidia_ampere,jeong:vegeta,liu2021s2ta,zhu2019micro} have proposed \emph{fine-grained} structured sparsity support.
Such designs force DNN developers to induce sparsity with certain constraints at a cost of achievable sparsity degree for iso-accuracy comparison, but promise predictable performance
gain on top of the existing DNN supports.
For example, NVIDIA’s fine-grained 2:4 structured sparsity support balances the imposed constraints and achievable performance and provides a good target for DNN developers to optimize the network for.
However, such methods impose an extra burden on DNN developers on top of the existing huge design space (DNN architectures, training recipes, etc.) to explore. Moreover, extending the existing support to more patterns~\cite{jeong:vegeta, sun2021domino} means more overhead and design space exploration for both HW designers and DNN developers.
We summarize different flows to exploit sparsity in \autoref{fig:tasd-high-level-fig}.

%In this paper, we ask "how can we design a system to provide the unstructured sparse interface to the DNN developers, but only with structured sparse hardware support, while providing predictable performance and efficiency gains?" 
\textbf{In this paper}, we ask ``Can we design a system to expose the flexible unstructured sparse interface to the DNN developers, but only with the efficient, less flexible structured sparse HW support?" 
Our answer is to introduce a new level of abstraction between DL model developers and hardware designers, similar to the abstraction layer in the instruction-set architectures. Specifically, we introduce a method, structured sparse tensor decomposition, to approximate any sparse tensor with a series of structured sparse tensors.
Leveraging the distributed property of tensor algebra,
we further propose to dynamically "decode" an unstructured
sparse tensor algebra into a series of "microcode", i.e., structured sparse tensor algebra, which are efficient and compatible with prior structured sparse hardware.
%\TK{I think somewhere in this section or in the first bullet a strong statement like ``First work to .." will be nice to have}
%To exploit the benefits of both approaches, we propose a novel method, Tensor Approximation via Structured Decomposition (TASD) and show how it can be used to leverage unstructured input sparsity using a set of structured sparse tensors.
%Furthermore, we have observed that different layers prefer different TASD configurations, so we propose an efficient method to choose TASD configurations per layer to minimize accuracy loss while maximizing performance gain.

We make the following contributions: 
\begin{itemize}
    \item We present the first work to bridge unstructured sparse DNN and structured sparse HW with Tensor Approximation via Structured Decomposition (TASD), which approximate any sparse tensor with a series of structured sparse tensors.
    \item We propose a framework, TASDER, which finds the TASD series for each DNN layer to accelerate dense/sparse DNNs with structured sparse hardware.
    \item We propose a simple architectural extension and dataflow on top of existing structured sparse accelerators~\cite{jeong:vegeta} to execute TASD series efficiently.
    \item For various off-the-shelf dense and sparse DNNs, we show that TASD improves EDP by up to 83\% and by 70\% on average. We also show that across a range of DNNs, TASD can reduce the computation by 40\%. We validate the effectiveness of TASD on a real NVIDIA GPU and achieve up to 39\% speed-up.
\end{itemize}


\begin{comment}
The organization of the paper is the following.
\begin{itemize}
    \item Section 2 reviews the background in DNN sparsity and
how DNN developers induce sparsity, as well as previous HW support DNN sparsity. We also show why
providing unstructured sparse HW support might not
be the best solution.
    \item Section 3 explains the idea of TASD and a preliminary analytical study of how effective TASD is as an
approximation method.
    \item Section 4 describes a TASD-based HW and SW codesign that enables the DNN developer to freely induce
sparsity without structured and granularity constraints.
    \item Section 5 shows the evaluation of the proposed system,
as well as a case study of applying TASD on off-the-shelf HW (NVIDIA Ampere GPUs).
    \item Finally, we discuss extra related work in Section 6 and conclude this paper in section 7.
\end{itemize}
\end{comment}

%Thus, For example, the only commercial HW that can leverage sparsity for efficient calculation is NVIDIA Sparse Tensor Core.
%During the pruning, This HW-agnostic design space and preference from the developer leads to a friendlier abstraction toward unstructured
%sparsity, because the designer does not need to think about
%HW, just to focus on the network accuracy and flops/model size tradeoff.





==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/1_new_intro.tex <==
\section{Introduction}
%My suggestion is to talk purely about 
% 1. sparsity being promising from model side but extremely expensive to support in HW .. 
% 2. then talk purely about HW - how there is a spectrum of choices (i think the figure from your thesis talk may be valuable) .. cite the diff works .. and show how HW is converging towards structured - mentioning NVIDIA STC, VEGETA etc ..
%And then say this limits this HW to only be used if model is trained in structured manner. And then say this work allows any unstructured sparse model to run on structured HW ..

%speech recognition~\cite{deepspeech2}, 
%DNNs have revolutionized various domains, such as computer vision~\cite{krizhevsky2012alexnet,convnext,vit}, personal recommendation~\cite{dlrm}, and natural language processing~\cite{gpt2,devlin-etal-2019-bert}. 

DNNs have revolutionized various domains~\cite{krizhevsky2012alexnet,convnext,vit, dlrm, gpt2,devlin-etal-2019-bert}, but DNN inference demands extreme compute power, memory footprints, and memory bandwidth as models scale to billions and trillions of parameters \cite{shoeybi2019megatron, fedus2021switch, chowdhery2022palm}.
%touvron2023llama2openfoundation
%and large input datasets~\cite{lin2017focal,cciccek20163d}.
To mitigate this growing demand, \emph{sparsity} has emerged as a promising opportunity. 
%DNN models.  
Model pruning~\cite{han2015deep} is the most popular method to remove a set of parameters in DNNs.
%based on certain criteria. %, inducing \emph{weight sparsity}.
This optimization exploits a phenomenon that large models are often overly parameterized and do not need all parameters to maintain the target accuracy. % at inference time.
Model pruning induces unstructured sparsity on weights (i.e. there is no specific pattern in the distribution of zeros) \text{unless} constraints are enforced during the pruning.
Also, many DNN models naturally exhibit activation sparsity due to the rectified linear unit (ReLU) that clips negative activation values to zeros resulting in unstructured sparsity.

%While unstructured sparsity is the preferred method to compress DNNs, 

Unfortunately, unstructured sparsity in DNNs leads to irregular memory accesses and diverged control/execution patterns, which are hostile to parallel architectures like GPUs, tensor cores~\cite{nvidia_volta}, and systolic arrays~\cite{jouppi2017tpu}. 
%and specialized dense tensor accelerators like tensor cores~\cite{nvidia_volta} and systolic arrays~\cite{jouppi2017tpu}.
This has led to a plethora of academic research on unstructured sparsity support in DNN accelerators~\cite{parashar2017scnn, extensor,qin2020sigma,wang:dual-side, eureka2023micro}. 
Nonetheless, the complexity in hardware required for unstructured sparsity, such as indexing logic~\cite{extensor} and flexible distribution/reduction logic~\cite{qin2020sigma}, has been prohibitive in their commercial adoption.

%nvidia_hopper
Recent sparse DNN accelerators \cite{zhu2019micro,nvidia_ampere, liu2021s2ta, jeong:vegeta, AMD_MI300, Moffett_antoum} have proposed \textit{structured sparsity} support. 
The most popular example is \emph{fine-grained} N:M sparsity, 
which constrains at most N non-zeros in each block composed of M consecutive elements.
A commercial example of this is NVIDIA's sparse tensor core (STC) with 2:4 structured sparsity.
%N:M structured sparsity imposes some degree of regularity in data, allowing lower overhead for sparsity support compared to unstructured sparsity while promising predictable performance gains.
%on top of the existing DNN supports.
Structured sparse hardware forces DNN model developers to induce sparsity with certain constraints. \textit{Otherwise, that hardware is unusable.}
%at a cost of achievable sparsity degree for iso-accuracy comparison.
For example, NVIDIA’s fine-grained 2:4 structured sparsity support could provide 2$\times$ throughput by skipping ineffectual computations \textit{only if} the model is tuned with 2:4 structured sparsity. 
A model that does not follow 2:4 structured sparsity would, in fact, need to run on the dense tensor core, losing the benefits of sparsification.
%\footnote{It may benefit from compressed storage in memory but has to be decompressed and run on dense tensor cores without taking compute benefits.}. 
On the flip side, a 2:4 structured sparse model cannot be accelerated on different structured sparse hardware, such as a sparse tensor core with 1:4 or 2:8 structured sparsity support.
Therefore, while the availability of structured sparse hardware is extremely promising, it remains limiting for model developers as it requires tuning the model to the specific sparsity support of the hardware, in addition to navigating the already vast design space, including DNN architectures and training recipes. This makes the broad adoption of structured sparse hardware challenging.
%Therefore, the availability of structured sparse hardware, while extremely promising, is still very limiting for model developers as it requires tuning the model for the specific sparsity support in the hardware, on top of the already huge design space (DNN architectures, training recipes, etc.) to explore, making the adoption of the structured sparse HW challenging. 
%Moreover, we get no benefits today from the structured sparse hardware for unstructured activation sparsity.
%To execute the model on another HW with 4:8 structured sparsity, the model has to be tuned again to meet the constraint.
%Therefore, such methods impose an extra burden on DNN developers to tune the model for each HW to leverage structured sparsity support on top of the existing huge design space (DNN architectures, training recipes, etc.) to explore, making the adoption of the structured sparse HW difficult. 
%Also, extending existing structured sparse hardware support to more patterns~\cite{jeong:vegeta, sun2021domino} means adding more overhead and a larger design space exploration and cost vs. benefit trade-off space.


%This forces DNN model developers today to constrain the DNN sparsity search space to only consider certain \emph{structured patterns}, such as channel or filter pruning~\cite{molchanov2022lana, chen2022coarsening} while maintaining iso-accuracy, thereby, moving the burden to DNN model developers.

%The only sparse DNN accelerators on commercial devices is NVIDIA Sparse Tensor Core\cite{nvidia_ampere}, which supports a fixed 2:4  structured sparsity.

%Deep learning (DL) model developers prefer to induce \textbf{unstructured sparsity} on weights so that they can focus on developing pruning algorithms to achieve better model accuracy and computation/model size trade-offs without any restriction.
%Also, many DNN models naturally exhibit \emph{activation sparisty} due to the rectified linear unit (ReLU) that clips negative activation values to zeros, which induces unstructured activation sparsity.
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/tasd-high-level-fig.pdf}
 \vspace{-1em}
	\caption{Different flows to exploit sparsity in DNNs.}
 \vspace{-1em}
	\label{fig:tasd-high-level-fig}
\end{figure}

In this paper, we ask and answer the following  question \textbf{``Can we decouple the dependency between DNN models and HW, so that a model with \textit{any sparsity pattern} can be accelerated on \textit{any structured sparse HW}?}"
%Can we design a system to expose the flexible unstructured sparse interface to the DNN developers, but only with the efficient, less flexible structured sparse HW support?" 
Our answer is to introduce a new level of abstraction between DL model developers and hardware designers. %similar to the abstraction layer in instruction-set architectures. 
Specifically, we introduce a method, structured sparse tensor decomposition, to approximate any sparse tensor (such as pruned weights or intrinsic sparse activations) with a series of structured sparse tensors.
%\TK{maybe add a footnote here saying we can also approximate dense tensors with TASD, allowing us to leverage multiple passed through the sparse hardware for dense tensors}
Leveraging the distributed property of tensor algebra,
we further propose to dynamically ``decode" an unstructured sparse tensor algebra into a series of %``microcode", i.e., 
structured sparse tensor algebra, which is efficient and compatible with prior structured sparse hardware. 
%\footnote{In fact, not only for sparse tensors, but also one can use our proposed method to approximate dense tensors to execute it over structured sparse HW, helping utilize sparse HW for dense workloads instead of keeping it idle.}. 
We contrast our proposed approach with current flows to exploit sparsity in \autoref{fig:tasd-high-level-fig}.
%\TK{I think somewhere in this section or in the first bullet a strong statement like ``First work to .." will be nice to have}
%To exploit the benefits of both approaches, we propose a novel method, Tensor Approximation via Structured Decomposition (TASD) and show how it can be used to leverage unstructured input sparsity using a set of structured sparse tensors.
%Furthermore, we have observed that different layers prefer different TASD configurations, so we propose an efficient method to choose TASD configurations per layer to minimize accuracy loss while maximizing performance gain.

We make the following contributions: 
\begin{itemize}
    \item We propose Tensor Approximation via Structured Decomposition (TASD), which approximates any sparse tensor with a series of structured sparse tensors. TASD is the first work to demonstrate running unstructured sparse DNNs on structured sparse HW.
    \item We propose a framework, TASDER, a bridge between HW and SW to find the TASD series % for each DNN layer to 
    to accelerate dense/sparse DNNs on structured sparse hardware.
    \item We propose a simple architectural extension and dataflow on top of existing structured sparse accelerators~\cite{jeong:vegeta} to execute TASD series efficiently.
    %off-the-shelf
    \item For various dense and sparse DNNs, we show that TASD improves EDP by up to 83\% and by 70\% on average. 
    We also show that across a range of DNNs, TASD can reduce the computation by 40\%.
    \item We show the effectiveness of TASD on commercial hardware (NVIDIA RTX 3080 GPU) with 2:4 sparse tensor cores and achieve up to 39\% performance gain.
\end{itemize}

==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/2_background.tex <==
\section{Background}
%In this section, we first explain several terminologies related to DNN sparsity as different terms are being used interchangeably in various communities such as HPC, ML, and hardware design. 
%Next, we summarize how sparsity is induced in DNN models and we illustrate the prior work on hardware acceleration exploiting DNN sparsity.

\subsection{Terminology}
%\textbf{Tensor} is a generalized form of scalars, vectors, and matrices with an arbitrary number of dimensions (or ranks), $N$, which are used to represent multi-dimensional data.

\textbf{Sparsity} is a characteristic of data that includes zeros. 
The sparsity degree of a given tensor is measured as the fraction of the number of zeros to the number of the total elements in the tensor.
If a tensor has 0\% sparsity degree, we call the tensor \emph{dense}. 
Sparsity by itself is often used to indicate sparsity degree.
To describe the distribution of zeros, a \textit{sparsity pattern} can be given to the tensor.
If there is no defined sparsity pattern, we call it \emph{unstructured sparsity}.
Various patterns can be classified as structured sparsity, such as block sparse~\cite{narang2017block}, butterfly sparse~\cite{dao2021pixelated}, and mixed patterns~\cite{zaheer2020big}.

One of the most popular patterns is \textbf{N:M structured sparsity}~\cite{zhou2021nm}, as it is supported in both commercial products~\cite{nvidia_ampere, AMD_MI300, Moffett_antoum} and academic proposals~\cite{liu2021s2ta,jeong:vegeta, bambhaniya2023accelerating} with active training recipe research~\cite{pool2021channel,mishra2021accelerating, nvidia_asp, NM_training_recipe,lu2023step, sparsegpt, bambhaniya2024progressive}.
% \TK{pls add more citations for N:M training recipe research - to showcase this is an active area. Also add venue (arxiv) for the current cited paper from Amir/Abhi.}.
%\TK{since this is background section, I *think* you can give examples of other structured sparse patterns like block sparse, butterfly (Beidi's paper), N:M .. and then add citations showing recent popularity of N:M and corresponding HW support,  fwd pointing to Sec 2.2 which will have more details.}
An N:M structured sparse tensor means that there can be at most N non-zeros in each M-element block in a certain rank of the tensor as shown in \autoref{fig:sparsity_patterns} (c).
%\autoref{fig:sparsity_patterns} shows different sparsity patterns.
%Sparsity constraint = the rules for the non-zero distribution in a tensor
%\TK{throughout the paper we seem to use structured and N:M interchangeably which is confusing. Maybe put a footnote here clarifying that in paper structured means flexible N:M}

We define \textbf{a view} of a tensor $A$ for a sparsity pattern as a tensor after potentially dropping some elements to meet the rule of the sparsity pattern.
For a matrix filled with non-zeros randomly, it is possible that the matrix does not meet the 2:4 sparsity pattern, i.e. there could be a block composed of 4 consecutive elements with more than two non-zeros.
To generate a 2:4 view of the matrix, some non-zeros in the matrix should be dropped (pruned in DNNs) to meet the pattern. As this process could drop some original values, it can be \textit{lossy}.
\autoref{fig:sparsity_patterns} also shows various tensors under different structured sparse views.

Prior work in DNN accelerators also proposed dense accelerators, unstructured sparse accelerators, 2:4 structured sparse accelerators, etc.
To clarify the nomenclatures, in this paper, \emph{if a sparsity pattern is used to describe a hardware accelerator, that accelerator should provide \textbf{lossless} and native support for any input tensor under such view.}
For example, we call Google TPU a dense accelerator and NVIDIA Sparse Tensor Core a 2:4 accelerator.
%\TK{I think I get what you mean but an example may help here. I think whats confusing is - the prev para said the view can make it lossy.}
%\TK{this is probably one of the most important lines in the paper .. but easy to missesp  .. esp as its in a background section II-A. }
%It also means that the accelerator assumes such a view of the input tensors with the sparsity pattern.
% sparse optimization -- skipping patterns
% hw constraint ISA
%the accelerator assumes a view 
%If a HW assumes a certain view X, then the HW should guarantee to provide the lossless result for any X.
% compressed

%\textbf{Compressed representations:}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.46\textwidth]{figures/different-sparsity-patterns-small.pdf}
 \vspace{-0.5em}
	\caption{Different sparsity patterns and views.
 %\TK{once we add a N:M ``view", shouldnt we add the block around the M elements?}
 }
 \vspace{-1em}
	\label{fig:sparsity_patterns}
\end{figure}
\subsection{DNN SW: Inducing sparsity in DNNs}
%\subsubsection{Sparsity in weights}
\textbf{Weight Sparsity.}
%The most popular method to introduce sparsity in DNNs is model pruning to generate weight sparsity.
%From 1980s, researchers have shown that DNN models are often overly-parameterized so that unimportant weights could be removed without causing loss of accuracy, which can reduce the size of models and the execution runtime while making the model generalize better~\cite{lecun:optimal}. 
Without a specific pattern in mind, common model pruning methods introduces unstructured sparsity in weights~\cite{SparseZoo}. 
%Unstructured sparsity is the most generic sparsity without any specific pattern in the data.
Due to the irregular accesses to handle non-zeros in unstructured sparse matrices, unstructured sparsity is not adequate for accelerating DNNs on the existing parallel hardware, such as GPUs.  

To address the issue, structured pruning forces pre-defined sparsity constraints in weights. For example, \textbf{N:M} structured sparsity~\cite{zhou2021nm,hubara2021accelerated,sun2021domino,mishra2021accelerating,fang2022algorithm,zhang2022learning,NM_training_recipe}
%\TK{add more citations -- there seem to be several N:M training recipe papers} 
ensures there are at most \textbf{N} non-zeros in each block composed of \textbf{M} consecutive elements, so the required acceleration hardware can be trivial by exploiting the regularity in sparsity patterns.
Thus, various accelerators, including recent sparse tensor cores in NVIDIA Ampere GPUs~\cite{nvidia_ampere}, target to exploit the fine-grained structured sparsity instead of unstructured sparsity.
Nonetheless, structured pruning suffers from a higher loss of accuracy~\cite{sparsegpt} than unstructured pruning since the extra pruning constraints reduce the flexibility.
This extra loss of accuracy often leads to longer fine-tuning time (e.g., repeat the whole training process again) than unstructured sparse method to recover the loss in accuracy due to pruning~\cite{mishra2021accelerating}.

%One of the major downsides of model pruning techniques, regardless of whether it is structured or unstructured, is that it often requires extra training steps to recover the loss in accuracy due to pruning~\cite{mishra2021accelerating}, with structured sparse pattern needs 

%, unless it is trained to be sparse from scratch \cite{zhou2021nm}.

%\subsubsection{Sparsity in activations}
\textbf{Activation Sparsity.}
%\PT{we can talk about activation sparsity in the self-attention block too}
Activation sparsity arises at runtime due to the non-linear activation functions such as ReLU, ReLU6~\cite{mobilenets}, and SquaredReLU~\cite{so2021primer}, which clips negative values to zero. Activation sparsity is prevalent in both conventional Convolutional Neural Networks (CNNs) and recent Transformers~\cite{li:transformer-sparsity}. Since it is intrinsic in DNN models, no extra fine-tuning or pruning steps is required to introduce activation sparsity.
%While the weight sparsity can be determined statically, 
Unlike weight sparsity, activation sparsity is dynamic as the intermediate input activation values depend on the inputs of the DNN model.
Thus, the location of non-zeros and the degree of sparsity are unpredictable, similar to unstructured pruning making it hard for structured sparse hardware to exploit input sparsity.
Another challenge is that recently proposed activation functions, such as GELU~\cite{gelu}, and Swish~\cite{ramachandran2017searching}, do not generate zero, which nullifies the benefits of exploiting activation sparsity in prior work~\cite{jang2021samsung}.


\subsection{DNN HW: Exploiting sparsity in DNNs}
\label{subsec:dnnhw}

%\subsection{Comparison of DNN HWs}
%In ~\autoref{table:nm-hw}, we summarize different DNN HWs (Dense, Unstructured Sparse, and Structured Sparse) and compare them with our work.

%As mentioned before, depending on the sparsity patterns, different sparsities can be categorized into unstructured sparse, structured sparse, and dense.
%In \autoref{fig:research-objective}, we position several sparse tensor accelerator architecture works based on their specialization.
%In \autoref{fig:sparsity_patterns}, we show three patterns, dense, unstructured sparsity, and N:M structured sparsity where N is 2 and M is 4.
%\autoref{table:nm-hw} shows the comparison of various sparse HW support. % for different DNN models.
Unstructured sparse accelerators, including SCNN \cite{parashar2017scnn}, SIGMA \cite{qin2020sigma}, Samsung NPU~\cite{jang2021samsung}, and dual-side sparse core (DSTC)~\cite{wang:dual-side} target unstructured sparsity and skip redundant computations aggressively, but they suffer from non-trivial area/power costs due to the complex indexing and reduction logic, often introducing workload imbalance problems~\cite{liu2022hpca} as well. 
For example, SIGMA \cite{qin2020sigma} introduces 38\% area overhead compared to the dense architecture due to its flexible and non-blocking distribution/reduction networks.
SCNN \cite{parashar2017scnn} and Griffin~\cite{shin2021griffin} produce 34\% and 32\% area overhead due to the support for the unstructured sparse dataflow.
%SIGMA’s key overheads are the highly flexible, non-blocking distribution and reduction networks that lead to a 37.7% area overhead.
%Samsung NPU~\cite{jang2021samsung} instead focuses on exploiting unstructured input sparsity to avoid extra training stages required to enforce weight sparsity in the target model.
Moreover, when the sparsity degree is low or zero, they provide no improvement or even degrade performance/efficiency due to the overhead for supporting unstructured sparsity \cite{highlight2023micro}.
%\input{tables/comparison3}
%Zhu et. al~\cite{zhu2019micro}
More recent structured sparse tensor accelerator architectures, such as STA \cite{liu2020sta}, Sparse Tensor Core from NVIDIA GPUs (NV-STC) \cite{nvidia_ampere}, and VEGETA \cite{jeong:vegeta}, provide HW support for structured sparsity
%\TK{no they only provide HW support for N:M structured sparsity}
with minimal area overhead.
However, these designs accelerate \textbf{only structured pruned models} with the specific pattern and focus on weight sparsity since exploiting unstructured activation sparsity without much overhead is not trivial.
%\PT{We need to have figures to provide example of structured sparsity.}
S2TA~\cite{liu2022hpca} has tried to circumvent the challenge by forcing structured sparse patterns dynamically, but it requires modifying the models and even more fine-tuning steps. %, which is not preferable for real-world deployments.
We compare different DNN HWs in \autoref{table:nm-hw}.
\input{tables/comparison4}

%\TK{given that the N:M HW is the target HW in this work, we are missing a figure explaining how N:M HW works. even logically showing a PE with a mux to pick N elements out of M .. }

%SCNN~\cite{parashar2017scnn} consumes around 30\% more energy for a dense workload.
%~\cite{shin2021griffin}.
%\PT{We need actual data to show unstructured sparsity is bad. "SCNN incur XX\% energy overdense, SIGMA introduce XX\% area over baseline, and blahblah"}
%Finally, dual-side sparse core~\cite{wang:dual-side} introduced an architecture to exploit both input and weight unstructured sparsity.

%\textbf{Our research objective of this project is to extend existing NVIDIA dense and sparse tensor cores so that they can leverage input sparsity to improve performance.}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/TASD-interface.pdf}
        \vspace{-1.5em}
	\caption{TASD Interface.
 }
        \vspace{-1em}
	\label{fig:tasd_inteface}
\end{figure}
\subsection{Tension between sparse DNN SW and HW}
\autoref{fig:tasd_inteface} shows the state of sparse DNN software and hardware. On the one hand, model developers have shown that unstructured sparsity provides better model accuracy and higher sparsity degree. On the other hand, hardware developers have shown that structured sparsity support is more practical to include in GPUs and other DNN accelerators. Such tension in the desired sparsity patterns hampers the progress in bringing sparse DNN acceleration to practice.

The main drawback of the previous hardware-specific patterns is that the pruning software and hardware support are tightly coupled, such that the software generates a model specifically pruned for the pattern supported by the hardware. For example, a model pruned for the NV-STC can only be accelerated by NV-STC, not by S2TA.
To decouple the tight relationship, we propose another layer of system software between the model developers and DNN hardware for sparsity. Our insight is to approximate a tensor by decomposing it into a series of structured sparse tensors. 
We leverage the distributive property in tensor algebra to execute the series of structured sparse GEMM. This mechanism provides an unstructured sparse interface for developers but only requires structured sparse support from hardware. As shown in \autoref{table:nm-hw}, by bridging DNN model and HW, this work is able to accelerate all types of sparsity seamlessly with a low area overhead.



%We illustrate our view in ~\autoref{fig:tasd_inteface}.
%Once we prove that TASD could achieve reasonable accuracy, we would explore HW design space to provide native TASD support.


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/3_tasd.tex <==
\section{TASD: Tensor Approximation via Structured Decomposition} 

In this section, we introduce a method to \textbf{approximate unstructured sparsity using a series of structured sparsity}, which we call \textbf{TASD}.
In this paper, we use a set of N:M structured sparsities for TASD to explain the method and show how to use it practically, but the method is general and not limited to only N:M structured sparsity.

\label{sec:tasd}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/tasd-example.pdf}
        \vspace{-1em}
	%\caption{TASD example using a 2$\times$8 matrix $A$ whose sparsity degree is 37.5\%.}
        \caption{TASD example using a 2$\times$8 matrix $A$.}
	\label{fig:tasd_example}
    \vspace{-2em}
\end{figure}

\subsection{Overview}
We use an unstructured sparse matrix $A$ to illustrate how TASD works in \autoref{fig:tasd_example}.
The matrix $A$ has 6 zero elements out of 16 total elements with a 37.5\% sparsity degree. 
Also, note that the sum of all elements in $A$ is 25.

Matrix $A$ can be rewritten as a 2:4 structured sparse matrix (a 2:4 view of $A$) plus a remaining matrix, $A_{1}^{2:4}$ and $R_1$, where $A_{1}^{2:4}$ is derived by extracting two \textbf{largest} elements out of four elements in each row in $A$ while $R_1$ is the remaining matrix (i.e. $A - A_{1}^{2:4}$) after the extraction, as shown in \autoref{ss-decomp}. 
\begin{align}
    A & = A_{1}^{2:4} + R_1 \label{ss-decomp}
\end{align}
The extracted matrix, $A_{1}^{2:4}$ covers 70\% in terms of the number of non-zero values while covering 84\% in terms of the sum of the magnitudes.
The percentage for the lost magnitudes is smaller than the percentage of the lost non-zero values because we extract two \textit{largest} elements out of four consecutive elements.
If we discard the remaining matrix $R_1$, then the original matrix $A$ can be \textit{approximated} as $A_{1}^{2:4}$.
Thus, we call this approximation, \textbf{structured decomposition}.
%and the metrics mentioned above can be used to describe how lossy the approximation is. 
If we approximate $A$ with a 3:4 pattern instead of the 2:4 pattern, we can derive matrix $A_{1}^{3:4}$ with a structured decomposition that drops only one non-zero element, covering 90\% of the number non-zeros and 96\% of the sum of total magnitudes.

Instead of using a denser N:M, we can further decompose $R_1$ using another structured pattern, such as 2:8.
$A_2$ can also be derived by extracting two largest elements out of \textbf{eight} consecutive elements in $R_1$, making $A_2$ as a 2:8 structured sparse matrix.
Similar to the previous decomposition, we call the remaining matrix $R_2$ as shown in \autoref{fig:tasd_example}.
%Instead of extracting two largest elements out of \textbf{four} consecutive elements in the remaining matrix, $B_2$ can also be derived by extracting two largest elements out of \textbf{eight} consecutive elements in the remaining matrix, making $B_2$ as a 2:8 structured sparse matrix. 
%In this case, not all elements of $B$ could be distributed across $B_1$ and $B_2$, so $B$ might not be equal to $B_1 + B_2$, but can be \textbf{approximated} as $B_1 + B_2$ as shown in \autoref{ss-decomp2}.
All elements of $A$ are covered by $A_{1}^{2:4}$ and $A_{2}^{2:8}$, so $A$ is equal to $A_{1}^{2:4} + A_{2}^{2:8}$, thus the approximation of $A$ to $A_{1}^{2:4} + A_{2}^{2:8}$ is lossless.
Since the unstructured sparse matrix is approximated using a set of structured sparse matrices, we call this method as Tensor Approximation via Structured Decomposition (TASD).

Theoretically, structured decomposition can have infinite terms. 
Below, we formalize the process more generally using different structured sparse patterns denoted as $s_i$.
%if one wants to approximate $B$ more precisely, i.e. $B_3$ can also be added by extracting two out of 16 consecutive elements (2:16) in the remaining matrix ($B - B_1 - B_2$) as shown in \autoref{ss-decomp3}, or until any $B_n$. 
\begin{align}
    A & \simeq A_1^{s_1} + A_2^{s_2} \label{ss-decomp2}\\ \label{ss-decomp3}
      & \simeq A_1^{s_1} + A_2^{s_2} + A_3^{s_3} \\ \label{ss-decomp4}
      & \simeq A_1^{s_1} + A_2^{s_2} + A_3^{s_3} ... + A_n^{s_n}
\end{align}
We call $A$ as the original matrix and $\sum A_i^{s_i}$ as \textbf{TASD series}, to draw an analogy to the classic Taylor series%
\footnote{Taylor series approximates any function with polynomials, while TASD series approximates any tensor with structured sparse tensors.}%
: Each successive term (residual structure sparse tensor) improves the accuracy of the approximation.
A TASD series configuration includes the number (``order") of TASD terms ($n$) and the structured sparsity pattern ($s_i$) for each TASD term.
Using TASD, one can generate a structured sparse view of a given tensor, and the error between the view and the original tensor would depend on the TASD series configuration.

\subsection{Using TASD for matrix multiplication}
TASD decomposes any tensor $A$ into a series of structured sparse tensors.
Decomposed tensors can be used in any tensor algebra, such as matrix multiplication ($C = A\times B$), which can be approximated as $A_1^{s_1}\times B$. If $s_1$ is 2:4, and the matrix multiplication is running on NVIDIA Sparse Tensor Cores, potentially 50\% of  Multiply-and-Accumulate (MAC) operations could be skipped.

With the distributive property of tensor algebra, matrix $A$ can be approximated using more TASD terms such as $(A_1^{s_1} + A_2^{s_2})B = A_1^{s_1}B + A_2^{s_2}B$. 
If $s_1$ is 2:4 and $s_2$ is 2:8, about 25\% of MAC operations could be skipped.
Finding the proper TASD series to minimize the error while maximizing compute reduction will determine the quality of the approximation.
We provide a detailed analysis of TASD with synthetic data in \autoref{append:additional_details}.


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/4_application.tex <==
\section{HW/SW Co-Design with TASD}
\label{sec:codesgin}
%\input{tables/potential_perf}
%\begin{figure}[!t]
%	\centering
%	\includegraphics[width=0.45\textwidth]{figures/tasd-high-level.pdf}
%	\caption{tasd-high-level. -- maybe table.. train once and get all the benefits}
%	\label{fig:tasd-high-level}
%\end{figure}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/system-overview-simple-new.pdf}
    \vspace{-0.5em}
	\caption{System overview with TASDER.}
	\label{fig:system_overview}
    \vspace{-0.5em}
\end{figure}

In \autoref{sec:tasd}, we introduce our approximation method, TASD, in general. In this section, we show how our method can be used to accelerate DNN models with sparse weights and inputs.
Although TASD can also be used to accelerate the DNN training, we focus on how to accelerate DNN inference in this work.
There are two main insights that inspired us to use TASD for DNN inference.

1) By its nature, DNN models are able to tolerate small errors in their internal computations. 

2) Although TASD is a lossy approximation method, carefully selected TASD terms can provide high-quality approximations with a limited number of non-zeros being dropped.

%\todo{Discuss and use "TCONV" for the whole section. Make the HW to be a TCONV HW and say any structured sparse HW can be a TCONV HW.}

\subsection{System architecture overview}
We introduce our optimizer system, TASDER, which takes a DNN model, sample data, target HW information including structured sparsity patterns, and hyperparameters as shown in \autoref{fig:system_overview}.
Internally, TASDER will search for the TASD configuration for each layer of the given DNN model and return the configurations.
In the following subsections, we introduce TASD-W and TASD-A, which are the methods to exploit TASD on weights and activations, respectively.
We also explain how the TASD configuration per layer is selected in our framework.
In this work, we only consider convolution (CONV) and fully-connected (FC) layers in DNN models to apply TASD as they usually consume most of the execution cycles, and they get converted to matrix multiplication operations using algorithms such as \texttt{im2col} for parallelization.
%TASD; TASD-W, TASD-I

%Outputs: TASD Group -- 
%SW/HW requirements for TASD
% Clearly state what is the assumption.
% Compiler phase
% profile guided optimized for the HW
% we can cover both dense/structured sparse

\subsection{TASD-W: Applying TASD on weights}
\label{subsec:tasd-w}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50_layer_sparsity.pdf}
        \vspace{-1em}
	\caption{Sparsity degrees for each layer in 95\% unstructured sparse ResNet50 from SparseZoo.}
	\label{fig:resnet50_layer_sparsity}
    \vspace{-1em}
\end{figure}

\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.95\textwidth]{figures/conv-spconv-tconv-wide.pdf}
        \vspace{-0em}
	\caption{Comparison of flows of an original model with a conventional CONV/FC layer and transformed models with a TCONV/TFC layer with structured sparse weights, and a TCONV/TFC/TASD layer with structured sparse activations. 
 %\TK{I was a little confused about how Figure 6 and Figure 8 gel together. Both seem to show TASDER but the outputs of TASDER seem to flow to HW in Fig 6 but seem to be within SW (say PyTorch) in Fig 8 .. this is just a high level glance, i didnt read the text describing it.}
 }
	\label{fig:conv-tconv}
    \vspace{-1em}
\end{figure*}

We expose an unstructured interface to ML model developers as the target of optimization so that they can focus on the techniques to prune their models as much as possible without considering any specific HW-friendly sparsity pattern.
Therefore, the optimization problem for TASD-W is that given the weights of DNN models as unstructured sparse tensors, use the available structured sparse HW to accelerate the model execution as much as possible. 

We assume that the target hardware can accelerate the structured sparsity patterns, $S_1, ..., S_n$.
A TASD configuration of the $i$th layer, $C_i$, is a sequence of $S$.
For a given DNN model $M$, a TASD transformation of the model, $T$, is defined as applying a sequence of $C_i$ where $C_i$ is the TASD configuration for each layer in the model.
%
Then, the target is to find a TASD transformation $T_{opt}$ for a given model where
\vspace{-0.5em}
\begin{align}
& T_{opt} = \argmin_T (Latency(M_T)) \\  %&= \{x \mid c(x) = \min_{x'} f(x')\}
& \text{such that } Accuracy(M_T) \approx {Accuracy}(M_{original}) 
\end{align}

\vspace{-0.5em}
A simple way to use TASD-W is using the same TASD configuration for all layers in  the model, i.e. applying \textbf{network-wise TASD-W}.
As the number of supported structured sparsity patterns, $n$, is not large enough, the $T_{opt}$ for network-wise TASD-W could be found with the exhaustive search.

A better method to use TASD-W is using different TASD configurations for different layers, i.e. \textbf{layer-wise TASD-W}.
The set of TASD transformations that can be covered by layer-wise TASD-W is a super-set of the TASD transformations in network-wise TASD-W. 
Usually, a pruned model with unstructured sparsity does not guarantee the same sparsity across layers, i.e. even though the overall sparsity is 95\% for the model, different layers could have different sparsity degrees as shown in \autoref{fig:resnet50_layer_sparsity}.
%there is a notable variance in sparsity degrees across different layers.
Unlike network-wise TASD-W where all the layers use the same TASD configuration, it is not straightforward how to choose a TASD configuration per layer as there could be numerous options per layer. 
To minimize the accuracy drop, it is crucial to reduce the number of dropped non-zeros after applying TASD, which would prefer conservative TASD configurations. 
On the other hand, to maximize the performance gain, it would be better to apply aggressive TASD configurations, which would be able to be translated into higher sparsity and efficiency gain. 

To address this, we design and implement a greedy-based algorithm that optimizes across all layers.
This greedy algorithm first measures the percentage of dropped non-zero elements of each TASD configuration for all layers and sorts the configuration-layer pairs by their percentage of dropped elements.
Next, it greedily applies the TASD configuration based on the sorted order until the model quality is $<$99\% of the original model (i.e., prioritize the option with the smallest dropped non-zeros). 
Since it only takes a single pass to all layers, the runtime overhead is trivial (a few seconds per model), while the extra training needed for structured sparse HW often takes hundreds of GPU hours~\cite{sun2021domino}.

We use TCONV/TFC to indicate a CONV/FC layer with TASD as shown in \autoref{fig:conv-tconv}, and the TASD configurations found above would be applied to the corresponding TCONV/TFC layers.
In \autoref{fig:conv-tconv} (a), we show how the conventional CONV/FC layer works with unstructured sparse activations (usually from ReLU) with dense weights. In \autoref{fig:conv-tconv} (b) shows how a TCONV/TFC layer works with unstructured sparse weight. 
TASDER would modify unstructured sparse weights to structured sparse weights with TASD-W.



\subsection{TASD-A: Applying TASD on activations}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/tasd-i-updated-2.pdf}
 \vspace{-1.5em}
	\caption{
 ResBlocks with CONV and TASD/TCONV and Transformer Blocks with FC and TASD/FC.}
 
	\label{fig:tasd-a}
 \vspace{-1.5em}
\end{figure}
TASD can also be applied to activations to improve a DNN execution as shown in \autoref{fig:conv-tconv} (c).
Unlike weights which are static, TASD should be applied for dynamic decomposition during the runtime as activations are dynamic. 
In \autoref{fig:tasd-a} (a) and (b), we show a baseline ResBlock and a ResBlock with TCONV and TASD layers, which decompose activation tensors with given TASD configurations. 
We add TASD layers after ReLU layers so that they can minimize the number of dropped non-zeros after approximation. 
The same can be applied to a Transformer Block, where the FC layers in the multi-layer perception module can be replaced with TFC by inserting a TASD layer before TFC layers as shown in \autoref{fig:tasd-a} (c) and (d).
Ideally, other FC layers in a Transformer Block could also be replaced with TASD and TFC layers, but empirically we found it hard to maintain the model quality.

Similar to TASD-W, the simplest way to choose a TASD configuration for each TASD layer is using network-wise TASD where all TASD configurations are same across all TASD layers. 
Assuming limited supported structured sparsity patterns from HW, only a handful number of options need to be explored.
However, similar to weights, this may not be efficient as activations from different layers show significantly different degrees of sparsity, as shown in \autoref{fig:resnet50_layer_sparsity}.

To address this issue, we again leverage layer-wise TASD as it can tailor the TASD configuration to each layer.
However, 
unlike the TASD-W,
it is not feasible to test every option for each layer to find out the best options as the target tensors (activations) are dynamically generated.
%, unlike the case of TASD-W (static weights). 
%due to the combinatorial explosion.
%To choose a TASD configuration for each layer, we use a sparsity-based TASD selection method instead of the non-zero-based method for TASD-W.
%that we introduced in \autoref{subsec:tasd-w}.
We find that a small set of calibration dataset (e.g., 1000 images for ImageNet~\cite{deng2009imagenet}) can provide enough insights. 
As shown in \autoref{fig:resnet50_layer_sparsity}, while different layers have different sparsity degrees, for a particular layer, the activation sparsity degree remains in a small range across different input images.
Therefore, TASDER takes calibration data as an input, so it can profile the given DNN model with the calibration data and collect the statistics (e.g., average, 99th percentile) about activation sparsity per layer. 

To choose a TASD-A configuration for each layer, we use a \emph{sparsity-based} selection method, instead of the dropped-non-zero-based method for TASD-W.
We use a hyperparameter, $\alpha$, to tune the aggressiveness of the TASD approximation. 
For a given layer $L_i$ and the available configurations in the target HW (e.g., $H_1, ... , H_4$), we choose $C_i$ as $H_j$ where $j$ is the largest integer where $S(L_i) + \alpha > H_j$.
If we use a larger $\alpha$, we choose the TASD configuration more aggressively (i.e. allowing more dropped non-zeros). 

%We summarize the algorithm in \autoref{lst:tasd}.
%\vspace{-1em}
%\input{algorithms/find_config}



\textbf{Beyond sparsity: Supporting non-ReLU-based DNNs.}
%ReLU-based DNNs naturally induce sparsity in activation tensors, so by collecting the sparsity statistics, TASD-A can find the appropriate configuration for each layer. 
%However, 
For better accuracy, state-of-the-art DNNs have replaced ReLU with other activation functions, such as GeLU \cite{gelu} and Swish~\cite{ramachandran2017searching}, which do not induce any sparsity in activations making the activations dense.
Thus, our sparsity-degree-based TASD selection to choose TASD configuration for TASD-A for each layer would not work for those DNNs.

\begin{table}[t]
\small
\caption{Supported sparse patterns with TTC-VEGETA.}
%\vspace{-1em}
\begin{center}
\begin{tabular}{cc|cc}
{\bf Pattern} & {\bf TASD series} & {\bf Pattern} & {\bf TASD series}\\
\hline
1:8 & 1:8 & 5:8 & 4:8 + 1:8\\
2:8 & 2:8 & 6:8 & 4:8 + 2:8\\
3:8 & 2:8 + 1:8 & 7:8 & - \\
4:8 & 4:8  & 8:8 & Dense\\

\end{tabular}
\label{tab-ttc-vegeta}
\end{center}
\vspace{-1em}
\end{table}

%(\autoref{lst:tasd})
To address this, we investigate the distribution of the magnitude of all elements in the activation tensors from GeLU/Swish-based DNN.
%as shown in \autoref{fig:tasd-pseudo-density}. 
We found that, while no element in the tensor is exactly zero, a huge number of elements have tiny magnitude, compared to the range of magnitude for all elements. Therefore, we let TASD-A leverage this skewed distribution and collect the magnitude statistics. We introduce another heuristic, \emph{pseudo-density}, which aims to preserve a fixed percentage (e.g., 99\%) of the sum of all elements in a tensor, to determine the best TASD configuration for every layer.
Using the pseudo-density for the non-ReLU-based DNNs, we can use the same sparsity-degree-based method 
%(\autoref{lst:tasd}) 
%that we proposed in \autoref{subsec:tasd-w} 
(i.e. by replacing \textit{sparsity} to \textit{1 - pseudo-density}). The approximating nature of TASD allows the system to also accelerate non-ReLU-based DNNs, while prior work that specifically targets activation sparsity cannot.

% TODO; Challenge of sparse activation
% random dropping / magnitude dropping ...
% magnitude based selection
% pseudo-sparsity
% define approximated sparsity
% Sparse BERT; sparse - dense act
% Dense BERT; dense - dense act

% ResNet50 sparseloop
% TASD-W for BERT-Base/ accuracy
% BERT-Base sparse using sparseloop
% BERT-Base dense using sparseloop
% qkv projection FF1 FF2

%In this section, we introduce how to use TASD to exploit input sparsity in DNNs. 
%The key intuitions are that 1) Input activations in each layer of a DNN already have many zeros 2) TASD configurations  3) Dropping a small number of non-zeros by approximation could be tolerable in terms of the accuracy of a DNN model. 
%Thus, we apply TASD on input activations in each layer of the target DNN.
%One can apply extreme [1:8] to the input activations of all layers, which could be able to achieve 8$\times$ reduction in terms of the number of required MAC operations, but this would lose many non-zero values, thus incurring significant accuracy drop. 
%A good TASD configuration should be able to decompose $B$ using a small number of sparse $B_i$ without losing a high number of zeros.
%If we apply good TASD configurations to all layers, we should be able to achieve reduced computation while maintaining the original accuracy.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-hw-overview-simple-new.pdf}
  \vspace{-1em}
	\caption{TASD-HW composed of four TTCs. 
 %\TK{I presume RF MAC etc is basically plug and play for different N:M accelerators (STC/VEGETA etc) .. might be good to just show a box called "N:M Accelerator" or sthg and expan it out to show the RF/MAC etc}
 }
	\label{fig:tasd-hw}
 \vspace{-1em}
\end{figure}
\subsection{Structured sparse HW for TASD}
TASD works best when there are at least a few supported structured sparse patterns in the target sparse accelerator. While the TASDER optimizer is HW-agnostic, we propose to build on top of a recently proposed flexible structured sparse tensor accelerator to maximize the benefit.
Inspired by previous structured sparse accelerators~\cite{nvidia_ampere,liu2021s2ta,jeong:vegeta}, we introduce TASD Tensor Core (TTC).
We adopt a design similar to VEGETA~\cite{jeong:vegeta} engine composed of multiple processing elements (PEs) while providing support for 1:8, 2:8, and 4:8 structured sparse patterns, and we call it TTC-VEGETA.
With TASD and a limit of up to 2 terms, a TTC-VEGETA engine can support 7
out of all the N:8 patterns 
%\footnote{The 7:8 pattern needs 3 TASD terms and is rarely used in practice.}%
as shown in \autoref{tab-ttc-vegeta} even though the original VEGETA supports only three sparse patterns.
Note that TTC can adopt other structured sparse designs, such as STC~\cite{zhu2019micro} with supports for 2:4 and dense, which we call TTC-STC. 
This would limit the flexibility in approximation using TASD compared to VEGETA-based TTC design, but TASDER is still able to optimize some layers. 
We explore the benefit of flexibility in \autoref{sec:eval}.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-flow.pdf}
    \vspace{-1em}
	\caption{Dataflow between PE array and TASD units.}
	\label{fig:tasd-flow}
    \vspace{-2em}
\end{figure}


In \autoref{fig:tasd-hw}, we show the overall design of a TASD HW composed of four TTCs similar to the one used in the previous work \cite{wu2022sparseloop}.
%\todo{walk throught the design}
The modification we add on top of the N:M accelerator, such as STC or VEGETA, is the TASD unit (shown in the right part of \autoref{fig:tasd-hw}) that dynamically extracts TASD terms from the activation tensor, similar to the DAP unit in S2TA~\cite{liu2022hpca}.
TASD-W can be applied offline through pre-processing since weights do not change during runtime, but TASD-A requires the TASD unit as activations will be dynamically generated at runtime.

Given the computation latency on TTCs, the minimum number of TASD units per TTC to hide the latency of TASD units depends on the mapping and TTC implementations.
%that we describe in the following. 
For example, each TTC-VEGETA with M=8 generates 16 (number of PE columns in each TTC) output elements per cycle (i.e. 2 blocks per cycle) as shown in \autoref{fig:tasd-flow}, which will be fed to TASD units. 
For an M-element block, a TASD unit sequentially extracts the largest values, so the decomposition takes up to M cycles %for any TASD configuration 
as the sum of Ns in a TASD configuration cannot be larger than M.


The example in \autoref{fig:tasd-flow} uses TASD configuration composed of 4:8 and 1:8, so it takes 5 cycles per block. 
At T1 (cycle 1), two blocks (Blk-1, Blk-2) will be produced from the PE array, and Blk-1 and Blk-2 will be processed by TASD Unit 1 and TASD Unit 2, respectively (each cycle, two TASD units start execution). 
During T2-T5, Blk-1 and Blk-2 will be used to extract Decomposed Blocks, DBlk-1 and DBlk-2 for 4:8 Tiles.
Then, during T6, DBlk-1 and DBlk-2 for 1:8 Tiles will be generated and stored. The decomposed blocks will be used as the inputs of the next layer.
With 16 TASD units, a TTC-VEGETA can operate without stalls on the PE array due to the decomposition as a TASD unit is always guaranteed to be available after M cycles (i.e. by Little's law, $16 = 2\times8$). 
%TODO ADD a sentence that DB will be used.
We present the area overhead for TASD units in \autoref{sec:eval}.
%How this is used to split a tensor into two? I can imagine that you sequentially output the largest values, and cut off the first 4 (out of 8) for a 4:8 term, and then the next 2 for a 2:8 term, etc. Such sequential execution seems to have very low throughput. How many such TASD units are needed then? What is the ratio between number of MAC units and number of TASD units to achieve a balanced throughput? The evaluation only mentions a 2% area overhead in 5.5 without any details.

%From our synthesis result, the area of a PE-M8 and TASD-M8 is 241um^2 and 88um^2 each. Considering the PE to TASD ratio (256:16), the area overhead of TASD on top of PEs is 88*16/241*256 = 2.3\%. To understand the impact of different M in terms of overhead, we also synthesized for different Ms (4 and 16), and observed 1.3\% and 3.4\% area overhead, respectively.


% I may need to fix the following
% The current arch file assumes
% LRF/PE holds A
% RF only holds C
% SMEM holds B
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-hw-mapping-simple.pdf}
 \vspace{-1em}
	\caption{A mapping of matrix multiplication on TTCs.
 }
    \vspace{-1em}
	\label{fig:tasd-mapping}
\end{figure}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/sparseloop_results.pdf}
    \vspace{-0.5em}
    \caption{
    Energy-delay-products for running dense and sparse ResNet50 and BERT. For TTC-STC and TTC-VEGETA, we use the TASD transformations found from TASDER.
    %and DNN layers assuming the VEGETA engines frequency as 0.5GHz.
    M4/M8 represents design with N:4/N:8 supports.
    }
    \vspace{0.5em}
    \label{fig:dense_sparse_comparison}
\end{figure*}
\textbf{Decomposition-aware dataflow.}
In \autoref{fig:tasd-mapping}, we show a mapping of a matrix multiplication with an approximated matrix A using a TASD configuration, 4:8 and 1:8 for the TTC.
We first show how we tile the matrices and how they are mapped in the private register file and shared buffer of each TTC.
When matrix $A$ is decomposed into two TASD terms, $A_1$, and $A_2$, the original matrix multiplication can be approximated as the sum of the two matrix multiplications and accumulation ($A_1\times B + A_2\times B$). 
As the two matrix operations share the same input $B$ and partial sum $C$, we \textbf{keep B tiles in the L2 Scratchpad Memory (SMEM) and C tiles stationary in the L1 SMEM} of TTC while changing decomposed A tiles to temporally reuse B and C tiles for data reuse (between timestep 1 and 2, timestep 3 and 4 in ~\autoref{fig:tasd-mapping} (b)).
For each accelerator tile, (i.e. for each timestep), we \textbf{keep each element of A tile stationary in the register file of each PE} for the temporal reuse, while the B and C elements are mapped correspondingly. 
By increasing the tile size for GEMM-N dimension, the reuse count for A tile at PE level could increase, which is limited by the size of the capacity of each SMEM.
We swap C tiles at the very end to minimize the number of write-back operations to other levels.
Although we maximize reuses for decomposed tiles, there is still unavoidable overhead such as reading C tiles again, but this is insignificant compared to the energy saving by skipping ineffectual computations using TASD.
In \autoref{subsec:energy_breakdown}, we quantify the energy overhead.

%Using the proposed accelerator, we show a mapping .

%Intuitively, it would be better to use a greedy approach which would allow $B_j$ be more important than $B_k$ if $j < k$.

% theoritical numbers for running 8:8 using 1:8
%  4 8 16?
% 1 : 16

% 2:4
% 2:4, 2:8
% 2:4, 2:8, 1:8

% 2:4
% 2:4, 2:8 --> 4:8, 2:8 == 6:8
% 2:4, 2:8, 1:8 --> 4:8, 2:8, 1:8
% 2^n : 2^m with fixed m
% use TASD


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/5_eval.tex <==





\section{Evaluation}
\label{sec:eval}
\subsection{Methodology}



TASD accelerates both sparse and dense DNNs \textit{without fine-tuning}, so we evaluate TASD-W on sparse DNNs from SparseZoo~\cite{SparseZoo} and TASD-A on dense DNNs from TorchVision~\cite{torchvision}.
We use a classic convolutional network, ResNet50~\cite{he2016resnet}, and a transformer-based network, BERT~\cite{devlin-etal-2019-bert}.  %to illustrate detailed trade-offs between accuracy and performance.
For the baseline HW, we compare against dense tensor core (TC)~\cite{nvidia_ampere} and dual-side sparse tensor core (DSTC)~\cite{wang:dual-side} as representative dense and unstructured sparse accelerators.
We configure these baselines as in the Sparseloop Artifacts~\cite{sparseloop-artifact}.
We use 4 variants of TTC, based on STC and VEGETA with N:4 and N:8 designs, to show the extra benefits of TASD from the flexibility of the structured sparse hardware as summarized in \autoref{tab:hw}.
%(TTC-STC-M4, TTC-STC-M8, TTC-VEGETA-M4, TTC-VEGETA-M8).
All designs use the same memory hierarchy and the same amount of PEs (MACs) to ensure a fair comparison.
We clarify that we do not exploit both sparsities concurrently for skipping computations. We either use TASD-W or TASD-A depending on the workloads since supporting both sparsities requires non-trivial area/energy costs~\cite{wu2021sparseloop, highlight2023micro} and is not compatible to approximate with TASD.

%We use one of the most popular DNN, ResNet50 (both dense and pruned with 95\% unstructured sparsity) 


%To evaluate the effectiveness of TASD methods on accelerators, 
We develop TASDER as a framework to search for TASD transformations and calculate the accuracy of the model with each TASD transformation using PyTorch~\cite{paszke2019pytorch}. 
Following the requirement in MLPerf~\cite{mlperf} inference benchmark, we only consider a model as valid with TASD \textit{if the model achieves an accuracy higher than 99\% of the accuracy of the original model.}
%For TASD-A, we randomly pick 0.1\% of the data for calibration.
Next, we run each DNN layer with the given TASD series configuration using Sparseloop~\cite{wu2022sparseloop}, a sparse accelerator modeling framework to obtain per-layer results and aggregate the results for the entire network, which is consistent with prior accelerator simulation frameworks~\cite{timeloop, cosa, maestro, zigzag, scale-sim}. Sparseloop estimates the performance and energy consumption of the given HW by analyzing data movements across different memory hierarchy levels and processing elements, and actual computation based on the given dataflow. 
\textbf{We simulate all layers in the networks (marked as ``Overall")}, but to show per-layer results additionally, we choose three representative layers (from early, mid, late) as shown in \autoref{tab:workload}.
%In \autoref{tab:hw} and \autoref{tab:workload}, we show specific HW designs and target workload configurations used in \autoref{sec:eval}.

%%%% Tables
\begin{small}
\begin{table}[t]

%\small
\begin{center}
\small

\caption{Summary of different HW designs. TASD 1T and 2T indicates using TASD 1 term and 2 terms, respectively.
}
\vspace{1em}
\begin{tabular}{c|c}
{\bf HW Design} & {\bf Sparsity Support from HW} \\
\hline
\hline
TC  & None  \\
\hline
DSTC & Unstructured \\
\hline
%\cline{1-3}
TTC-STC-M4 & 2:4 (TASD 1T) \\               
\hline
TTC-STC-M8 & 4:8 (TASD 1T) \\
\hline
TTC-VEGETA-M4 & 
\begin{tabular}[c]{@{}c@{}}1:4, 2:4 (TASD 1T) \\ + 3:4 (TASD 2T)\end{tabular} 
  \\
\hline
TTC-VEGETA-M8 
&\begin{tabular}[c]{@{}c@{}}1:8, 2:8, 4:8 (TASD 1T) \\ + 3:8, 5:8, 6:8 (TASD 2T)\end{tabular}  

\end{tabular}

\label{tab:hw}
\end{center}
\end{table}
\end{small}


\begin{small}
\begin{table}[t]
%\small
\begin{center}
\footnotesize

\caption{Representative layers from the target workloads. L1, L2, and L3 are representative layers. RN and Act. refer to ResNet and Activation, respectively.
%We use ``Overall" for the entire network. 
%Sp: Sparse, D: Dense. Wgt: Weights. Act: Activations. %\TK{I initially thought L1, L2 and L3 are layers 1, 2 and 3 .. but seems like they are some other representative ones. Why not explicitly mention which layer it is? Eg L4, L31, L40 ..}
}
\begin{tabular}{c|c|c|c}
{\bf Model} &{\bf Weight}& {\bf Act.} & {\bf Layers Dimensions}\\
\hline
\hline   

\begin{tabular}[c]{@{}c@{}}Dense RN50 \\ (ReLU-based)\end{tabular}     &Dense& Sparse & 
\begin{tabular}[c]{@{}c@{}}L1: M784-N128-K1152 \\ L2: M3136-N64-K576\end{tabular}
\\
\cline{1-3}
Sparse RN50 &Sparse& Sparse & L3: M196-K2304-N256 \\
    
\hline
\begin{tabular}[c]{@{}c@{}}Dense BERT \\ (GeLU-based)\end{tabular}     &Dense& Dense & 
\begin{tabular}[c]{@{}c@{}}L1: M768-N128-K768 \\ L2: M3072-N128-K768\end{tabular}
\\
\cline{1-3}
Sparse BERT &Sparse& Dense & L3: M768-N128-K3072 \\




\end{tabular}

\label{tab:workload}
\end{center}
\end{table}
\end{small}
%\section{Experiments Settings}

We use energy-delay product (EDP), latency, and energy for the metrics. We also provide additional experiment results on the theoretical MACs reductions for other various DNNs, comparison against structured sparse accelerators, and TASD on a real system.
%in \autoref{append:additional_experiments}.

%To show the applicability of TASD for other sparse and dense DNNs, we evaluate the MACs reductions for 8 DNNs, similar to prior work in pruning for structured sparse patterns~\cite{chmiel2022optimal,sun2021domino}.


%First, we show the impact of applying different TASD configurations, both network-wise and layer-wise, on the DNN accuracy.
%Fine-tuning can be used for the target TASD configurations to regain lost accuracy, but we have not assumed that as it will add extra training costs.

%show preliminary results of a few experiments to estimate the potential of TASD to leverage input sparsity in DNN inferences.


\subsection{DNN acceleration with TASD}


\autoref{fig:dense_sparse_comparison} shows the EDP for the 4 workloads on various DNN accelerators, normalized to the dense TC.
Even though DSTC is able to exploit unstructured sparsity, the overhead of unstructured sparse acceleration (such as accessing accumulation buffer frequently) offsets the benefit and even outweighs the benefits when the workload has only one sparse operand or there is no sparse operand, causing 12\% and 167\% \textbf{larger} EDP for dense ResNet50 and dense BERT while reducing EDP by 55\% for sparse BERT.
DSTC works best for sparse ResNet50 and improves EDP by 87\%, as both weight and activation tensors are unstructured sparse with a high sparsity degree (95\% sparse weight).
%with expensive gather-scatter operations. 
Overall, it is able to reduce EDP by 35\% across all workloads on average.
%\footnote{For the conservative evaluation, we assume 2$\times$ L1 SMEM bandwidth for DSTC compared to TTC.}
%TTC only required 4$\times$. 
%while costing 30-40\% area overhead as discussed in \autoref{subsec:dnnhw}
%}.

%DSTC works best for sparse ResNet50 and improves EDP by 87\%, as both weight and activation tensors are unstructured sparse with a high sparsity degree (95\% sparse weight) only if L1 SMEM bandwidth is large enough (). 
%Moreover, 
%(55\% for sparse BERT)

Unlike DSTC, TASD-based TTC accelerators improve EDP over the TC baseline for all workloads. 
With the flexibility in sparsity patterns, TTC-VEGETA-M8 improves EDP for all workloads, by 58\%/61\% for dense ResNet50/BERT and 83\%/82\% for sparse ResNet50/BERT. 
Even with a single fixed pattern, TTC-STC-M4 improves by 4\%/32\% for dense ResNet50/BERT and 49\%/53\% for sparse ResNet50/BERT. 
This result shows that TASD can effectively leverage structured sparse hardware for off-the-shelf dense and sparse DNNs with no fine-tuning, and the extra flexibility (increasing M) in the baseline accelerator increases the benefit.



\autoref{fig:overall_energy_latency_edp} provides end-to-end latency and energy consumption for various designs. TTC-VEGETA-M8 is the most energy-efficient across all workloads and is slightly slower than DSTC only for sparse ResNet50. % (by 22\%). 
This result shows TASD provides a better overall tradeoff than unstructured sparse accelerators, considering their high area overheads.










 
\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/overall_energy_latency_edp.pdf}
        \vspace{-3em}
	\caption{
        Latency and energy for various designs.
 }
        %\vspace{-0.5em}
	\label{fig:overall_energy_latency_edp}
 \end{figure}

  \begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/resnet50-95-networkwise-w.pdf}
 	\includegraphics[width=0.49\textwidth]{figures/resnet50-95-networkwise-a.pdf}
        \vspace{-1em}
	\caption{
Network-wise and Layer-wise TASD on ResNet50. Upper: TASD-W. Lower: TASD-A.
 }
        \vspace{-1em}
	\label{fig:resnet50-95-networkwise-w}
\end{figure}
%\subsection{Analysis of TASD-W on sparse DNNs} 
\subsection{Analysis of TASD} 
%\vspace{-1mm}
%To understand the impact of TASD on accuracies of DNN models, we implement TASDER using PyTorch~\cite{paszke2019pytorch} and conducted experiments for both TASD-W and TASD-A.
%\subsubsection{Network-wise vs. layer-wise TASD}
\paragraph{Network-wise vs. layer-wise TASD.}
The upper plot of \autoref{fig:resnet50-95-networkwise-w} shows the impact of network-wise TASD-W on the top-1 accuracy of unstructured sparse ResNet50 (95\% sparsity).
We applied network-wise TASD-W with N:4, N:8, and N:16 structured sparsities. 
For example, the network-wise TASD-W with 2:4 uses one TASD term with the 2:4 pattern to the weights of all convolution and fully-connected layers in the sparse ResNet50. 
Since TASD is a lossy method, aggressive TASD series approximation can result in a notable accuracy drop.
Among different N:4, N:8, N:16 options, we found that 3:4, 5:8, 10:16 is the most aggressive approximation among the available options while meeting the 99\% accuracy requirement. 
Especially, using network-wise TASD-W 5:8 (4:8 + 1:8 for TTC-VEGETA) and gating the compute units for sparse activations, compared to the dense baseline, we observe it achieves 24\% and 53\% reduction in cycle and energy respectively, thus reducing 75\% EDP for Sparse ResNet50. 

%networkwise 5:8
%energy,,,0.472,,,,,,
%cycles,,,0.7579,,,,,,
%edp,,,0.2493,,,,,,

%layerwise G 0.35
%energy,,,0.4136,,,,,,
%cycles,,,0.5891,,,,,,
%edp,,,0.2053,,,,,,

%\subsubsection{Layer-wise TASD-W on sparse ResNet50}

Using different TASD series configurations for different layers is more effective as it can adjust the aggressiveness for each layer. 
To choose a TASD configuration per layer, we use the sparsity-based selection method that we introduce in \autoref{sec:codesgin}. %\autoref{subsec:tasd-w}. 
By changing the hyperparameter, alpha, we are able to adjust the aggressiveness of our approximation method.
%We show how the top-1 accuracy and the dropped number of non-zero percentage changes with varying alphas in \autoref{fig:resnet50-95-layerwise-w}.
As layer-wise TASD-W can be adaptive to each layer, the overall approximation can be applied more aggressively.
As a result, compared to the dense baseline, we observe 47\% and 61\% reduction in energy and cycle, respectively, thus reducing 83\% EDP for Sparse ResNet50 as shown in \autoref{fig:dense_sparse_comparison}.


%\subsection{Analysis of TASD-A on dense DNNs} 
%{'cycles': {'TASD-L':0.77 3690167}, 'energy_pJ': {'TASD-L':0.70 6021474651.840003}, 'edp': {'TASD-L':0.42 389056984145620.25}, 'utilization': {'TASD-L': 82.015625}}
%TC-RF2x-24-bandwidth 1.0 4777536
%energy_pJ TC-RF2x-24-bandwidth 1.0 8593036953.436165
%edp TC-RF2x-24-bandwidth 1.0 917293317143056.9
%\subsubsection{Network-wise TASD-A on dense ResNet50}
In the lower plot of \autoref{fig:resnet50-95-networkwise-w}, we show the top-1 accuracy when network-wise and layer-wise TASD-A is applied with different TASD series.
Similar to TASD-W, layer-wise TASD-A is more effective than network-wise TASD-A.
However, the accuracy loss due to approximation shows up with a much smaller approximated sparsity.
As shown earlier in ~\autoref{fig:resnet50_layer_sparsity}, the sparsity degree is larger in weights compared to that in activations for sparse ResNet50.
Thus, the same TASD series drops a larger portion of non-zeros in TASD-A than TASD-W, incurring a higher loss of accuracy.

%\subsubsection{Layer-wise TASD-A on dense ResNet50}

%\autoref{fig:resnet50-95-networkwise-a} shows a similar trend compared to the result of the layer-wise TASD-W on sparse ResNet50.
%With the same approximated sparsity, TASD-A gives lower accuracy while being more tolerant in terms of dropping non-zeros. 
%It is because the sparse weight in ResNet50 is a result of aggresive pruning, so each remaining element is more valuable than the dense model.
%Using the most sparse configuration which meets the requirement, we observe 30\% and 23\% reduction in energy and cycle respectively, thus reducing 58\% EDP, compared to the dense baseline.
%Compared to the dense baseline, we observe 30\% and 23\% reduction in energy and cycle respectively, thus reducing 58\% EDP. 
%\subsubsection{Impact of TASD on more DNN models} 




 



\subsection{
Energy and area overhead due to TASD
}
\label{subsec:energy_breakdown}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth,]{mlsys2025style/figures/energy_breakdown_update.png}
        \vspace{-1.5em}
	\caption{
        Energy Breakdown: TTC vs. Dense TC.}
        \vspace{-0.5em}
        
	\label{fig:energy_breakdown}
 \end{figure}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/sparse-resnet34-rtx3080-tasd-w.pdf}
	        \vspace{-0.5em}
    \caption{
        TASD-W on NVIDIA RTX3080 GPU with Sparse ResNet34.}
        \vspace{-0.5em}
	\label{fig:gpueval}
 \end{figure}
 
\autoref{fig:energy_breakdown} shows the energy breakdown for a representative layer from sparse ResNet50 for dense TC and TTC-VEGETA with a TASD configuration of 4:8+1:8. TTC-VEGETA exploits sparsity and saves energy at all levels of the architecture, which saves 55\% energy over the dense TC. Moreover, the decomposition-aware dataflow in \autoref{sec:codesgin} minimizes decomposition overheads by accessing the RF (with C reuse) and SMEM (with B reuse) instead of accessing DRAM.
%\subsection{Area overhead of the TASD unit}

We measured the area overhead to support TASD on top of the existing structured sparse HW (the TASD units) through RTL prototyping and synthesis with Nangate 15nm Technology Library. We observe up to 2\% of the area for all PEs as TASD units are composed of simple comparator trees.


\subsection{Using TASD on a real system}
To validate the effectiveness of TASD, we evaluate TASD on a real system.
%we apply TASD-W to the unstructured sparse ResNet34 model from SparseZoo \cite{SparseZoo} and run it with NVIDIA TensorRT 8.5.0 on an NVIDIA RTX3080 GPU.
First, we use our framework, TASDER, to find the TASD-W configuration that meets the accuracy constraint with an unstructured sparse ResNet34 model from SparseZoo \cite{SparseZoo}. For the accuracy evaluation, we use ImageNet as the dataset. Next, we export the model using ONNX format. 
To properly measure the inference latency of DNNs exported with ONNX format, we use TensorRT, the state-of-the-art deep learning inference runtime maintained by NVIDIA. We build TensorRT engines for both the baseline model and the model with TASD-W exported in the previous step. Finally, we execute the engine with (3, 224, 224) inputs, with a batch size of 32-128, and measure the latency for each model. We achieved 28\%/39\% speed-up compared to the dense model execution with 0.9\%/1.5\% accuracy drop as shown in \autoref{fig:gpueval}. We also evaluated TASD-W with ResNet50, ResNet101, BERT, and observed up to 25\% speed-up.

%by applying TASD with \textbf{the same TASD configuration} on the input tensors of all convolution layers except the first convolution layer in the pretrained models (AlexNet~\cite{krizhevsky2012alexnet} and ResNet18~\cite{he2016resnet}) during inference. 

%We enforced the structured sparsity to the channel dimension of the tensors.
%We used 1,000 images from the ImageNet~\cite{deng2009imagenet} validation dataset.
%\input{tables/alexnet_results.tex}
%\input{tables/resnet_results.tex}

%In \autoref{table:alexnet_results} and \autoref{table:resnet_results}, we show the Top 1/Top 5 accuracies, a percentage of the number of pruned (dropped) non-zeros, and potential speedup for each TASD configurations and the base pre-trained model. 
%Potential speedup is calculated based on the total effectual computations of convolution layers compared to the base case (dense).
%These preliminary results show that using some TASD configurations could achieve comparable accuracies to the base model, which is encouraging for this direction.
%Still, there are a few things to consider carefully to validate the idea of TASD.
%Since we applied TASD right after ReLU layers instead of right before convolution layers, the numbers would be different when we apply TASD right before convolution layers.
%First, the overhead of applying TASD is not estimated yet, which could harm the overall potential speedup.
%Also, how to support and schedule multiple TASD configurations in tensor cores has not been explained.
%Next, deeper and larger recent DNN models using different activation functions could behave differently.
%Finally, different layers can prefer different TASD configurations and a layer-dependent decomposition scheme might achieve a better trade-off between accuracy and speedup.
%since different layers exhibit different input activation sparsities.




==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/6_related_work.tex <==
\section{Related Work}
\subsection{SW techniques for structured sparse HW}
%Since the structured sparse (2:4) accelerator is available in off-the-shelf NVIDIA GPUs with Ampere~\cite{nvidia_ampere} and Hopper~\cite{nvidia_hopper} architecture,
%ample work has focused on exploiting structured sparse acceleration for DNNs.

\textbf{Solutions with fine-tuning.}
DominoSearch \cite{sun2021domino} proposed a method to find layer-wise N:M sparsity during training. 
Optimal N:M~\cite{chmiel2022optimal} enforces the structured pattern during training and applies the structured pattern to input activations.
This line of work is orthogonal to our work as we focus on approximating unstructured sparsity without fine-tuning.
%We can also fine-tune DNNs with TASD series configurations and adopt the above approaches.
Fine-tuning will increase the benefit of TASD, as more aggressive approximation can now maintain the same model accuracy. 
Doping~\cite{thakker2021doping} uses an extremely sparse matrix in addition to a compressed matrix derived from Kronecker products to improve the quality of the model, but unlike TASD, it uses the extra extremely sparse matrix to give additional freedom during the training.
%, not for the approximating the given sparse matrix.

\textbf{Solutions without fine-tuning.}
SparseTIR~\cite{ye2023sparsetir} introduces composable formats and transformations for sparse compilation of DL workloads.
%, which also exploits the distributive property to effectively decompose any sparse tensor algebra into multiple well-optimized sparse GPU kernels.
However, they have not considered approximating sparse tensors and accelerating DNNs using structured sparse hardware. Another work~\cite{pool2021channel} shows permuting channels in the weight tensors can recover accuracy easily when training N:M sparse networks. 
%The work also briefly explored turning unstructured sparse models into 2:4 structured sparse models with channel permutations.
TASD is compatible with channel permutation, and we believe combining these two orthogonal techniques will further improve the accuracy of decomposed models with approximation.

\subsection{HW support for sparse DNNs}
%Meanwhile, extensive work has focused on exploiting sparsity in DNNs through specialized HW acceleration.

\textbf{Sparsity support for DNN inference.}
Different architectures have been proposed to support for weight sparsity~\cite{eyerissv2, nvidia_ampere, rasa, eureka2023micro},
for activation sparsity~\cite{jang2021samsung},
and more recently, for both~\cite{wang:dual-side, rmstc2023micro, highlight2023micro}.
%As mentioned earlier, these accelerators can be broadly classified as structured sparse or unstructured sparse HW. 
As mentioned earlier, unstructured sparse HW provides native support for any sparsity pattern but is more costly to build; structured sparse HW is efficient but requires model fine-tuning.
TASD bridges the gap by providing an unstructured sparse interface while only requiring structured sparse HW.

\textbf{Sparsity support for DNN training.}
Since weight tensors are mostly dense during training, prior work has focused on activation and gradient sparsity during DNN training.
A simpler support is to compress sparse activation and gradient, such as CompressDMA~\cite{rhu2018cdma} and ZComp~\cite{akin2019zcomp}. These techniques save data movements and memory requirements, but not overall compute.
The more complex techniques target reducing computation during training, such as TensorDash~\cite{mahmoud2020tensordash} and SAVE~\cite{gong2020save}. However, they need to give up data movement savings for better support for sparse tensor transposition during training.
TASD can potentially be used to approximate sparse activations and gradients, but we leave this to future work. 
%As prior work~\cite{li2022large, rhu2018cdma} has shown that the degree of activation and gradient sparsity stays stable, TASD-A can approximate these dynamic tensors during runtime to enable the efficient structured sparse HW support for sparse training. We leave this to future work.

%OFA ...
%\begin{itemize}
%    \item Add more works related to weight sparsity
%    \item Add more works related to input sparsity
%    \item Add more works related to converting unstructured to structured
%    \item Add more works on sparse HW
%    
%\end{itemize}

==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/7_conclusion.tex <==
% Conv/FF -> GEMM
% Inference
% Define Approximated sparsity
% 2 TASD terms -> 1:8 to 6:8
% small value distribution for GELU
% figure 8; across images

% 4 workloads representative layers
% dense resnet50/bert
% spares resnset50/bert


\section{Conclusion}
%Exploiting sparsity is a promising area to improve DNN efficiency. 
%However, 
Sparse DNN model developers prefer to induce unstructured sparsity for expressibility, while sparse DNN hardware designers prefer to support structured sparsity for HW efficiency.
This mismatch of the desired sparsity pattern 
between different parties
prevents sparse DNN acceleration from being widely adopted in practice.
To close the gap,
%between sparse DNN models and hardware,
we introduce TASD, a method that approximates an unstructured sparse tensor with a series of structured sparse tensors.
Next, we propose a framework, TASDER, which finds TASD configuration for each DNN layer
% to apply TASD
to accelerate sparse and dense DNNs.
To maximize the benefit of TASD,
we propose a simple architectural extension and dataflow on top of structured sparse accelerators.
%We evaluate TASD across DNN workloads to show TASD enables pragmatic sparse DNN acceleration.
%For four different DNNs,
TASD improves EDP up to 83\% and 74\% on average, while maintaining 99\% of the model accuracy without any fine-tuning.
We also show it achieves up to 39\% performance improvement on a real system evaluation.
    



%~\ref{sample-table}.


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/sections/backups.tex <==
%%%%
\subsection{Search algorithm for TASD selection}
\begin{algorithm}[tb]
   \caption{TASD Selection Algorithm}
   \label{alg:tasd_sel}
\begin{algorithmic}
   \STATE {\bfseries Input:} $target\_sparsity$, $alpha$, $H$
   \STATE $target\_sparsity = sparsity + alpha$
   \IF{$target\_sparsity > H[3]$}
   \STATE return $H[3]$
   \ENDIF
   \IF{$target\_sparsity > H[2]$}
   \STATE return $H[2]$
   \ENDIF
   \IF{$target\_sparsity > H[1]$}
   \STATE return $H[1]$
   \ENDIF
   \IF{$target\_sparsity > H[0]$}
   \STATE return $H[0]$
   \ENDIF
\end{algorithmic}
\end{algorithm}

In \autoref{alg:tasd_sel}, we show the sparsity-degree-based TASD Selection algorithm explained in \autoref{subsec:tasd-w}.
%\vspace{-2em}
%\input{algorithms/find_config}
%%%%
%%%% Background
\begin{comment}
     
    Dense: 
    - "8:8"
    Unstructured sparse is 
    - "flexible N: fix M"

    Data itself: 
    View? 

    Matrix (c)
    matrix c is sparse. -- data 
    Matrix C has 2:4 sparsity patterns. -- compression format
    Matrix C has unstructured sparsity patterns -- compression format
    Matrix C has flexible N:8 sparsity patterns.
    
    Matrix C is 2:4 sparse.
    Matrix C is unstructured sparse. 
    Matrix C is flexible N:8 sparse.

    Matrix A is 2:4 sparse. -- false
    Matrix A is unstructured sparse. 
    
    Matrix A is flexible N:8 sparse. -- yes
    Matrix B is flexible N:8 sparse. -- yes
    Dense and unstructured sparsity are same?
    
    Matrix B is 2:4 sparse.
    Matrix B is unstructured sparse. 

    "Dense" in HW and SW means differently

    tensor
    "a view of a tensor" from SW
    "a view of a tensor" from HW
    architecture contract
    
    
    flexible N:M == unstructrued sparsity pattern
\end{comment}

\begin{comment}
To summarize, there are two main research questions in this project.
\begin{enumerate}
    \item Could TASD be applied to DNN models without losing significant accuracy compared with the baseline model?
    \item What are the efficient accelerator architecture and programming model to support TASD?
\end{enumerate}

\end{comment}
%%%% TASD
\begin{comment}
With the insight from \autoref{subsec:tasd_analysis}, we propose a sparsity-degree-based method to choose the TASD configuration based on the sparsity degree of each layer.
Consider a flexible structured sparse HW with 2:4 and 2:8 support as the target, 
to express the approximated sparsity, the sparsity degree covered by a TASD configuration $C$, we use $S(C)$.
For example, $S([2:4]) = 50\%$ while $S([2:4, 2:8]) = 25\%$.
There are four TASD configurations available with the target HW, $H_1$ = [1:1], $H_2$ = [2:4, 2:8], $H_3$ = [2:4], and $H_4$ = [2:8] where the corresponding sparsity covered by the TASD configuration is 0\%, 25\%, 50\%, and 75\%.

We use a hyperparameter, $\alpha$, to tune the aggressiveness of the TASD approximation. 
For a given layer $L_i$ and the TASD configurations available to the target HW ($H_1, ... , H_4$ for this case), we choose $C_i$ as $H_j$ where j is the largest integer where $S(L_i) + \alpha > H_j$.
If we use a larger $\alpha$, we choose the TASD configuration more aggressively (allowing more dropped non-zeros). 
We summarize the algorithm in \autoref{lst:tasd}.
We use TCONV/TFC to indicate a CONV/FC layer with TASD as shown in \autoref{fig:conv-tconv}, and the TASD configurations found above would be applied to the corresponding TCONV/TFC layers.
In \autoref{fig:conv-tconv} (a), we show how the conventional CONV/FC layer works with unstructured sparse activations (usually from ReLU) with dense weights. In \autoref{fig:conv-tconv} (b) shows how a TCONV/TFC layer works. As explained above, TASDER would modify unstructured sparse weights to structured sparse weights with TASD-W.
\vspace{-1em}
\input{algorithms/find_config}
\vspace{-1em}
\end{comment}

\begin{comment}
% PDF For ConvNEXT Pseudo Density
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-pseudo-density.png}
        %\vspace{-1.5em}
	\caption{PDF of the element magnitude of an activation tensor from a GELU-based DNN, \textit{ConvNext-Tiny}. TASD-A uses a pseudo-density heuristic for non-ReLU DNNs.}
	\label{fig:tasd-pseudo-density}
 \vspace{-1em}
\end{figure}
\end{comment}
\begin{comment}
For simplicity, let $B$ be an unstructured sparse matrix representing input activations (usually derived by the image-to-column algorithm to convert a convolution operation into a general matrix multiplication, GEMM with $D = A \times B + C$ where $A$, $C$, and $D$ refer to a weight, bias, and output, respectively).  

Then, the matrix multiplication $AB$ can be expressed as $A(B_1 + B_2) = AB_1 + AB_2$ and each $AB_i$ can be executed on a sparse tensor core which supports 2:4 structured sparsity (such as the ones in NVIDIA Ampere GPUs).
However, this decomposition does not reduce the number of computations required for the entire $AB$, so it cannot improve performance under the same number of Multiply and Accumulate (MAC) units.
\end{comment}
\begin{comment}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.47\textwidth]{figures/uniform_result.pdf}
 \vspace{-0.5em}
	\caption{Percentages of dropped non-zeros and the sum of dropped non-zeros after applying different TASD series on a matrix generated with \textbf{uniform random distribution}.}
	\label{fig:uniform_result}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-w.pdf}
	\caption{ResBlocks from ResNet50 with CONV and TCONV layers.}
	\label{fig:tasd-w}
\end{figure}
\end{comment}

\section{Po-An's brain dump}
Sparsity in the DNNs gives a huge opportunity to improve efficiency and performance, by eliminating storing, transferring, and computing on zeros. The most effective and natural way to induce sparsity while preserving accuracy is to introduce sparsity across the whole network and make a global decision on 1) which elements (in both weight and activation tensors) and 2) how much (sparsity degree) to introduce zeros. This HW-agnostic design space and preference from the developer leads to a friendlier abstraction toward unstructured sparsity, because the designer does not need to think about HW, just to focus on the network accuracy and flops/model size tradeoff.

Nonetheless, unstructured sparsity often is incompatible with the popular and emerging parallel HW architecture that serves the DNN need well. For example, unstructured sparsity introduces irregular memory accesses and diverged control/execution patterns that are hostile to parallel HW GPU and specialized HW like tensor core/systolic array.

To address this issue, a new method to bridge between sparsity and its HW performance is to introduce extra design spaces that are parallel HW-oriented, namely structure (or the degree of structuredness) and granularity. Such design space forces the DNN designer to induce sparsity with certain constraints at a cost of achievable sparsity degree for iso-accuracy comparison, but promises predictable performance and energy efficiency benefits on top of the existing parallel or specialized HW. For example, NVIDIA's fine-grained structured sparsity support balances the imposed constraints and achievable performance and provides a good target for DNN developers to optimize the network for.

However, such methods also move the burden from the HW designers to DNN developers, as there is already a massive design space (network architecture, training recipe, hyperparameters) to explore. Moreover, extending the existing support to more patterns (e.g., not only 2:4, cite VEGETA and S2TA) also means more overhead and burden for both HW designers and DNN developers.

In this paper, we ask "how can we design a system to provide the free and simple unstructured sparse interface to the DNN developers, but only use structured sparse HW support while providing predictable performance and efficiency gains?" Our answer is to redefine the DL sparsity programming abstraction and introduce a level of indirection through DL system SW and HW. Specifically, we introduce an idea named structured tensor decomposition to approximate any unstructured sparse tensor with a series of structured sparse tensors. Leveraging the distributed property of tensor algebra, we further propose to dynamically "decode" an unstructured sparse tensor algebra operation into a series of "microcode", structured sparse tensor algebra operations, which are efficient and compatible with existing parallel and specialized HW architecture. 

%%%% Eval
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/acc_flop_resnet50_overview.pdf}
	\caption{Evaluation of TASD-A on ResNet50.}
	\label{fig:maccounts}
\end{figure}


\begin{comment}
\subsection{
Impact of TASD configuration search
}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/greedy-search.pdf}
         \vspace{-2em}
	\caption{
        \rev{EDP comparison between different TASD configuration selection methods on Sparse ResNet50. CHANGE THIS TO TABLE!!
        }
 }
	\label{fig:greedy-search}
 \end{figure}

In \autoref{subsec:tasd-w}, we introduced a simple, per-layer sparsity-based heuristic to determine the TASD configuration.
Such a heuristic may not lead to the optimal configuration for the whole DNN that preserves 99\% model quality and minimizes total computation.
To address this, we design and implement another greedy-based algorithm that optimizes across all layers.
This greedy algorithm first measures the percentage of dropped non-zero elements of each TASD configuration for all layers and sorts the configuration-layer pairs by their percentage of dropped elements.
Next, it greedily applies the TASD configuration based on the sorted order until the model quality is <99\% of the original model (i.e., prioritize the option with the smallest dropped non-zeros).


We find that this global, greedy-search-based method further improves EDP for TTC-VEGETA-M8 by 18\%, and TTC-VEGETA-M4 by 10\% for sparse ResNet50, which shows that finding a high-quality TASD configuration can further improve the effectiveness. 
We leave developing the optimal algorithm leveraging other metrics for future work. 
\end{comment}

\begin{comment}    
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-networkwise-a.pdf}
 \vspace{-0.5em}
	\caption{
 \rev{Network-wise and Layer-wise TASD-A on dense ResNet50.}
 }
	\label{fig:resnet50-95-networkwise-a}
\end{figure}
\end{comment}    

\begin{comment}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-layerwise-a.pdf}
 \vspace{-0.5em}
	\caption{Layer-wise TASD-A on dense ResNet50.}
	\label{fig:resnet50-95-layerwise-a}
\end{figure}
\end{comment}
\begin{comment}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-a-maccounts.pdf}
         \vspace{-0.5em}
	\caption{Layer-wise TASD-A on more DNN models.}
	\label{fig:maccounts}
 \end{figure}
\end{comment}

\begin{comment}    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-layerwise-w.pdf}
 \vspace{-0.0em}
	\caption{Layer-wise TASD-W on sparse ResNet50.}
	\label{fig:resnet50-95-layerwise-w}
\end{figure}
\end{comment}



%%% Table
\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/tables/comparison.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
%\newcommand{\xmark}{ %\textcolor{darkyellow}{\ding{56}}}
\newcommand{\xmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}

\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
&
{\textbf{Dense}}
&
{\textbf{Unstructured}}
&
{\textbf{Structured}}
&

\\
&
{\textbf{Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Pruned Model}}
&

\\
\hline
Sparsity Degree
&
None
&
High
&
Low-Mid
&
{\textbf{Extra}}
\\
\cline{1-4}
Fine-tuning Time
%& \textbf{Intrinsics} 
&
None
&
Short
&
Long
&
{\textbf{Area}}
\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& None
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured HW
\end{tabular}
& \downmark
& \upmark
& \xmark~or \upmark
& High
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured HW
\end{tabular}
& \xmark
& \xmark
& \upmark
& Low
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark %~(TASD-A)
& \upmark
& \upmark
& Low
\\
\hline

\end{tabular}

\hfill
\caption{Comparison of sparse DNN models and sparse DNN HW supports.  \upmark~: Better than dense HW in EDP (Energy Delay Product). \downmark~: Worse than dense HW in EDP. \xmark~: No EDP Improvement.}
%\vspace{-1.em}
\label{table:nm-hw}
\end{table}

==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/tables/comparison2.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
%\newcommand{\xmark}{ %\textcolor{darkyellow}{\ding{56}}}
\newcommand{\xmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}

\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
&
{\textbf{Dense}}
&
{\textbf{Unstructured}}
&
{\textbf{Structured}}
&
{\textbf{Extra}}
\\
&
{\textbf{Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Area}}
\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense HW~\cite{jouppi2017tpu}
\end{tabular}
& \xmark
& \xmark
& \xmark
& None
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstr. HW~\cite{qin2020sigma,parashar2017scnn,wang:dual-side}
\end{tabular}
& \downmark
& \upmark
& \xmark~or \upmark
& High
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Str. HW~\cite{liu2021s2ta,jeong:vegeta}
\end{tabular}
& \xmark
& \xmark
& \upmark
& Low
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark %~(TASD-A)
& \upmark
& \upmark
& Low
\\
\hline

\end{tabular}

\hfill
\caption{Comparison of sparse DNN models and sparse DNN HW supports. \xmark~: No EDP Improvement over dense HW. \upmark~: Better than dense HW in EDP (Energy Delay Product). \downmark~: Worse than dense HW in EDP. }
\vspace{-1.em}
\label{table:nm-hw}
\end{table}

==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/tables/comparison3.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
%\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
\newcommand{\xmark}{ \textcolor{darkred}{\ding{56}}}
\newcommand{\hmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}
\begin{scriptsize}
\begin{table}[t] 
\scriptsize
\centering
\caption{Comparison of DNN HWs. Unstr: Unstructured sparse. Str: Structured sparse. Wgt: Weights. Act: Activations.}
\begin{tabular}{|c|c|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
HW Support
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Str}}
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Area}}

\\
$\downarrow$
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Act}}
&{\textbf{Act}}
&
{\textbf{Cost}}

\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense~\cite{jouppi2017tpu, nvidia_volta, rasa}
\end{tabular}
& \cmark
& \xmark
& \xmark %\xmark~or \upmark
& \cmark
& \xmark
& \cmark\cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstr~\cite{qin2020sigma,parashar2017scnn,wang:dual-side}
\end{tabular}
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
%\tablefootnote{Unstructured sparse HW could be energy efficient if the workload is very sparse, which is not often the case for DNN models.}
& \cmark
& \cmark %\xmark~or \upmark
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
& \cmark
& \xmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Str~\cite{zhu2019micro, liu2020sta,jeong:vegeta, nvidia_ampere}
\end{tabular}
& \cmark
& \xmark
& \cmark
& \cmark
& \xmark
& \cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \cmark %~(TASD-A)
& \cmark
& \cmark
& \cmark\cmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[7]
%\tablefootnote{TASD enables further acceleration through approximation.}
& \cmark 
& \cmark
\\
\hline

\end{tabular}

\hfill
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\begin{minipage}{1.0\linewidth}
\footnotemark[1]{With extra wiring/logic, unstructured sparse HW is inefficient if the tensor is dense.}\mbox{}\hfill
\end{minipage}
\begin{minipage}{1.0\linewidth}
\footnotemark[7]{TASD enables further acceleration by approximating dense tensors with sparse tensors.}\mbox{}\hfill
\end{minipage}

\vspace{-2.5em}
\label{table:nm-hw}
\end{table}
\end{scriptsize}


==> mlsys_arxiv_qgydymzpsvvgmcpzhxqmcnkjpjwzgfmz/mlsys2025style/tables/comparison4.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
%\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
\newcommand{\xmark}{ \textcolor{darkred}{\ding{56}}}
\newcommand{\hmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}
\begin{small}
\begin{table*}[!ht] 
\small
\centering
\caption{Comparison of DNN HWs. Unstr: Unstructured sparse. Str: Structured sparse. Wgt: Weights. Act: Activations.}
\begin{tabular}{|c|c|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
HW Support
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Str}}
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Area}}

\\
$\downarrow$
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Act}}
&{\textbf{Act}}
&
{\textbf{Cost}}

\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense~\cite{jouppi2017tpu, nvidia_volta, rasa}
\end{tabular}
& \cmark
& \xmark
& \xmark %\xmark~or \upmark
& \cmark
& \xmark
& \cmark\cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstr~\cite{qin2020sigma,parashar2017scnn,wang:dual-side}
\end{tabular}
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
%\tablefootnote{Unstructured sparse HW could be energy efficient if the workload is very sparse, which is not often the case for DNN models.}
& \cmark
& \cmark %\xmark~or \upmark
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
& \cmark
& \xmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Str~\cite{zhu2019micro, liu2020sta, nvidia_ampere,jeong:vegeta}
\end{tabular}
& \cmark
& \xmark
& \cmark
& \cmark
& \xmark
& \cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \cmark %~(TASD-A)
& \cmark
& \cmark
& \cmark\cmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[7]
%\tablefootnote{TASD enables further acceleration through approximation.}
& \cmark 
& \cmark
\\
\hline

\end{tabular}

\hfill
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\begin{minipage}{1.0\linewidth}
\footnotemark[1]{With extra wiring/logic, unstructured sparse HW is inefficient if the tensor is dense.}\mbox{}\hfill
\end{minipage}
\begin{minipage}{1.0\linewidth}
\footnotemark[7]{TASD enables further acceleration by approximating dense tensors with sparse tensors.}\mbox{}\hfill
\end{minipage}

%\vspace{-2.5em}
\label{table:nm-hw}
\end{table*}
\end{small}


==> sections/1_intro_old.tex <==
\section{Introduction}

\TK{pls rewrite! see my comment on slack}

DNNs have revolutionized various domains, such as computer vision~\cite{krizhevsky2012alexnet,convnext,vit}, personal recommendation~\cite{dlrm}, speech recognition~\cite{deepspeech2}, and natural language processing~\cite{gpt2,devlin-etal-2019-bert}. 
%Meanwhile, DNNs are also demanding more computation for diverse model capabilities and higher operational performance. The DNN models are scaling to billions of model parameters \cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron} often with high-resolution 2D and 3D inputs~\cite{lin2017focal,cciccek20163d} under real-time requirements.
Meanwhile, DNN inference is also demanding more computation as they scale to billions of model parameters \cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron} and consume an enormous amount of input data~\cite{lin2017focal,cciccek20163d}.
%Recently, Deep Learning (DL) has achieved great success across various domains including, but not limited to, computer vision, personal recommendation, speech recognition, and natural language processing~\cite{lecun2015deep}. 
%To squeeze out the full potential of DNN models with large datasets and powerful compute resources, one of the recent trends is making the model deeper and larger, often exceeding billions or trillions model parameters such as Megatron, PaLM, and Switch Transformer~\cite{fedus2021switch, chowdhery2022palm, shoeybi2019megatron}.
%On the other hand, some DNN models use high-resolution inputs to exploit more information from the input to achieve higher accuracy while incurring larger intermediate feature maps as the trade-off.
%The enormous number of parameters and large feature maps cause huge memory footprint as well as an extremely large number of computations, which is a critical problem for both edge devices and datacenter computers.
%Since performance is an overloaded term, we distinguish computational (i.e., latency, throughput, etc.) and operational (i.e., the accuracy of DNN classification) performance in this paper.
To address the increasing demand for DNN models, researchers propose to exploit \emph{sparsity} in DNN models.  
%Fortunately, researchers have found a technique called model compression to reduce the memory footprint and improve performance.
%that there are two sparsities that they can exploit to reduce the burden; weight (static) sparsity and input (dynamic) sparsity; the former is extrinsic while the latter is intrinsic.
%Weight sparsity is the result of a well-known model compression technique, model pruning~\cite{han2015deep}, which removes a set of parameters in the target DNN model based on certain rules, thereby potentially reducing both memory footprint and the required number of computations. 
Model pruning~\cite{han2015deep} is the most popular method to remove a set of parameters in the target DNN model based on certain criteria, inducing \emph{weight sparsity}.
%Weight sparsity is often called as static sparsity since the sparsity pattern is fixed across different inferences using the model.
This optimization exploits a phenomenon that empirically, large models are often overly parameterized and do not need all parameters to maintain the target accuracy at inference time.
Deep learning (DL) model developers prefer to induce \textbf{unstructured sparsity} on weights so that they can focus on developing pruning algorithms to achieve better model accuracy and computation/model size trade-offs without any restriction.
Also, many DNN models naturally exhibit \emph{activation sparisty} due to the rectified linear unit (ReLU) that clips negative activation values to zeros, which induces unstructured activation sparsity.

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/tasd-high-level-fig.pdf}
 \vspace{-1.5em}
	\caption{Different flows to exploit sparsity in DNNs.}
 \vspace{-1.5em}
	\label{fig:tasd-high-level-fig}
\end{figure}
%While unstructured sparsity is the preferred method to compress DNNs, 
As a result, early sparse DNN accelerators~\cite{parashar2017scnn,wang:dual-side,qin2020sigma} target unstructured sparsity and can accelerate any sparse DNNs.
Unfortunately, unstructured sparsity support is challenging to deploy as a specialized HW unit 
%support for unstructured sparsity in commercial devices, 
as it causes significant area and energy overhead for indexing logic and flexible distribution/reduction logic~\cite{jeong:vegeta}.
Without native HW support, unstructured sparsity in DNNs lead to irregular memory accesses and diverged control/execution patterns, which are hostile to parallel architectures like GPUs%
\footnote{The only sparse DNN accelerators on commercial devices is NVIDIA Sparse Tensor Core\cite{nvidia_ampere}, which supports a fixed 2:4 
 structured sparsity.} and specialized tensor accelerators like tensor core and systolic array. 
This forces DNN model developers today to constrain the DNN sparsity search space to only consider coarse-grained \emph{structured patterns}, such as channel or filter pruning~\cite{molchanov2022lana, chen2022coarsening}, while maintaining iso-accuracy, thereby, moving the burden to DNN model developers.

%To address this issue, an alternative to bridge
%DNN sparsity and HW performance is to introduce extra design
%spaces that are parallel HW-oriented, namely structure (or
%the degree of structuredness) and granularity.
To balance the need, recently, hardware (HW) designers~\cite{nvidia_ampere,jeong:vegeta,liu2021s2ta,zhu2019micro} have proposed \emph{fine-grained} structured sparsity support.
Such designs force DNN developers to induce sparsity with certain constraints at a cost of achievable sparsity degree for iso-accuracy comparison, but promise predictable performance
gain on top of the existing DNN supports.
For example, NVIDIA’s fine-grained 2:4 structured sparsity support balances the imposed constraints and achievable performance and provides a good target for DNN developers to optimize the network for.
However, such methods impose an extra burden on DNN developers on top of the existing huge design space (DNN architectures, training recipes, etc.) to explore. Moreover, extending the existing support to more patterns~\cite{jeong:vegeta, sun2021domino} means more overhead and design space exploration for both HW designers and DNN developers.
We summarize different flows to exploit sparsity in \autoref{fig:tasd-high-level-fig}.

%In this paper, we ask "how can we design a system to provide the unstructured sparse interface to the DNN developers, but only with structured sparse hardware support, while providing predictable performance and efficiency gains?" 
\textbf{In this paper}, we ask ``Can we design a system to expose the flexible unstructured sparse interface to the DNN developers, but only with the efficient, less flexible structured sparse HW support?" 
Our answer is to introduce a new level of abstraction between DL model developers and hardware designers, similar to the abstraction layer in the instruction-set architectures. Specifically, we introduce a method, structured sparse tensor decomposition, to approximate any sparse tensor with a series of structured sparse tensors.
Leveraging the distributed property of tensor algebra,
we further propose to dynamically "decode" an unstructured
sparse tensor algebra into a series of "microcode", i.e., structured sparse tensor algebra, which are efficient and compatible with prior structured sparse hardware.
%\TK{I think somewhere in this section or in the first bullet a strong statement like ``First work to .." will be nice to have}
%To exploit the benefits of both approaches, we propose a novel method, Tensor Approximation via Structured Decomposition (TASD) and show how it can be used to leverage unstructured input sparsity using a set of structured sparse tensors.
%Furthermore, we have observed that different layers prefer different TASD configurations, so we propose an efficient method to choose TASD configurations per layer to minimize accuracy loss while maximizing performance gain.

We make the following contributions: 
\begin{itemize}
    \item We present the first work to bridge unstructured sparse DNN and structured sparse HW with Tensor Approximation via Structured Decomposition (TASD), which approximate any sparse tensor with a series of structured sparse tensors.
    \item We propose a framework, TASDER, which finds the TASD series for each DNN layer to accelerate dense/sparse DNNs with structured sparse hardware.
    \item We propose a simple architectural extension and dataflow on top of existing structured sparse accelerators~\cite{jeong:vegeta} to execute TASD series efficiently.
    \item For various off-the-shelf dense and sparse DNNs, we show that TASD improves EDP by up to 83\% and by 70\% on average. We also show that across a range of DNNs, TASD can reduce the computation by 40\%. We validate the effectiveness of TASD on a real NVIDIA GPU and achieve up to 39\% speed-up.
\end{itemize}


\begin{comment}
The organization of the paper is the following.
\begin{itemize}
    \item Section 2 reviews the background in DNN sparsity and
how DNN developers induce sparsity, as well as previous HW support DNN sparsity. We also show why
providing unstructured sparse HW support might not
be the best solution.
    \item Section 3 explains the idea of TASD and a preliminary analytical study of how effective TASD is as an
approximation method.
    \item Section 4 describes a TASD-based HW and SW codesign that enables the DNN developer to freely induce
sparsity without structured and granularity constraints.
    \item Section 5 shows the evaluation of the proposed system,
as well as a case study of applying TASD on off-the-shelf HW (NVIDIA Ampere GPUs).
    \item Finally, we discuss extra related work in Section 6 and conclude this paper in section 7.
\end{itemize}
\end{comment}

%Thus, For example, the only commercial HW that can leverage sparsity for efficient calculation is NVIDIA Sparse Tensor Core.
%During the pruning, This HW-agnostic design space and preference from the developer leads to a friendlier abstraction toward unstructured
%sparsity, because the designer does not need to think about
%HW, just to focus on the network accuracy and flops/model size tradeoff.





==> sections/backups.tex <==
%%%%
\subsection{Search algorithm for TASD selection}
\begin{algorithm}[tb]
   \caption{TASD Selection Algorithm}
   \label{alg:tasd_sel}
\begin{algorithmic}
   \STATE {\bfseries Input:} $target\_sparsity$, $alpha$, $H$
   \STATE $target\_sparsity = sparsity + alpha$
   \IF{$target\_sparsity > H[3]$}
   \STATE return $H[3]$
   \ENDIF
   \IF{$target\_sparsity > H[2]$}
   \STATE return $H[2]$
   \ENDIF
   \IF{$target\_sparsity > H[1]$}
   \STATE return $H[1]$
   \ENDIF
   \IF{$target\_sparsity > H[0]$}
   \STATE return $H[0]$
   \ENDIF
\end{algorithmic}
\end{algorithm}

In \autoref{alg:tasd_sel}, we show the sparsity-degree-based TASD Selection algorithm explained in \autoref{subsec:tasd-w}.
%\vspace{-2em}
%\input{algorithms/find_config}
%%%%
%%%% Background
\begin{comment}
     
    Dense: 
    - "8:8"
    Unstructured sparse is 
    - "flexible N: fix M"

    Data itself: 
    View? 

    Matrix (c)
    matrix c is sparse. -- data 
    Matrix C has 2:4 sparsity patterns. -- compression format
    Matrix C has unstructured sparsity patterns -- compression format
    Matrix C has flexible N:8 sparsity patterns.
    
    Matrix C is 2:4 sparse.
    Matrix C is unstructured sparse. 
    Matrix C is flexible N:8 sparse.

    Matrix A is 2:4 sparse. -- false
    Matrix A is unstructured sparse. 
    
    Matrix A is flexible N:8 sparse. -- yes
    Matrix B is flexible N:8 sparse. -- yes
    Dense and unstructured sparsity are same?
    
    Matrix B is 2:4 sparse.
    Matrix B is unstructured sparse. 

    "Dense" in HW and SW means differently

    tensor
    "a view of a tensor" from SW
    "a view of a tensor" from HW
    architecture contract
    
    
    flexible N:M == unstructrued sparsity pattern
\end{comment}

\begin{comment}
To summarize, there are two main research questions in this project.
\begin{enumerate}
    \item Could TASD be applied to DNN models without losing significant accuracy compared with the baseline model?
    \item What are the efficient accelerator architecture and programming model to support TASD?
\end{enumerate}

\end{comment}
%%%% TASD
\begin{comment}
With the insight from \autoref{subsec:tasd_analysis}, we propose a sparsity-degree-based method to choose the TASD configuration based on the sparsity degree of each layer.
Consider a flexible structured sparse HW with 2:4 and 2:8 support as the target, 
to express the approximated sparsity, the sparsity degree covered by a TASD configuration $C$, we use $S(C)$.
For example, $S([2:4]) = 50\%$ while $S([2:4, 2:8]) = 25\%$.
There are four TASD configurations available with the target HW, $H_1$ = [1:1], $H_2$ = [2:4, 2:8], $H_3$ = [2:4], and $H_4$ = [2:8] where the corresponding sparsity covered by the TASD configuration is 0\%, 25\%, 50\%, and 75\%.

We use a hyperparameter, $\alpha$, to tune the aggressiveness of the TASD approximation. 
For a given layer $L_i$ and the TASD configurations available to the target HW ($H_1, ... , H_4$ for this case), we choose $C_i$ as $H_j$ where j is the largest integer where $S(L_i) + \alpha > H_j$.
If we use a larger $\alpha$, we choose the TASD configuration more aggressively (allowing more dropped non-zeros). 
We summarize the algorithm in \autoref{lst:tasd}.
We use TCONV/TFC to indicate a CONV/FC layer with TASD as shown in \autoref{fig:conv-tconv}, and the TASD configurations found above would be applied to the corresponding TCONV/TFC layers.
In \autoref{fig:conv-tconv} (a), we show how the conventional CONV/FC layer works with unstructured sparse activations (usually from ReLU) with dense weights. In \autoref{fig:conv-tconv} (b) shows how a TCONV/TFC layer works. As explained above, TASDER would modify unstructured sparse weights to structured sparse weights with TASD-W.
\vspace{-1em}
\input{algorithms/find_config}
\vspace{-1em}
\end{comment}

\begin{comment}
% PDF For ConvNEXT Pseudo Density
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-pseudo-density.png}
        %\vspace{-1.5em}
	\caption{PDF of the element magnitude of an activation tensor from a GELU-based DNN, \textit{ConvNext-Tiny}. TASD-A uses a pseudo-density heuristic for non-ReLU DNNs.}
	\label{fig:tasd-pseudo-density}
 \vspace{-1em}
\end{figure}
\end{comment}
\begin{comment}
For simplicity, let $B$ be an unstructured sparse matrix representing input activations (usually derived by the image-to-column algorithm to convert a convolution operation into a general matrix multiplication, GEMM with $D = A \times B + C$ where $A$, $C$, and $D$ refer to a weight, bias, and output, respectively).  

Then, the matrix multiplication $AB$ can be expressed as $A(B_1 + B_2) = AB_1 + AB_2$ and each $AB_i$ can be executed on a sparse tensor core which supports 2:4 structured sparsity (such as the ones in NVIDIA Ampere GPUs).
However, this decomposition does not reduce the number of computations required for the entire $AB$, so it cannot improve performance under the same number of Multiply and Accumulate (MAC) units.
\end{comment}
\begin{comment}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.47\textwidth]{figures/uniform_result.pdf}
 \vspace{-0.5em}
	\caption{Percentages of dropped non-zeros and the sum of dropped non-zeros after applying different TASD series on a matrix generated with \textbf{uniform random distribution}.}
	\label{fig:uniform_result}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-w.pdf}
	\caption{ResBlocks from ResNet50 with CONV and TCONV layers.}
	\label{fig:tasd-w}
\end{figure}
\end{comment}

\section{Po-An's brain dump}
Sparsity in the DNNs gives a huge opportunity to improve efficiency and performance, by eliminating storing, transferring, and computing on zeros. The most effective and natural way to induce sparsity while preserving accuracy is to introduce sparsity across the whole network and make a global decision on 1) which elements (in both weight and activation tensors) and 2) how much (sparsity degree) to introduce zeros. This HW-agnostic design space and preference from the developer leads to a friendlier abstraction toward unstructured sparsity, because the designer does not need to think about HW, just to focus on the network accuracy and flops/model size tradeoff.

Nonetheless, unstructured sparsity often is incompatible with the popular and emerging parallel HW architecture that serves the DNN need well. For example, unstructured sparsity introduces irregular memory accesses and diverged control/execution patterns that are hostile to parallel HW GPU and specialized HW like tensor core/systolic array.

To address this issue, a new method to bridge between sparsity and its HW performance is to introduce extra design spaces that are parallel HW-oriented, namely structure (or the degree of structuredness) and granularity. Such design space forces the DNN designer to induce sparsity with certain constraints at a cost of achievable sparsity degree for iso-accuracy comparison, but promises predictable performance and energy efficiency benefits on top of the existing parallel or specialized HW. For example, NVIDIA's fine-grained structured sparsity support balances the imposed constraints and achievable performance and provides a good target for DNN developers to optimize the network for.

However, such methods also move the burden from the HW designers to DNN developers, as there is already a massive design space (network architecture, training recipe, hyperparameters) to explore. Moreover, extending the existing support to more patterns (e.g., not only 2:4, cite VEGETA and S2TA) also means more overhead and burden for both HW designers and DNN developers.

In this paper, we ask "how can we design a system to provide the free and simple unstructured sparse interface to the DNN developers, but only use structured sparse HW support while providing predictable performance and efficiency gains?" Our answer is to redefine the DL sparsity programming abstraction and introduce a level of indirection through DL system SW and HW. Specifically, we introduce an idea named structured tensor decomposition to approximate any unstructured sparse tensor with a series of structured sparse tensors. Leveraging the distributed property of tensor algebra, we further propose to dynamically "decode" an unstructured sparse tensor algebra operation into a series of "microcode", structured sparse tensor algebra operations, which are efficient and compatible with existing parallel and specialized HW architecture. 

%%%% Eval
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/acc_flop_resnet50_overview.pdf}
	\caption{Evaluation of TASD-A on ResNet50.}
	\label{fig:maccounts}
\end{figure}


\begin{comment}
\subsection{
Impact of TASD configuration search
}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/greedy-search.pdf}
         \vspace{-2em}
	\caption{
        \rev{EDP comparison between different TASD configuration selection methods on Sparse ResNet50. CHANGE THIS TO TABLE!!
        }
 }
	\label{fig:greedy-search}
 \end{figure}

In \autoref{subsec:tasd-w}, we introduced a simple, per-layer sparsity-based heuristic to determine the TASD configuration.
Such a heuristic may not lead to the optimal configuration for the whole DNN that preserves 99\% model quality and minimizes total computation.
To address this, we design and implement another greedy-based algorithm that optimizes across all layers.
This greedy algorithm first measures the percentage of dropped non-zero elements of each TASD configuration for all layers and sorts the configuration-layer pairs by their percentage of dropped elements.
Next, it greedily applies the TASD configuration based on the sorted order until the model quality is <99\% of the original model (i.e., prioritize the option with the smallest dropped non-zeros).


We find that this global, greedy-search-based method further improves EDP for TTC-VEGETA-M8 by 18\%, and TTC-VEGETA-M4 by 10\% for sparse ResNet50, which shows that finding a high-quality TASD configuration can further improve the effectiveness. 
We leave developing the optimal algorithm leveraging other metrics for future work. 
\end{comment}

\begin{comment}    
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-networkwise-a.pdf}
 \vspace{-0.5em}
	\caption{
 \rev{Network-wise and Layer-wise TASD-A on dense ResNet50.}
 }
	\label{fig:resnet50-95-networkwise-a}
\end{figure}
\end{comment}    

\begin{comment}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-layerwise-a.pdf}
 \vspace{-0.5em}
	\caption{Layer-wise TASD-A on dense ResNet50.}
	\label{fig:resnet50-95-layerwise-a}
\end{figure}
\end{comment}
\begin{comment}
    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tasd-a-maccounts.pdf}
         \vspace{-0.5em}
	\caption{Layer-wise TASD-A on more DNN models.}
	\label{fig:maccounts}
 \end{figure}
\end{comment}

\begin{comment}    
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/resnet50-95-layerwise-w.pdf}
 \vspace{-0.0em}
	\caption{Layer-wise TASD-W on sparse ResNet50.}
	\label{fig:resnet50-95-layerwise-w}
\end{figure}
\end{comment}



%%% Table
\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


==> tables/comparison.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
%\newcommand{\xmark}{ %\textcolor{darkyellow}{\ding{56}}}
\newcommand{\xmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}

\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
&
{\textbf{Dense}}
&
{\textbf{Unstructured}}
&
{\textbf{Structured}}
&

\\
&
{\textbf{Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Pruned Model}}
&

\\
\hline
Sparsity Degree
&
None
&
High
&
Low-Mid
&
{\textbf{Extra}}
\\
\cline{1-4}
Fine-tuning Time
%& \textbf{Intrinsics} 
&
None
&
Short
&
Long
&
{\textbf{Area}}
\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& None
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured HW
\end{tabular}
& \downmark
& \upmark
& \xmark~or \upmark
& High
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured HW
\end{tabular}
& \xmark
& \xmark
& \upmark
& Low
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark %~(TASD-A)
& \upmark
& \upmark
& Low
\\
\hline

\end{tabular}

\hfill
\caption{Comparison of sparse DNN models and sparse DNN HW supports.  \upmark~: Better than dense HW in EDP (Energy Delay Product). \downmark~: Worse than dense HW in EDP. \xmark~: No EDP Improvement.}
%\vspace{-1.em}
\label{table:nm-hw}
\end{table}

==> tables/comparison2.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
%\newcommand{\xmark}{ %\textcolor{darkyellow}{\ding{56}}}
\newcommand{\xmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
%\newcommand{\cmark}{\ding{51}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}

\begin{comment}

\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models}
&
\multicolumn{2}{c|}{\textbf{Off-the-shelf}}
&
\multicolumn{2}{c|}{\textbf{Extra training}}
\\
\cline{2-5}
\textbf{} 
%& \textbf{Intrinsics} 
&
\textbf{Dense}~\cite{torchvision}
&
\textbf{Sparse}~\cite{SparseZoo}
&
\textbf{Dense}
&
\textbf{Sparse}
%& 
%\textbf{Row-wise}
\\
%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Unstructured Sparse HW
\end{tabular}
& \downmark
& \upmark
& \downmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Structured Sparse HW
\end{tabular}
& \xmark
& \xmark
& \xmark
& \upmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark
& \upmark
& \upmark
& \upmark
\\
\hline

\end{tabular}
\label{tab1}
\label{table:nm-hw}
\hfill
\caption{Comparison of different sparse DNN supports. \upmark: Better than dense. \downmark: Worse than dense. \xmark: No Gain.\TK{This table is a little confusing to me. I think ``Sparse" is ambiguous - is it structured or unstructured. For off-the shelf i understand it means unstructured .. but then sparse in extra training meaning structured right? And what does dense in extra training signify? What does extra training and creating dense mean in the context of TASD work?}}
\vspace{-1.5em}
\end{table}

\end{comment}


\begin{table}[t] 
\scriptsize
\centering
\begin{tabular}{|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
&
{\textbf{Dense}}
&
{\textbf{Unstructured}}
&
{\textbf{Structured}}
&
{\textbf{Extra}}
\\
&
{\textbf{Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Pruned Model}}
&
{\textbf{Area}}
\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense HW~\cite{jouppi2017tpu}
\end{tabular}
& \xmark
& \xmark
& \xmark
& None
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstr. HW~\cite{qin2020sigma,parashar2017scnn,wang:dual-side}
\end{tabular}
& \downmark
& \upmark
& \xmark~or \upmark
& High
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Str. HW~\cite{liu2021s2ta,jeong:vegeta}
\end{tabular}
& \xmark
& \xmark
& \upmark
& Low
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \upmark %~(TASD-A)
& \upmark
& \upmark
& Low
\\
\hline

\end{tabular}

\hfill
\caption{Comparison of sparse DNN models and sparse DNN HW supports. \xmark~: No EDP Improvement over dense HW. \upmark~: Better than dense HW in EDP (Energy Delay Product). \downmark~: Worse than dense HW in EDP. }
\vspace{-1.em}
\label{table:nm-hw}
\end{table}

==> tables/comparison3.tex <==
\definecolor{darkred}{rgb}{.65,0,0}
\definecolor{darkgreen}{rgb}{0,.5,0}
\definecolor{darkyellow}{rgb}{0.95,.6,0.1}
%\newcommand{\cmark}{ \textcolor{darkgreen}{\ding{52}}}
\newcommand{\xmark}{ \textcolor{darkred}{\ding{56}}}
\newcommand{\hmark}{ %\textcolor{darkyellow}
{\textbf{--}}}
\newcommand{\upmark}{ \textcolor{darkgreen}{\ding{115}}}
\newcommand{\downmark}{ \textcolor{darkred}{\ding{116}}}

%\newcommand{\xmark}{\ding{54}}%
\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}%
%\newcommand{\circlemark}{\ding{108}}
%\newcommand{\tmark}{\ding{115}}
\begin{scriptsize}
\begin{table}[t] 
\scriptsize
\centering
\caption{Comparison of DNN HWs. Unstr: Unstructured sparse. Str: Structured sparse. Wgt: Weights. Act: Activations.}
\begin{tabular}{|c|c|c|c|c|c||c|}
\hline
%\multirow{2}{*}{\textbf{DNN Model}}
HW Support
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Str}}
&
{\textbf{Dense}}
&
{\textbf{Unstr}}
&
{\textbf{Area}}

\\
$\downarrow$
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Wgt}}
&
{\textbf{Act}}
&{\textbf{Act}}
&
{\textbf{Cost}}

\\

%\cline{2-4} 
\hline
\hline

\begin{tabular}[c]{@{}c@{}}
Dense~\cite{jouppi2017tpu, nvidia_volta, rasa}
\end{tabular}
& \cmark
& \xmark
& \xmark %\xmark~or \upmark
& \cmark
& \xmark
& \cmark\cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Unstr~\cite{qin2020sigma,parashar2017scnn,wang:dual-side}
\end{tabular}
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
%\tablefootnote{Unstructured sparse HW could be energy efficient if the workload is very sparse, which is not often the case for DNN models.}
& \cmark
& \cmark %\xmark~or \upmark
& \xmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[1]
& \cmark
& \xmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
Str~\cite{zhu2019micro, liu2020sta,jeong:vegeta, nvidia_ampere}
\end{tabular}
& \cmark
& \xmark
& \cmark
& \cmark
& \xmark
& \cmark
\\
\hline

\begin{tabular}[c]{@{}c@{}}
\textbf{TASD} (This work)
\end{tabular}
& \cmark %~(TASD-A)
& \cmark
& \cmark
& \cmark\cmark\renewcommand{\thefootnote}{\fnsymbol{footnote}}\footnotemark[7]
%\tablefootnote{TASD enables further acceleration through approximation.}
& \cmark 
& \cmark
\\
\hline

\end{tabular}

\hfill
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\begin{minipage}{1.0\linewidth}
\footnotemark[1]{With extra wiring/logic, unstructured sparse HW is inefficient if the tensor is dense.}\mbox{}\hfill
\end{minipage}
\begin{minipage}{1.0\linewidth}
\footnotemark[7]{TASD enables further acceleration by approximating dense tensors with sparse tensors.}\mbox{}\hfill
\end{minipage}

\vspace{-2.5em}
\label{table:nm-hw}
\end{table}
\end{scriptsize}

